Learning to Deceive Knowledge Graph Augmented Models via Targeted Perturbation

Knowledge graphs (KGs) have helped neural models improve performance on various knowledge-intensive tasks, like question answering and item recommendation. By using attention over the KG, such KG-augmented models can also "explain" which KG information was most relevant for making a given prediction. In this paper, we question whether these models are really behaving as we expect. We show that, through a reinforcement learning policy (or even simple heuristics), one can produce deceptively perturbed KGs, which maintain the downstream performance of the original KG while significantly deviating from the original KG's semantics and structure. Our findings raise doubts about KG-augmented models' ability to reason about KG information and give sensible explanations.

==> backup/0_abstract_old_sep27.tex <==
% !TEX root = main.tex
Recent commonsense question answering and recommendation systems rely on knowledge graphs to provide them with critical external knowledge to boost their performance. Further, the provided knowledge is claimed to serve as the explanation for the KG-augmented models' prediction. In this work, we challenge the faithfulness of KG in providing interpretability and their contribution to the models' improvement by perturbing the underlying KG.
We introduce various perturbation strategies ranging from simple heuristics, where we randomly perturb the edges or relations, to more targeted perturbation with reinforcement learning. %Through the use of heuristics we randomize the relations and the structure of the KG, for example permuting the set of relations and analyze the performance on the downstream task. Using reinforcement learning we perturb the graph in a more targeted way to analyze the effect on the downstream task. 
% \ryan{adding a sentence briefly mentioning what the randomization/heuristics do, may be good, to help the reader understand the significance of our claims/findings below.}
% These perturbation strategies randomize the
Our study shows that despite significant perturbation, the models maintain a competitive performance, indicating that KG is not being appropriately utilized.
%We observe that on some tasks even after corrupting the KG completely with simple heuristics we are able to maintain the performance of the downstream task. On other tasks we are able to get competitive performance after perturbing the complete KG with the reinforcement learning perturbation policy, thus indicating that the KG might not be properly utilized in these tasks.
% Our study shows that the models could still maintain a competitive performance, indicating that KG is not being appropriately utilized. 
What's worse, this implies the model is prone to predict based on the wrong reason and casts doubt on KG's ability to explain. 
We thus aim to raise awareness about the soundness of leveraging KG as the provider of both knowledge and explanation.
% Therefore, this paper aims to raise awareness about the soundness of leveraging KG as the provider of both knowledge and explanation.
% We thus aim to raise the awareness of the researchers in this field about the justness of leveraging KG as the provider of both knowledge and explanation.




==> backup/Exp_Sep29.tex <==
% !TEX root = main.tex

\section{Experiments}
\label{sec:exp}
\vspace{-0.2cm}

In this section we introduce our experimental setup. With the help of these experiments we try to validate our hypothesis that current models on many tasks do not model the KG effectively. We use different types of perturbation techniques to show even if the KG is completely corrupted we can maintain the downstream performance. We also perform some analysis on the paths that the models deem important for a prediction which pose questions on the interpretability of such models.

% \vspace{-0.2cm}
% \subsection{Experiment Setup}
% \vspace{-0.2cm}

\vspace{-0.2cm}
\subsection{Baselines for Graph Perturbations}
\vspace{-0.2cm}

In addition to the Relation Swapping(RS) and Greedy Relation Replacement(GRR) perturbation heuristics described in~\ref{sec: pilotexpts}, we further introduce two other perturbation methods as baselines in our experiments.

\textbf{Edge Rewiring (ER): } It alters the structure of the graph but keep the relation distribution across the KG constant. In this heuristic we first randomly select an edge $(h,r,t)$ in the KG. We denote by $\mathcal{N}(h)$, the set of neighbors for the node/entity $h$. Let $k \in \mathcal{E} \setminus \mathcal{N}(h)$. 
Then:
\begin{align}\label{rewiring-heuristic}
    \mathcal{T} \leftarrow (\mathcal{T} \setminus \{(h,r,t)\}) \cup \{(h,r,k)\}
\end{align}
 

\textbf{Edge Deletion (ED):} We randomly select an edge and delete it.
% \begin{align}\label{eq:deletion-heuristic}
%   &i \sim \text{UniformDiscrete}\{1,2,\ldots,|\mathcal{T}|\} \\
% %   ,\quad \text{for } j=1,2,\ldots\\
%     &\mathcal{T} \leftarrow \mathcal{T} \setminus \{e_i=(h,r,t)\} \nonumber
% \end{align}\noindent
This heuristic clearly changes both the structure of the graph as well as the distribution of relations across the KG.
This is a heuristic that clearly changes both the structure of the graph as well as the relation distribution across the KG. 
A very interesting observation should be that the embedding based evaluation metric will fail to recognize these perturbations to the KG by design. Since even if we delete edges the remaining edges are still valid triples of the KG which in turn keeps this evaluation metric almost unchanged.

% In the next subsection we denote Relation Swapping Heuristic and Greedy Heuristic as Semantic Heuristic 1 and Semantic Heuristic 2 respectively. We denote Deletion Heuristic and Rewiring Heuristic as Structure Heuristic 1 and Structure Heuristic 2 respectively. Next we introduce the tasks on which we perform our experiments.

% \vspace{-0.2cm}
% \subsection{Implementation Details}
% \vspace{-0.2cm}

  

\subsection{Experiments on Question Answering}
\vspace{-0.2cm}

We first introduce our experimental setup for the commonsense question answering task.

\xiang{what is the task/problem setting (input and output, goal)? Should introduce before going into models..}

\textbf{Datasets.} In addition to CommonsenseQA dataset that we introduced in section\ref{sec: pilotexpts}, we also exhibit our experiments on \textbf{OpenBookQA} which is a question answering dataset that consists of science questions and shows improvement in performance after augmenting a Language Model with a KG. The labels for the official test set are available and we report our results on the official test set. We run our experiments MHGRN \citep{feng2020scalable}, RelationNet \citep{santoro2017simple} and Graph Networks \citep{battaglia2018relational}.

\textbf{Graph Encoders.} In addition to MHGRN which was introduced in section \ref{sec: pilotexpts}, we also use \textbf{Relation Networks} \citep{santoro2017simple} and \textbf{Graph Networks} \citep{battaglia2018relational} adapted for the commonsense question answering task for our experiments.

\textbf{Evaluation Metrics.} As discussed above, the embedding based validation score is not very robust to structure changes in the KG. To this end we suggest the \textbf{clustering coefficient based evaluation metric}. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$ we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$ i.e $\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
    where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$
% \ryan{This strategy looks at triangles that are all homogeneous in terms of their relation $r$, what about triangles that are not all of the same relation $r$, but mixed relations? There are typically far more of these, just by chance. But in any case, its unclear why they were ignored. It was probably done since the above way just makes it simple to apply standard algorithms, but hopefully we have a more solid reason and justification for this.}
We then compute the relation specific clustering coefficient vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective} of the $i^{th}$ node and compute the average clustering vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e $\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$
We denote by $\mathbf{c_{o}}$, the average clustering vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{c_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ i.e
$V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$
with $b$ as a constant for avoiding zero division.

\textbf{Results and Discussion.}
For experiments on Question Answering, we take the complete conceptnet graph and prune it first such that it only contains edges that are relevant for the given dataset i.e for each edge either the head entity or the tail entity is a part of the given dataset. In table \ref{tab:results:csqa} we report our results after perturbing all the triples of the KG. We also report the embedding based and the clustering coefficient evaluation metric to get an idea about how much corrupted the KG is. From table\ref{tab:results:csqa} we observe that using heuristic perturbations the performance almost always drop to the level of non KG baseline on the CSQA dataset. Whereas on the OBQA dataset we observe that even with a randomly corrupted KG, we are able to maintain the performance. Using Reinforcement Learning based  targeted perturbation policy we observe that on both graph models with CSQA we achieve a statistically significant improvement according to the t-test over both heuristics and non KG baselines. With the help of our human evaluations we also show the edges on which the model gives more weight are not interpretable and the few interpretable edges can also be corrupted.

We also plot curves to monitor the change in performance of MHGRN with CSQA for different types of perturbations. From figure\ref{fig:final_curves}, we observe that for all scales of perturbations the RL policy can keep the performance of the model better than the heuristics and also better than the non KG baseline which validates our RL policy. We also observe that the RL policy is able to perturb the KG to the same extent if not more as is evident from the drastic drop in evaluation metrics.

\textbf{Human Evaluation on Model Explanation.}
\xiang{let’s write out the human evaluation paragraph and talk about the scores, inter-annotator agreement metric, and correlation metric}
We also conduct human evaluations on the edges and paths that are deemed important by models according to attention weights. We take 10 question from the test which are predicted correctly by the model and extract paths with the highest attention weights. We then ask human annotators to annotate each path for its validity and interpretability. The average scores over the 10 question instances over 5 annotators is reported in Table~\ref{tab:user_study}.



% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on CommonsenseQA and OBQA perturbation experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA and on the official set of OBQA}
% \label{tab:results:csqa}
% \scalebox{0.62}{
% \begin{tabular}{lcccccccccccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{8}{c}{ \textbf{CSQA}}&\multicolumn{8}{c}{ \textbf{OBQA}}\\
%     \cmidrule(lr){2-9} \cmidrule(lr){10-17}
%     & \multicolumn{4}{c}{ \textbf{RN}}&\multicolumn{4}{c}{ \textbf{MHGRN}} &\multicolumn{4}{c}{ \textbf{RN}} &\multicolumn{4}{c}{ \textbf{MHGRN}}\\
%     \cmidrule(lr){2-5}
%     \cmidrule(lr){6-9}
%     \cmidrule(lr){10-13}
%     \cmidrule(lr){14-17}
%     & Acc & Emb & CC & DC &  Acc & Emb & CC & DC & Acc & Emb & CC & DC  & Acc & Emb & CC & DC \\
%     \midrule
%     {w/o KG $^{\dagger}$} & ~53.71 & - & - & - & ~53.71 & - & - & - & ~62.00 & - & - & - & ~62.00 & -&-&- \\
%     \midrule
%     {w KG} & 56.87 & 9.4E-1&-&- & 56.87 & 9.4E-1&-&- & 58.97 & 9.3E-1&-&- & 58.97 & 9.3E-1&-&- \\
%     {Relation Swapping} & 53.42 & 8.3E-1&1.6E-1&6.2E-3 & 52.21 & 9.3E-1&1.4E-1&2.0E-3 & 66.80 & 8.5E-1&1.8E-1&7.8E-3 & 66.80 & 9.2E-1&1.5E-1&2.2E-3 \\
%     {Greedy} & 53.42 & 3.3E-1&1.0E-1&1.7E-3 & 52.53 & 5.6E-1&1.3E-1&5.4E-4 & 66.80 & 2.7E-1&1.1E-1&1.8E-3 & 66.60 & 6.2E-1&1.7E-1&7.3E-3 \\
%     {Rewiring} & 55.12 & 3.1E-1&1.1E-1&1.1E-2 & 54.15 & 5.1E-1&8.2E-2&5.2E-4 & 66.40 & 2.7E-1&1.0E-1&1.8E-3 & 66.60 & 6.5E-1&1.6E-1&8.8E-3 \\
%     {Deletion} & 57.21 & 9.4E-1/-/- & 57.21 & 9.4E-1&-&- & 68 & 9.3E-1&-&- & 68 & 9.3E-1&-&- \\
%     {RL Relation} & 53.42 & 8.3E-1&1.6E-1&6.2E-3 & 51.00 & 9.3E-1&1.4E-1&2.0E-3 & 67.80 & 8.5E-1&1.8E-1&7.8E-3 & 67.60 & 9.2E-1&1.5E-1&2.2E-3 \\
%     {RL Edge} & 53.74 & 3.3E-1&1.0E-1&1.7E-3 & 53.02 & 6.4E-1&1.6E-1&6.1E-3 & 67.60 & 2.7E-1&1.1E-1&1.8E-3 & 67.00 & 6.5E-1&1.6E-1&8.8E-3 \\
%     % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
%     % \midrule
%     % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
%     % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
%     % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*} 

\begin{table*}[t]
\centering
\caption{\textbf{Performance comparison on CommonsenseQA and OBQA perturbation experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA and on the official set of OBQA. 
\xiang{Use full names for the baselines?}
}
\label{tab:results:csqa}
\scalebox{0.62}{
\begin{tabular}{lcccccccccccc}
    \toprule  
    \multirow{2}{*}{\textbf{Methods}}&
    \multicolumn{6}{c}{ \textbf{CSQA}}&\multicolumn{6}{c}{ \textbf{OBQA}}\\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13}
    & \multicolumn{3}{c}{ \textbf{RN}}&\multicolumn{3}{c}{ \textbf{MHGRN}} &\multicolumn{3}{c}{ \textbf{RN}} &\multicolumn{3}{c}{ \textbf{MHGRN}}\\
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    \cmidrule(lr){11-13}
    & Acc & Emb & CC &  Acc & Emb & CC & Acc & Emb & CC  & Acc & Emb & CC \\
    \midrule
    {w/o KG $^{\dagger}$} & ~53.71 & - & - & ~53.71 & - & - & ~62.00 & - & - & ~62.00 & -&- \\
    \midrule
    {w KG} & 56.87 & 0.94&- & 57.21 & 0.94&- & 66.80 & 0.93&- & 68.00 & 0.93&- \\
    {RS} & 53.42 & 0.83&0.17 & 53.42 & 0.83& 0.17 & 67.00 & 0.86&0.18& 67.80& 0.86&0.18 \\
    {GRR} & 53.42 & 0.33&0.10 & 52.22 & 0.33&0.10 & 66.80 & 0.27&0.11 & 67.60 & 0.27&0.11 \\
    {ER} & 53.42 & 0.56&0.13 & 52.22 & 0.56&0.13 & 66.60 & 0.62&0.17 & 67.00 & 0.62&0.17 \\
    {ED} & 52.21 & 0.93&0.14 & 51.00 & 0.93&0.14 & 66.80 & 0.92&0.16 & 67.60 & 0.92&0.16 \\
    {RL Relation} & 55.12 & 0.31&0.11 & 54.63 & 0.31&0.10 & 66.40 & 0.27&0.10 & 67.20 & 0.28&0.11 \\
    {RL Edge} & 54.15 & 0.51&0.08 & 54.15 & 0.54&0.07 & 66.60 & 0.41&0.16 & 67.20 & 0.34&0.09 \\
    % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
    % \midrule
    % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
    % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
    % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    \bottomrule 
\end{tabular}
}
\vspace{-0.1cm}
\end{table*} 

\begin{figure}[tb!]
\centering
\subfloat[][Test Acc on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Rel_Acc_MHGRN.png}}
\subfloat[][Emb Val Score]{\includegraphics[width=0.25\textwidth]{figures/Rel_Val_Score_MHGRN.png}}
\subfloat[][Test Acc on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Edge_Acc_MHGRN.png}}
\subfloat[][Degree Val Score]{\includegraphics[width=0.25\textwidth]{figures/EDGE_val_MHGRN.png}}
\caption{Variation of Performance and Validation Scores with scale of perturbation on MHGRN with CSQA}
\label{fig:final_curves}
\end{figure}

\begin{table}[t]
\parbox{0.33\linewidth}{
\small
\scalebox{0.8}{
    \begin{tabular}{lrrrr}
\toprule
\multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c}{CSQA} & \multicolumn{2}{c}{OBQA} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} & Val. & Int. & Val. & Int. \\
\midrule
Ori.& 3.03&2.17&3.48&2.17  \\
\midrule
RL1 &2.68&2.19&2.82&1.90\\
RL2 &2.99&2.29&2.79&2.09\\
\bottomrule
    \end{tabular}}
    \caption{User Study on Paths}
    \label{tab:user_study}
}
%\quad
\parbox{0.33\linewidth}{
\small
\begin{tabular}{lccc}
\toprule
        Model & Test Acc & Emb  \\
        \midrule
         Model1& 56 & 0.46\\
         Model2& 56 & 0.46\\
         Model3& 56 & 0.46\\
\bottomrule
    \end{tabular}
    \caption{Ablation Study}
    \label{tab:ablation}
}
%\quad
\parbox{0.33\linewidth}{
\small
\begin{tabular}{lrr}
\toprule
& RN&MHGRN\\
\midrule
+ KG&56.87&57.21\\
+ zero&53.10&53.99\\
+ rand&52.60&52.48\\
\bottomrule
\end{tabular}
\caption{Results of randomized baselines on CSQA.}
\label{tab:randomized_baseline}
}
\end{table}




\subsection{Experiments on Recommender Systems}
\vspace{-0.2cm}

\xiang{what is the task/problem setting (input and output, goal)? Should introduce before going into models..}

\textbf{Datasets:} In addition to the Last.FM dataset that we introduced in section \ref{sec: pilotexpts} we also demonstrate our experiments on the MovieLens 20M dataset. This dataset consists of approximately 20 million explicit ratings (ranging from 1 to 5) from the MovieLens website.

\textbf{Graph Encoders: }In addition to KGCN that we introduced in section \ref{sec: pilotexpts} we also experiment on RippleNet as a recommendation model. 

\textbf{Evaluation Metric.}
The KG used for recommendation tasks have a very low value of low clustering coefficient. Therefore we introduce another evaluation metric robust to structural changes namely \textbf{degree evaluation metric}. Similar to the clustering coefficient based evaluation metric we first create a set of graphs $\mathcal{G}^{r}$ for each relation $r \in \mathcal{R}$. We then calculate the relation specific degree vector $\mathbf{d^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{d^r}$ represents the degree of the $i^{th}$ node and calculate the average degree vector $\mathbf{d}$ for the whole graph as the mean of $\mathbf{d^r}$ over all $r \in \mathcal{R}$ i.e $\mathbf{d} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{d^r}$
We denote by $\mathbf{d_{o}}$, the average degree vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{d_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$ i.e
$
V_{dc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{d_{o}} - \mathbf{d_{p}} \rVert_2 + b}.
$

\textbf{Results and analysis: }As in the CommonsenseQA task we report our results after perturbing all the triples in the KG. Since clustering coefficient based evaluation metric is not very suitable for this task, we report the degree evaluation metric along with the embedding based evaluation metric. The key takeaway from table\ref{tab:results:reco} is that even after perturbing the KG by a significant amount the change in performance is statistically insignificant no matter what type of perturbation we do. These results provide a strong evidence to us for validating our claims.

We also plot curves showing the variation of performance with scale of perturbation on KGCN with Last.FM dataset. The important point to note from the curves is that the drop in performance is insignificant for all scales of perturbation but the KG changes considerable as can be seen from the drastic drop in the evaluation metrics.
\begin{table*}[t]
\centering
\vspace{-0.2cm}
\caption{\textbf{Performance comparison on recommendation based perturbation experiments} We report the test AUC on Last.FM and MovieLens-20M}
\label{tab:results:reco}
\scalebox{0.65}{
\begin{tabular}{lcccccccccccc}
    \toprule  
    \multirow{2}{*}{\textbf{Methods}}&
    \multicolumn{6}{c}{ \textbf{Last.FM}}&\multicolumn{6}{c}{ \textbf{MovieLens 20M}}\\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13}
    & \multicolumn{3}{c}{ \textbf{KGCN}}&\multicolumn{3}{c}{ \textbf{RippleNet}} &\multicolumn{3}{c}{ \textbf{KGCN}} &\multicolumn{3}{c}{ \textbf{RippleNet}}\\
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    \cmidrule(lr){11-13}
    & AUC & Emb&DC &  AUC & Emb&DC & AUC & Emb&DC  & AUC & Emb&DC \\
    \midrule
    {w/o KG $^{\dagger}$} & ~50.75 & -&- & ~50.75 & -&- & ~91.30 & -&- & ~91.30 & -&- \\
    \midrule
    {w KG} & 55.99 & 0.97&- & 56.23 & 0.95&- & 96.62 & 0.96&- & 96.62 & 0.96&- \\
    {RS} & 55.98 & 0.68&0.97 & 56.23 & 0.78&0.97 & 96.62 & 0.68&0.18 & 97.46 & 0.61&0.17 \\
    {GRR} & 55.98 & 0.42&0.34 & 56.22 & 0.50&0.34 & 96.50 & 0.41&0.12 & 97.45 & 0.46&0.13 \\
    {ER} & 56.04 & 0.44&0.41 & 56.22& 0.44&0.43 & 96.24 & 0.68&0.07 & 96.62 & 0.68&0.07 \\
    {ED} & 55.96 & 0.94&0.36 & 56.21 & 0.94&0.36 & 96.36 & 0.98&0.03 & 97.22 & 0.98&0.03 \\
    {RL Relation} & 56.23 & 0.95&- & 56.23 & 0.95&- & 97.46 & 0.96&- & 97.46 & 0.96&- \\
    {RL Edge} & 56.23 & 7.8E-1&9.6E-1 & 56.21 & 9.4E-1&3.6E-1 & 97.46 & 6.1E-1&1.7E-1 & 97.43 & 9.3E-1&3.1E-2 \\
    % {RippleNet- Heuristic2} & 56.22 & 4.9E-1/-/3.4E-1 & 52.22 & 7.8E-1/-/4.2E-1 & 97.45 & 4.5E-1/-/1.3E-1 & 93.62 & 7.9E-1/-/7.6E-2 \\
    % {RippleNet- RL} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    \bottomrule 
\end{tabular}
}
\vspace{-0.1cm}
\end{table*}

\begin{figure}[tb!]
\vspace{-0.2cm}
\centering
\subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_AUC_Music.png}}
\subfloat[][Emb Val Score]{\includegraphics[width=0.25\textwidth]{figures/Relation_Val_score_music.png}}
\subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Edge_AUC_Music.png}}
\subfloat[][Degree Val Score]{\includegraphics[width=0.25\textwidth]{figures/Edge_Val_score_music.png}}
\vspace{-0.2cm}
\caption{Variation of Performance and Validation Scores with scale of perturbation on KGCN with Last.FM}
\label{fig:heur_curvesKGCN}
\end{figure}
% % In addition to MHGRN which we introduced in \ref{sec: pilotexpts} we also experiment on the following models for Commonsense Question Answering. 

% \textbf{Relation Net \citep{santoro2017simple}}: This is a path based model that has been adapted by \citep{feng2020scalable} for commonsense question answering. We use this model as it is simple yet powerful for the Commonsense Question Answering task. We augment this model with bert-base and use it on the CSQA \citep{talmor-etal-2019-commonsenseqa} and with roberta-large to use it on OBQA \citep{mihaylov-etal-2018-suit}. 

% \textbf{Graph Networks \citep{battaglia2018relational}}: Graph Networks is a general framework of encoding relational graphs such as a KG which we adapt to perform Commonsense Question Answering. As for Relation Net we augment this model with bert-base on CSQA and with roberta-large on OBQA.

% Since we will also perturb the structure of the KG, we need some evaluation metric that is more robust to structural changes than the ones introduced \ref{sec: pilotexpts}. To this end we introduce the following evaluation metric:

% \textbf{Clustering Coefficient based evaluation metric}: We design this evaluation metric in a way that it is robust to structural perturbation to the KG as well as perturbation to the edge types. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$ we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$ i.e $\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
%     where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$
% % \ryan{This strategy looks at triangles that are all homogeneous in terms of their relation $r$, what about triangles that are not all of the same relation $r$, but mixed relations? There are typically far more of these, just by chance. But in any case, its unclear why they were ignored. It was probably done since the above way just makes it simple to apply standard algorithms, but hopefully we have a more solid reason and justification for this.}
% We then calculate the relation specific clustering coefficient vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective} of the $i^{th}$ node and calculate the average clustering vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e $\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$
% We denote by $\mathbf{c_{o}}$, the average clustering vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{c_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ i.e
% $$V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$$
% with $b$ as a constant for avoiding zero division.

% \subsection{Recommendation}
% We introduce KGCN in \ref{sec: pilotexpts} for showcasing our pilot experiments. For this task we also work on the following model

% \textbf{Ripplenet \citep{wang2018ripplenet}} This is a KG based recommendation model that combines path based encoding and embedding based encoding of a KG. We use this model on the Last.FM and the Movie-Lens 20M datasets.

% One thing to note here is that we have a different KG for each dataset. The local clustering coefficients for the KG in this task are very small and do not provide much information. Thus for this task we introduce another evaluation metric which is quite similar to the clustering coefficient based evaluation metric.

%  \textbf{Degree Coefficient based evaluation metric: } Similar to the clustering coefficient based evaluation we first create a set of graphs $\mathcal{G}^{r}$ for each relation $r \in \mathcal{R}$. We then calculate the relation specific degree vector $\mathbf{d^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{d^r}$ represents the degree of the $i^{th}$ node and calculate the average degree vector $\mathbf{d}$ for the whole graph as the mean of $\mathbf{d^r}$ over all $r \in \mathcal{R}$ i.e $$\mathbf{d} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{d^r}$$
% We denote by $\mathbf{d_{o}}$, the average degree vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{d_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$ i.e
% \begin{equation}
% V_{dc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{d_{o}} - \mathbf{d_{p}} \rVert_2 + b}.
% \end{equation}

% To perturb the KG to a much lower evaluation metric while preserving the accuracy, we use DQNs to model the process.To ensure we only perturb relevant facts in the KG, we extract the subgraph containing only those concepts that appear in the Question Answer statements.

% We decompose the perturbation of a relation edge into three sub-actions: choosing a subject, choosing a object connected with the chosen subject, and substituting the relation edge between the chosen subject and object with another one. We choose the first sub-action randomly at each step, and use two DQNs to predict the reward after a fixed number of steps for the other two sub-actions.
% After a fixed number of steps, we use the change of accuracy on downstream tasks as the rewards.

% We've also tried 2 variants of DQN.

% For DQN Variant 1,
% we use the difference in probabilities of the correct answer in place of accuracy as the reward. We feel this can be a more informative reward.

% For DQN Variant 2, in order to make evaluation metric as low as possible,
% we use only 1 DQN to select the tail entity and use the relation that has the lowest evaluation metric as the action. Here we only use the probability change as reward and use the greedy strategy to decrease the evaluation metric.

% In comparison, we use two random methods for perturbation.  The heuristic 1 is that we select two edges at random and swap relations and heuristic 2 is we choose tail relation randomly and select the relation which minimizes the val metric of the triple.

% Results show that our RL method does work.

% Currently our DQN method does not contain previous actions as states, but only gives predictions based on current actions. Therefore, at evaluation, if we choose the same first sub-action, the second and third sub-action will be the same, which will limit the total number of changes. 
% Therefore, we'll next try to contain previous actions as states, and use it to make more changes. This will make evaluation metric much lower.
% In addition to the models, introduced in \ref{sec: pilotexpts} we also experiment on the following models.
% % \subsection{Heuristics}
% % We consider the following heuristics as a baseline for comparison of the experiments.

% % \textbf{Heuristic1}: Choose two edges at random and swap relations. (Write it more formally)

% % \textbf{Heuristic2}: Choose an edge at random and select the relation that minimizes the embedding based evaluation metric.(Write it more formally)

% % \textbf{Edge Heuristic1}: Select an edge at random and delete it. (Write it more formally)

% % \textbf{Edge Heuristic2}: Choose an edge at random and a third node at random. Remove the original edge and add it to the third node.

% % \subsection{Question Answering}
% % We experiment on the following Question Answering datasets. We also mention the Graph Encoder used in each of them. For this set of experiments we take the complete conceptnet graph and prune it first such that it only contains edges that are relevant for the given dataset i.e for each edge either the head entity or the tail entity is a part of the given dataset.

% % \textbf{CommonsenseQA}: CommonsenseQA is a commonsense question answering benchmark dataset that is derived from conceptnet and is one of those tasks which requires external knowledge in the form of a KG to perform well. Since the labels for the official test are not available we report our results on the inhouse test split of \citep{lin2019kagnet}. We exhibit our experiments on this dataset using MHGRN \citep{feng2020scalable}, RelationNet \citep{santoro2017simple} and Graph Networks \citep{velivckovic2018graph}. 

% % \textbf{OpenBookQA}: OpenBookQA is question answering dataset that consists of science questions which shows improvement in performance after augmenting a Language Model with a KG. The labels for the official test set are available and we report our results on the official test set. As in the case of CSQA we run our experiments on MHGRN, RelationNet and Graph Networks. 

% % \subsection{Recommendation}
% % We experiment on the following Recommendation datasets. We also mention the Graph Encoder used in each of them.

% % \textbf{Last.FM}: Last.FM contains user rating information on musicians and music from a set of 2 thousand users from Last.fm online music system. We demonstrate our experiments on this dataset on KGCN and Ripplenet

% % \textbf{MovieLens 20M}: MovieLens 20M is a widely used benchmark dataset in movie recommendations, which consists of approximately 20 million explicit ratings (ranging from 1 to 5) on the MovieLens website. We showcase our experiments on this dataset using KGCN and Ripplenet.
% \textbf{Relation Net \citep{santoro2017simple}}: This is a path based model that has been adapted by \citep{feng2020scalable} for commonsense question answering. We use this model as it is simple yet powerful for the COmmonsense Question Answering task. We augment this model with bert-base and use it on the CSQA \citep{talmor-etal-2019-commonsenseqa} and with roberta-large to use it on OBQA \citep{mihaylov-etal-2018-suit}. 

% \textbf{Graph Networks \citep{battaglia2018relational}}: Graph Networks is a general framework of encoding relational graphs such as a KG which we adapt to perform Commonsense Question Answering. As for Relation Net we augment this model with bert-base on CSQA and with roberta-large on OBQA.

% \textbf{Ripplenet \citep{wang2018ripplenet}} This is a KG based recommendation model that combines path based encoding and embedding based encoding of a KG. We use this model on the Last.FM and the Movie-Lens 20M datasets.

% In the next subsection we introduce some baseline methods for the perturbation of KG.
% \subsection{Baseline Methods}
% We introduced some heuristic perturbation methods in section \ref{sec: pilotexpts}. Now we introduce some other baselines to compare our perturbation policy in addition to those introduced in \ref{sec: pilotexpts}.

% \textbf{Rewiring Heuristic: } This is a heuristic that we design to alter the structure of the graph but keep the relation distribution across the KG constant. In this heuristic we first select an edge $(h,r,t)$ randomly. We denote by $\mathcal{N}(v)$, the set of neighbors of the node v. Let $k \in \mathcal{E} \setminus \mathcal{N}(h)$. 
% Then:
% \begin{align}\label{rewiring-heuristic}
%     \mathcal{T} \leftarrow \mathcal{T} \setminus \{(h,r,t)\} \cup \{(h,r,k)\}
% \end{align}
 

% \textbf{Deletion Heuristic:} In this heuristic we randomly select an edge and delete it.
% \begin{align}\label{eq:deletion-heuristic}
%   &i \sim \text{UniformDiscrete}\{1,2,\ldots,|\mathcal{T}|\} \\
% %   ,\quad \text{for } j=1,2,\ldots\\
%     &\mathcal{T} \leftarrow \mathcal{T} \setminus \{e_i=(h,r,t)\} \nonumber
% \end{align}\noindent
% This heuristic clearly changes both the structure of the graph as well as the distribution of relations across the KG.
% This is a heuristic that clearly changes both the structure of the graph as well as the relation distribution across the KG. 
% A very interesting observation should be that the embedding based evaluation metric will fail to recognize these perturbations to the KG by design. Since even if we delete edges the remaining edges are still valid triples of the KG which in turn keeps this evaluation metric almost unchanged. 
% For the next section we denote Relation Swapping Heuristic and Greedy Heuristic as Semantic Heuristic 1 and Semantic Heuristic 2 respectively. We denote Deletion Heuristic and Rewiring Heuristic as Structure Heuristic 1 and Structure Heuristic 2 respectively

% We also introduce two more evaluation metrics in this section that are more robust to structure of the KG than the embedding based evaluation metric.

% \textbf{Clustring Coefficient/Degree based evaluation metrics} We design this evaluation metric in a way that it is robust to structural perturbation to the KG as well as perturbation to the edge types. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$ we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$ i.e $\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
%   where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$
% We then calculate the relation specific clustering coefficient vector/ degee vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective}/ degree of the $i^{th}$ node and calculate the average clustering vector/ degree vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e $$\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$$
% We denote by $\mathbf{c_{o}}$, the average clustering/degree vector of the unperturbed KG and denote the average clustering/degree vector of the perturbed KG with $\mathbf{c_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ i.e
% $$V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$$
% with $b$ as a constant for avoiding zero division.

% In the next section we report our results and analysis of our experiments.

% \begin{table}[t]
% \parbox{0.45\linewidth}{
%     \begin{tabular}{lrrrr}
% \toprule
% \multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c}{CSQA} & \multicolumn{2}{c}{OBQA} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} & Val. & Int. & Val. & Int. \\
% \midrule
% Ori.& 3.03&2.17&3.48&2.17  \\
% \midrule
% RL1 &2.68&2.19&2.82&1.90\\
% RL2 &2.99&2.29&2.79&2.09\\
% \bottomrule
%     \end{tabular}
%     \caption{User Study on Paths}
%     \label{tab:user_study}
% }
% \quad
% \parbox{0.55\linewidth}{
% \begin{tabular}{c|c}
% \toprule
%          &  \\
%          & 
%     \end{tabular}
%     \caption{Abalation Study}
%     \label{tab:ablation}
% }
% \end{table}

==> backup/backup_Nov15/0_abstract.tex <==
% !TEX root = main.tex
\vspace{-0.2cm}
% by Xiang
Symbolic knowledge (e.g., entities, relations, and facts in a knowledge graph) has become an increasingly popular component of neural-symbolic models applied to machine learning tasks, such as question answering and recommender systems. Besides improving downstream performance, these symbolic structures (and their associated attention weights) are often used to help explain the model's predictions and provide ``insights" to practitioners. 
In this paper, we question the faithfulness of such symbolic explanations. We demonstrate that, through a learned strategy (or even simple heuristics), one can produce deceptively perturbed symbolic structures which maintain the downstream performance of the original structure while significantly deviating from the original semantics. In particular, we train a reinforcement learning policy to manipulate relation types or edge connections in a knowledge graph, such that the resulting downstream performance is maximally preserved. Across multiple models and tasks, our approach drastically alters knowledge graphs with little to no drop in performance. These results raise doubts about the faithfulness of explanations provided by learned symbolic structures and the reliability of current neural-symbolic models in leveraging symbolic knowledge.

%%% old version
% Recent commonsense question answering and recommendation systems rely on knowledge graphs to provide them with critical external knowledge to boost their performance. Further, the provided knowledge is claimed to serve as the explanation for the KG-augmented models' prediction. In this work, we challenge the faithfulness of KG in providing interpretability and their contribution to the models' improvement by perturbing the underlying KG.
% We introduce various perturbation strategies ranging from simple heuristics, where we randomly perturb the edges or relations, to more targeted perturbation with reinforcement learning.
% Our study shows that despite significant perturbation, the models maintain a competitive performance, indicating that KG is not being appropriately utilized.
% What's worse, this implies the model is prone to predict based on the wrong reason and casts doubt on KG's ability to explain. 
% We thus aim to raise awareness about the soundness of leveraging KG as the provider of both knowledge and explanation.

==> backup/backup_Nov15/1_introduction.tex <==
% !TEX root = main.tex
\section{Introduction}
\vspace{-0.1cm}

%%% 1st paragraph: neural-symbolic models which incorporate symbolic structures from external knowledge graph are gaining growing popularity. 
% --> what are these models like in general?
% --> they are gaining popularity because: 1) improved accuracy on downstream tasks (e.g., overcoming data sparsity in recommendation; augmenting with commonsense knowledge in QA); and 2) these structures, in conjunction with the learn attention weights, are claimed to help provide explanation of model predictions. [Cite papers that claiming the above points].
%%

% Aaron
Recently, neural reasoning over symbolic knowledge graphs (KGs) has emerged as a popular paradigm for various machine learning tasks, such as question answering (QA) ~\citep{lin2019kagnet, feng2020scalable, Lv2020GraphBasedRO}, recommender systems~\citep{wang2018ripplenet, wang2019aknowledge, wang2019knowledge}, and natural language inference (NLI) ~\citep{kapanipathi2020infusing, wang2019improving}. 
For a given data instance, such neural-symbolic KG (NSKG) methods extract a relevant subgraph from the KG, use a neural network to encode the subgraph -- either via message passing ~\citep{wang2018ripplenet,wang2019aknowledge} or path pooling~\citep{lin2019kagnet,feng2020scalable} -- then use the subgraph encoding to make a prediction. 
This incorporation of KG information has been shown to improve performance on a number of downstream tasks: for QA, the KG provides additional context about how a given answer choice is related to the question~\citep{talmor2018commonsenseqa}; for recommender systems, the KG mitigates data sparsity and cold start issues~\citep{wang2018shine}.
Besides improving performance, the KG can also be used to help explain the model's predictions, through inspection of high-scoring reasoning paths~\citep{feng2020scalable, lin2019kagnet, cao2019unifying, gao2019explainable}.

% Recently the neural-symbolic models which  incorporate symbolic structures from external knowledge graphs (KGs) are gaining growing popularity in machine learning tasks such as recommender systems~\citep{wang2018ripplenet, wang2019aknowledge, wang2019knowledge}, question answering~\citep{lin2019kagnet, feng2020scalable, Lv2020GraphBasedRO}, and natural language inference~\citep{kapanipathi2020infusing, wang2019improving}. 
% A typical KG-augmented (neural-symbolic) model either leverages the encoding of the grounded relational structures as additional input features~\citep{lin2019kagnet,feng2020scalable}, or models the relational connections in KG to propagate information among the entities (\textit{i.e.}, message passing)~\citep{wang2018ripplenet,wang2019aknowledge}. 
% By doing so, these methods successfully improve the performance on downstream tasks by bringing symbolic knowledge which is essential yet absent in the input as in commonsense reasoning tasks~\citep{talmor2018commonsenseqa}, or help to address data sparsity and cold start issues as in recommender systems~\citep{wang2018shine}.
% In addition to enhancing model performance, such symbolic knowledge, together with its learned (attention) weights, are used as explanations for the model predictions~\citep{feng2020scalable, lin2019kagnet, cao2019unifying, gao2019explainable}, providing ``insights" to practitioners for understanding the reasoning process.



%%% 2nd paragraph: 
% 1) should start the paragraph with "we question whether the symbolic structures from KG (together with the associated weights) necessarily indicate the model's predictions and enhance the performance." 
% 2） and then bring out the pilot study with these simple heuristics. The main focus should be on faithfulness of the explanation (we also will include human evaluation and those are direct proof; pls stress on that).
% 3) the performance drop is a secondary claim. Please follow the abstract narrative.

% Aaron
Despite the vast KG literature and increasing prevalence of NSKG models, the process in which NSKG models reason about KG information is still not well understood. When solving a reasoning task with a KG, a human might intuitively base their predictions on semantically faithful chains of entities and relations in the KG \citep{feng2020scalable, lin2019kagnet,Song2019ExplainableKG,gao2019explainable}. Meanwhile, it is assumed that NSKG models perform a similar reasoning process and that this process is responsible for the KG-associated performance gains. In this paper, we challenge this assumption and question whether existing NSKG models actually use KGs in a faithful manner. We study this question primarily by measuring model performance with respect to increasing amounts of KG perturbation. To perturb the KG, we propose several simple perturbation heuristics as well as a more powerful reinforcement learning (RL) based perturbation approach. Whereas the heuristic-based perturbations are generally agnostic to the model and downstream task, the RL-based perturbations are specifically tailored to both the model and the dataset of the given task. Surprisingly, we find that the KG can be extensively perturbed with little effect on model performance, thus yielding unfaithful explanations and raising doubts about the role of the KG in current NSKG models.


% Our pilot study applies simple heuristics to perturb all the edges and relations in the KG.
% % and see whether a well-trained KG-augmented model would have significant performance drop. 
% In some cases, despite a deceptive symbolic structure, which completely deviates from the original KG, we observe that existing models still manage to maintain their performance on downstream tasks. For cases where model performance has noticeable drops, our human evaluation on the model explanation shows that the perturbed structure does not provide faithful explanations. 


% Due to the increased usage of neuro-symbolic models for various tasks, it is of paramount importance  to analyze the structures  learned by these models. In this paper, we question whether the KG structures associated with the data instances provide faithful explanation for the model's predictions and information carried by these structures--\textit{i.e.}, relations and connections between entities--necessarily contribute to the performance improvement on the models.
% Through a series of experiments on diverse tasks and KG-augmented models, we show that one can manipulate the KG structures without significant impact on the performance of the model, yielding deceptive model explanation and raising doubts on what information from the KG are actually captured.
% %
% Our pilot study applies simple heuristics to perturb all the edges and relations in the KG.
% % and see whether a well-trained KG-augmented model would have significant performance drop. 
% In some cases, despite a deceptive symbolic structure, which completely deviates from the original KG, we observe that existing models still manage to maintain their performance on downstream tasks. For cases where model performance has noticeable drops, our human evaluation on the model explanation shows that the perturbed structure does not provide faithful explanations. 


% On other cases, however, we observe noticeable performance drop for the models, indicating that a more targeted perturbation is necessary.
%Using these heuristics we try to challenge the faithfulness of the interpretations generated by the models. We also perform a user study to show the unfaithful explanations generated for a prediction by the models. There are some models that have a drastic performance drop with simple heuristic perturbations.



%%% 3rd paragraph: We need a paragraph to talk about:
% 1）what is our proposed method for solving the remaining issue in previous paragraph, and thus motivate the RL policy learning. 
% 2) And briefly introduce the solution idea of the proposed method

%In our pilot studies we observe a drastic performance drop of a recent KG-augmented model, MHGRN~\citep{feng2020scalable} on the commonsense QA task. 
% \xiang{1. this paragraph needs expansion and polishing; 2. we need leading sentence to make transition from the prior paragraph --- to give motivation on why we need such learning-based approach.}
% For these cases, we question whether a more sophisticated policy can be applied to deceive such specific KG models and maintain the performance on downstream tasks with large perturbations. To this end, we propose a reinforcement learning (RL) based perturbation algorithm and show the existence of such policies. 


% The preliminary results indicate that KG can be easily manipulated and lost its benefit. It brings more worrisome scenario that KG is perturbed in a more systematic way so that even advanced KG-augmented models can be deceived by such a perturbed KG without noticeable performance drop. To show the feasibility of such perturbation policies, we conduct a more sophisticated study where we propose a reinforcement learning (RL) based perturbation algorithm. We leverage the Deep Q-network (DQN) to model the change of downstream task performance given specific perturbation actions, and restrict the agent's action space to ensure nearly maximal perturbation. In this way, the agent learns a perturbation policy with a dual objective of maximally perturbing the graph but maintaining the original accuracy. We show that the agent learns to identify which edges or relations in the KG to perturb while preserving the competitive performance of these KG-augmented models. %compared with non-KG baselines.
% Unlike the heuristic methods, the RL agent can be tailored to a certain KG-augmented model by making use of its performance change as the training signal, and thus yield a perturbed graph with less structural and semantic information and a better performance compared with heuristic methods. %manage to learn deceptive symbolic structures which enable it to perform better than non KG baselines. 
%Both studies indicate that KG is not being leveraged appropriately, and the interpretations generated by the models cannot be relied upon.



%%% 4th paragraph: 1) summary of our exps and findings; 2) discuss about the implications/insights we could give to the community.

% Aaron
Our contributions can be summarized as follows: \textbf{(1)} We introduce four KG perturbation heuristics, which entail different ways to reassign relation types and edge connections in the KG. \textbf{(2)} We propose two RL-based KG perturbation algorithms, which train a policy to reassign either relation types or edge connections, respectively, while maximizing the perturbed KG's semantic distance from original KG and the downstream performance. \textbf{(3)} Across two downstream tasks (commonsense QA, recommender systems), four datasets (CSQA, OBQA, Last.FM, MovieLens-20M), and four NSKG models (RN, MHGRN, KGCN, RippleNet), we demonstrate that NSKG models are largely able to maintain their original performance even when the KG has been significantly perturbed to the point that humans struggle to read or use it. To the best of our knowledge, this is the first work to analyze the effects of targeted KG perturbations on NSKG model performance.         


% \xiang{this paragraph needs more revision.}
% In summary, our main findings and contributions are as follows: (1) \textbf{Knowledge Graph Perturbation Framework:} 
% We study perturbations to the knowledge graph along two dimensions, \emph{semantically} by randomization of the relation types while holding the distribution of those types to be the same (and therefore controlling for the different factors), and \emph{structure-based perturbations} that changes the connections in the knowledge graph.
% (2) \textbf{RL-based Targeted Perturbation:} We demonstrate that on some tasks it is non-trivial to achieve our goal of perturbing a KG while maintaining downstream performance with simple perturbations. Therefore we present RL-based perturbation policy learning to maximally perturb the graph while trying to maintain the downstream performance.
% % summarize the main finding maybe?
% (3) We find via our experiments that even with a KG that is corrupted by a sizeable amount, we are able to maintain the downstream performance on most tasks. Through our different types of perturbations and human evaluation, we demonstrate how faithful are the explanations generated by  KG-augmented models and how much are the models sensitive to changes in the KG. 
% To the best of our knowledge this is the first work that deals with the analysis of graph augmented models using targeted perturbations. 


==> backup/backup_Nov15/2_background.tex <==
% !TEX root = main.tex

% \xiang{Need an illustrative figure in 2nd/3rd page for the problem setup and proposed approach @Mrigank.}

% \section{Deceiving KG-Augmented Models by Graph Perturbation}
\section{Problem Setting}\label{sec: problem_setting}
\vspace{-0.2cm}
% \xiang{I envision this section to given overview of our work by defining the problem and laying out some background context. Regarding this, in current writing we're missing: 

% 1) more formal problem definition (after introducing the necessary concepts and notations); should be in the first paragraph. @Mrigank, I recall that you had some formulation in your slides earlier.

% 2) in current writing there is no mention of ``explanation" or ``interpretability" by the KG structures used in these models. This is a critical point and should be well introduced, with notations.

% 3) an overview of the rest of the paper after this section (should be a short paragraph at the end of this section.)}

% Aaron
Our goal is to investigate: \textbf{(A)} whether NSKG models faithfully use KGs for making predictions and \textbf{(B)} whether KGs facilitate sensible explanations of model predictions. For \textbf{(A)}, across various perturbation techniques, we measure model performance as a function of the number of KG perturbations applied. If a KG has been perturbed to the point where even humans have difficulty understanding it, then a faithful NSGK model should not be able to use this perturbed KG to achieve high performance on downstream tasks. For \textbf{(B)}, we ask human subjects to rate original and perturbed KGs with respect to readability and usefulness for solving downstream tasks. If a KG receives higher ratings, then it is more likely to provide sensible explanations.      

\textbf{Notation~} Let $\mathcal{F}_{\theta}$ be an NSKG model, and let $(X_{train}, X_{dev}, X_{test})$ be a dataset for some downstream task. We denote a KG as $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$, where $\mathcal{E}$ is the set of entities (nodes), $\mathcal{R}$ is the set of relation types, and $\mathcal{T}=\{(e_1,r,e_2) \hspace{1.5mm} | \hspace{1.5mm} e_1,e_2 \hspace{-0.5mm} \in \hspace{-0.5mm} \mathcal{E}, \hspace{1mm} r \hspace{-0.5mm} \in \hspace{-0.5mm} \mathcal{R}\}$ is the set of facts (edges) composed from existing entities and relations. Let $\mathcal{G}^{'}=(\mathcal{E},\mathcal{R},\mathcal{T}^{'}), \hspace{1mm} \mathcal{T}^{'} \hspace{-1mm} \neq\mathcal{T}$ be the KG obtained after perturbing the edges in $\mathcal{G}$. 

Let $f(\mathcal{G},\mathcal{G}^{'})$ be a function that measures the semantic distance between $\mathcal{G}$ and $\mathcal{G}^{'}$. Let $g(\mathcal{G})$ be the downstream performance when evaluating $\mathcal{F}_{\theta}$ on $X_{test}$ and $\mathcal{G}$. Let $s_\mathcal{G}$ be an edge scoring function, such that $s_{\mathcal{G}}(e_1, r, e_2)$ measures how likely edge $(e_1, r, e_2)$ is to exist in $s_\mathcal{G}$. Furthermore, let $\oplus$ denote the concatenation operation, and let $\mathcal{N}_L(e)$ denote the set of $L$-hop neighbors for entity $e\in\mathcal{E}$.

\textbf{High-Level Procedure~} First, we train $\mathcal{F}_{\theta}$ on $X_{train}$ and $\mathcal{G}$, then evaluate $\mathcal{F}_{\theta}$ on $X_{test}$ and $\mathcal{G}$ to get the original performance $g(\mathcal{G})$. Second, we freeze $\mathcal{F}_{\theta}$, then perturb $\mathcal{G}$ to obtain $\mathcal{G}^{'}$. Third, we evaluate $\mathcal{F}_{\theta}$ on $X_{test}$ and $\mathcal{G}^{'}$ to get the perturbation performance $g(\mathcal{G}^{'})$. Therefore, our perturbation objective can be formalized as: 
\vspace{-2mm}
\begin{equation}
\mathcal{G}^{*}=\argmax_{\mathcal{G}^{'}} \hspace{1mm} f(\mathcal{G},\mathcal{G}^{'}) + g(\mathcal{G}^{'}).
\end{equation}
\vspace{-3mm}

In this paper, we consider two downstream tasks: commonsense QA and recommender systems. Each task has its own specific settings and models, which are described in the rest of this section.

%%%
% We aim to investigate whether KGs are being leveraged appropriately by the KG-augmented models. A KG is denoted as $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$, where $\mathcal{E}$ and $\mathcal{R}$ are the entity set and relation set respectively. It consists of a set of relational edges $\mathcal{T}=\{(h,r,t)|h,t\in\mathcal{E},r\in\mathcal{R}\}$. Let $\mathcal{N}_L(e)$ denote the set of L-hop neighbors for the entity $e\in\mathcal{E}$. Let $\mathcal{G}^{'}=(\mathcal{E},\mathcal{R},\mathcal{T}^{'}),\mathcal{T}^{'}\neq\mathcal{T}$ be a perturbed version of $\mathcal{G}$.
% We define a KG evaluation metric function $f(\mathcal{G},\mathcal{G}^{'})$ which quantifies how much relational information in the KG is \textit{preserved} after perturbation. We further define a performance measurement function $g(\mathcal{G},\mathcal{G}^{'})$ which quantifies the difference in a model's performance, \textit{e.g.}, accuracy on the downstream task. 
% Our goal (\textit{i.e.}, deceiving KG-augmented models) is to identify a \textit{perturbed} KG, $\mathcal{G}^{'}$, which maximally deviates from the original KG, $\mathcal{G}$; while minimally affecting the downstream performance of the KG-augmented model. This perturbation can be formalized into the following objective. 
% \vspace{-0.2cm}
% \begin{equation}
% \mathcal{G}^{*}=\argmin_{\mathcal{G}^{'}} f(\mathcal{G},\mathcal{G}^{'})+g(\mathcal{G},\mathcal{G}^{'}).
% \end{equation}
% In specific, the KG-augmented model is well-trained on $\mathcal{G}$ to get the original performance and fixed. Later the model is tested on $\mathcal{G}^{'}$ to get its performance after perturbation.
%We aim to investigate whether KGs are being leveraged appropriately by the KG-augmented models. 
%We conduct such an investigation through perturbing the underlying KGs of these models to a large extent while still preserving their competitive performance. Formally, a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$, where $\mathcal{E}$ and $\mathcal{R}$ are the entity set and relation set respectively, consists of a set of relational edges $\mathcal{T}=\{(h,r,t)|h,t\in\mathcal{E},r\in\mathcal{R}\}$. We perturb the \textbf{semantic} of KG by revising the relation type (\textsection\ref{}) as well as the graph \textbf{structure} by deleting/rerouting the edges (\textsection\ref{}) for a subset of $\mathcal{T}$  under the guidance of our proposed RL algorithm (\textsection\ref{}). By doing so, we cast doubt on whether the KGs truly contribute to the improvement brought by the models in a way we expect them to and thus raise the researchers' awareness in this field that KGs are not fully utilized. 
% In this work, we look into two different tasks across different domains, \textit{e.g.}, commonsense question answering (QA) and recommender system, as introduced in the rest of this section. %since KGs are shown to be helpful empirically for both tasks by recent works~\cite{}. For each task, we introduce respectively their problem setting and how KGs are leveraged to solve the tasks in the following.
%as well how knowledge is encoded by different kinds of graph encoder respectively in \textsection\ref{sec:task}. We then depict two typical graph encoders that the KG-augmented models adopt to encode the knowledge from a KG in \textsection\ref{}.

% \textbf{Commonsense Question Answering.}
\textbf{Commonsense QA~}
% \label{sec:csqa}
% \vspace{-0.3cm}
% Aaron
Given a question $q$ and a set of $k$ possible answers $\mathcal{A} = \{a_{1}, ... , a_{k}\}$, the task is to predict a plausibility score for each answer, such that the highest score is predicted for the correct answer. In commonsense QA, the questions are designed to require commonsense knowledge which is typically unstated in natural language, but more likely to be found in KGs. 

Given KG $\mathcal{G}$, let $\mathcal{E}_{(q,a)}\subset\mathcal{E}$ be the set of all entities mentioned in the text sequence $q \oplus a$, and let $\mathcal{T}_{(q,a)} \subset \mathcal{T}$ be the set of all edges connecting the entities in $\mathcal{E}_{(q,a)}$. Following \citet{lin2019kagnet} and \citet{feng2020scalable}, for each question-answer pair $(q, a)$, we first use off-the-shelf string matching tools to extract $\mathcal{E}_{(q,a)}$ from $q \oplus a$. Next, from $\mathcal{G}$, we construct a subgraph $\mathcal{G}_{(q,a)}$, which consists of $\mathcal{E}_{(q,a)}$ and $\mathcal{T}_{(q,a)}$.

Recall that the NSKG model is denoted as $\mathcal{F}_{\theta}$. For this task, let $\mathcal{F}_{\phi}^{text}$ be a text encoder, $\mathcal{F}_{\psi}^{graph}$ be a graph encoder, and $\mathcal{F}_{\xi}^{cls}$ be a classifier, where $\phi, \psi, \xi \subset \theta$. We then compute a text embedding $\mathbf{h}_{text} = \mathcal{F}_{\phi}^{text}(q \oplus a)$ and a graph embedding $\mathbf{h}_{graph} = \mathcal{F}_{\phi}^{graph}(\mathcal{G}_{(q,a)})$. After that, we compute the score for $(q,a)$ as $y_{(q,a)} = \mathcal{F}_{\xi}^{cls}(\mathbf{h}_{text} \oplus \mathbf{h}_{graph})$. Finally, we select the highest scoring answer: $a^{*} = \argmax_{a \in A} \hspace{1mm} y_{(q,a)}$ 

Since the graph encoder $\mathcal{F}_{\psi}^{graph}$ plays the critical role of leveraging information from the KG, significant research effort has been devoted to designing better graph encoders. Two common types of graph encoders are graph neural networks (GNNs) and path-based models. GNNs iteratively update each node's embedding by aggregating its neighbor nodes' embeddings, then obtain the graph embedding by pooling the final node embeddings ~\citep{kipf2016semi, schlichtkrull2018modeling}. Path-based models treat the graph as a set of paths, encode each path separately, then obtain the graph embedding by aggregating the path embeddings ~\citep{lin2019kagnet, santoro2017simple}. More recently, MHGRN ~\citep{feng2020scalable} was proposed as a hybrid of GNNs and path-based models, achieving better interpretability, scalability, and performance on commonsense QA benchmarks. In these graph encoders, the aggregation weights computed for $\mathcal{G}_{(q,a)}$ can serve as an explanation for the model prediction.


%\textbf{Problem Setting}. We focus on multi-choice commonsense QA which is the general format for most of the benchmarks in this field. Given a question $q$, a system is required to select one of the choices $\{a\}$ as the answer. The task is on-purposely designed to omit the key background knowledge that leads to the answer, so as to test the system for its understanding of commonsense. 
% Given a question $q$ and a set of choices $\mathcal{C}$, the task requires a system to select one of the choices $a\in\mathcal{A}$ as the answer.
% To tackle the task, the KG-augmented QA systems such as KagNet~\citep{lin2019kagnet} and MHGRN~\citep{feng2020scalable}
% %In response, systems solving these tasks usually resort to some external KG for obtaining knowledge necessary for answering the question. They 
% first extract the set of entities $\mathcal{E}_{(q,a)}\subset\mathcal{E}$ mentioned in the pair of $(q,a)$ with existing entity recognition tools and later construct a sub-graph $\mathcal{G}_{(q,a)}$ containing $\mathcal{E}_{(q,a)}$ and their multi-hop relations in the KG. Then the system encodes the $(q,a)$ pair to a context embedding $\mathbf{c}$ and encodes $\mathcal{G}_{(q,a)}$ to a knowledge embedding $\mathbf{k}$. Finally, both $\mathbf{c}$ and $\mathbf{k}$ are concatenated for calculating the plausibility score. 
% %a general QA framework consisting one context encoder and one graph encoder is adopted to solve the task. The context encoder, which is usually a pre-trained LM~\cite{}, takes as input the QA pair $(q,a)$ and outputs a context embedding $\mathbf{c}$. The graph encoder takes as input the sub-graph and outputs the knowledge embedding $\mathbf{k}$. Both output embeddings are concatenated together as the input to the final classifier that gives a score for a choice: $f(q,a)=\mathbf{w}\cdot[\mathbf{c};\mathbf{k}]+b$.
% The choice with the highest score is selected as the answer.
% %\textbf{Graph Encoders for QA-KG}. 
% Two types of graph encoders are generally adopted to encode $\mathcal{G}_{(q,a)}$ to $\mathbf{k}$ as described below. 

% (1) Graph Neural Networks ~\citep{kipf2016semi,schlichtkrull2018modeling} firstly represent each node by its feature embedding $\{\mathbf{h}^0_i\},i\in\mathcal{G}_{(q,a)}$ and then iteratively update a node's representation  by aggregating its neighbors' embedding, i.e., $\mathbf{h}^l_i=\text{Aggregation}(\{\mathbf{h}^{l-1}_j|j\in \mathcal{N}_1(i)\})$. Finally, a pooling over all the node embeddings is used as the graph representation: $\mathbf{k}=\text{Pooling}(\{\mathbf{h}^{L}_i\})$ with $L$ indicating each node receives information from its neighbors up to $L$ hops. 

% (2) Path-Based Models~\citep{lin2019kagnet,santoro2017simple} treat an input graph as a set of relational paths $\mathcal{P}$ connecting the entities. Then each path $p_i\in\mathcal{P}$ is encoded as an embedding $\mathbf{p}_i$  and further aggregated to obtain the knowledge embedding: $\mathbf{k}=\text{Aggregation}(\{\mathbf{p}_i\})$.

% In both graph encoders, the subgraph $\mathcal{G}_{(q,a)}$ together with the aggregation weights serve as the explanation for the prediction.

\textbf{Recommender Systems~} 
% \vspace{-0.3cm}
%\textbf{Problem Setting}. 
% Aaron
We consider a set of users $\mathcal{U}=\{u_1,u_2,...,u_M\}$, a set of items $\mathcal{V}=\{v_1,v_2,...,v_N\}$, and a user-item interaction matrix $\mathbf{Y}\in\mathcal{R}^{M\times N}$. If user $u$ has engaged with item $v$ before, then $y_{uv}=1$ in the user-item interaction matrix; otherwise, $y_{uv}=0$. Additionally, we consider a KG $\mathcal{G}$, in which $\mathcal{R}$ is the set of relation types in $\mathcal{G}$. In $\mathcal{G}$, nodes are items $v \in \mathcal{V}$, and edges are facts of the form $(v_{i}, r, v_{j})$, where $r \in \mathcal{R}$ is a relation. For the zero entries in $\mathbf{Y}$ (i.e., $y_{uv}=0$), our task is to predict a compatibility score for user-item pair $(u, v)$, indicating how likely user $u$ is to want to engage with item $v$. We represent each user $u$, item $v$, and relation $r$ as embeddings $\mathbf{u}$, $\mathbf{v}$, and $\mathbf{r}$, respectively. Given a pair $(u, v)$, its compatibility score is computed as $\langle \mathbf{u}, \mathbf{v} \rangle$, the inner product between $\mathbf{u}$ and $\mathbf{v}$. 

Two prominent examples of NSKG recommender systems are KGCN ~\citep{wang2019knowledge} and RippleNet ~\citep{wang2018ripplenet}. In KGCN, we first retrieve $\mathbf{u}$ and $\mathbf{v}$ from $\mathcal{G}$'s embedding table, which is learned. Next, a neural network iteratively updates $\mathbf{v}$ by aggregating its subgraph of $L$-hop neighbor embeddings, the corresponding relation embeddings, and $\mathbf{u}$. After $\mathbf{v}$ is done updating, we compute $\langle \mathbf{u}, \mathbf{v} \rangle$. In RippleNet, we retrieve $\mathbf{v}$ from $\mathcal{G}$'s embedding table, which is learned, and set the items $u$ has interacted with as seed nodes. Next, a neural network computes $\mathbf{u}$ via iterative aggregating its subgraph of seed node embeddings, their $L$-hop neighbor embeddings, and the corresponding relation embeddings. After obtaining $\mathbf{u}$, we again compute $\langle \mathbf{u}, \mathbf{v} \rangle$. In both KGCN and RippleNet, the aggregation weights from the subgraph can be used to explain the model prediction.           

% In this task, we consider a set of users $\mathcal{U}=\{u_1,u_2,...,u_M\}$ and a set of items $\mathcal{V}=\{v_1,v_2,...,v_N\}$, as well as their interaction matrix $\mathbf{Y}\in\mathcal{R}^{M\times N}$. An observed interaction ($y_{uv}=1$) indicates that the user $u$ engages with the item $v$ before while
% the task is to predict the unobserved interaction ($y_{uv}=0$).
% The KG-augmented recommender systems assume there exists 
% an item KG which provides bountiful relational connections between the items. They further represent each user and item as embeddings $\mathbf{u}$ and $\mathbf{v}$ and then use their interaction, e.g., inner product for recommending $v$ to $u$. Below we introduce two recent works we investigate in this paper which differ in how they leverage the item KG and represent the users and items.

%\textbf{KG-Augmented Recommendation System}.Recent work on Knowledge Graph augmented Recommendation Systems can be classified into 3 categories namely Embedding based, Path based and Hybrid Models. Embedding based models \citep{huang2018improving,wang2018dkn, wang2019multi} try to learn entity embeddings using a knowledge graph embedding (KGE) techniques and then use these learned embeddings for recommendation. Path based models \citep{hu2018leveraging,yu2014personalized,zhao2018learning} explore the connectivity between different items that can be leveraged for the recommendation task. Embedding based methods focus heavily on the relation types between two entities. In this way using path based models seems a more natural approach for recommendation but these models include finding meta paths/graphs which are not easy to tune in practice. Hybrid models \citep{wang2019knowledge, wang2018ripplenet} try to combine best of both worlds by learning embeddings of an entity based on its local neighbourhood and using these embeddings for the recommendation task. The two well known hybrid models for recommendation systems are described below.


% KGCN~\citep{wang2019knowledge} represents an item as each aggregation over its neighbors in the KG, i.e., $\mathbf{v}=\text{Aggregation}_u(\{\mathbf{v}^{'}|v^{'}\in\mathcal{N}_1(v)\})$, where the aggregation weights are personalized for $u$. This aggregation is repeated $L$ times to obtain information from $L$-hops neighbors (similar to GNN). The user embedding is initialized randomly and learned during training.
%tries to learn a user personalized embedding for the neighbourhood N(v) of a given entity v by weighting the features of the neighbouhood entities with learnable user personalized weights i.e $\mathbf{v_{N(v)}^u} = \sum_{e \in N(v)}^{}\pi_{r_{v,e}}^u\mathbf{e}$ where $r_{v,e}$ is the label of the edge connecting v and e and $\mathbf{e}$ is the embedding for entity e. Then this neighbourhood embedding is aggregated with the the embedding of v and passed thorough non linearities to get a personalized entity embedding $\mathbf{v^u}$ and then use this along with the user embedding $\mathbf{u}$ to get a score for a given user-entity pair.
% In contrast, RippleNet~\citep{wang2018ripplenet} represents each user $u$ as the aggregation over the $L$-hops neighbors of the items $\mathcal{V}_u$ which $u$ has been interacted with before, i.e., $\mathbf{u}=\text{Aggregation}(\{\mathbf{v}|v\in\mathcal{N}_L(v^{'}),\forall v^{'}\in\mathcal{V}_u\})$. The item embedding is initialized randomly and learned during training. In both KGCN and RippleNet, the aggregation weights on the items' neighbors are used to explain the recommendation results.
%tries to learn user embeddings using his/her preferred items. For a given user u, they construct a ripple set of triples that are k hop away from entities in which u is interested. Then they pass messages among the triples in this ripple set and set the embedding \textbf{u} of user u to be the aggregation of these messages. For a user-entity pair they use this learned user embeddings and the entity embeddings to estimate the probability that the given user engages in the given item.  

% \xiang{Need a short paragraph as an overview of the rest of the paper after this section}
% In the rest of the paper, we will first present the pilot study that motivates the work, and then describe the targeted RL perturbation policy that we propose for our analysis. Finally we detail our experimental setup and show our results and analysis that support the claim of the paper.


\begin{figure}[t]
%{0.57\textwidth}
    \centering
\vspace{-0.4cm}
    \includegraphics[width=1.0\textwidth]{figures/pert_kg.pdf}
    %\vspace{-0.4cm}
    \caption{\textbf{KG Perturbation Framework.} First, we perturb relations/edges in a KG using either heuristics or an RL policy. After perturbation, the perturbed KG is provided to a pre-trained NSKG model as context for performing some downstream task. Finally, we evaluate the perturbed KG's distance from the original KG, the model's downstream performance, and the faithfulness of the model's explanations for its predictions.}
    \label{fig:pert_framework}
\vspace{-0.4cm}
\end{figure}

% \subsection{Graph Encoders}
% Recently there has been a boom in the research of Graph Representation Learning Models \citep{velivckovic2018graph, hamilton2017representation, hamilton2017inductive,you2019position} but a very few of them can be adapted successfully to heterogeneous graphs such as Knowledge Graphs. To this end we introduce Graph Networks \citep{battaglia2018relational} and Relation Networks \citep{santoro2017simple} which aim to capture the relational information present in Knowledge Graphs.
% \begin{itemize}
%     \item Path Based Models: 
%     \item Message Passing based Models: Details about Graph Networks
% \end{itemize}
% \subsection{Deep Q Networks}
% In this paper we try to leverage Reinforcement Learning to come up with a targeted perturbation policy. We use Deep Q Networks (DQN) to learn the perturbation policy. DQN and its variants have been shown very powerful in playing games, where the policy of agents is trained through the feedback reward from the environment. 
% In this work, we view our perturbation policy as agent, and the downstream task performance as environment. Every time we use our policy to perturb KG for a fixed steps, we will get reward from the environment reflecting how well we maintain the downstream task performance. In this way, we have our policy trained and the DQN will learn a good policy suiting for our purpose.

% In a typical DQN, at each step we will have to feed the embeddings of state to get the approximated Q function. However, in our work, if we directly use a GNN-based model to embed the current KG as state, it will conflict with the purpose of our work, which is to examine the effect of the GNN-based model of KG. Therefore, we alternatively apply a LSTM to represent the state as hidden state, and at the same time form the DQN. The initialized embedding of LSTM is randomized and trainable. At each time step, the LSTM cell takes in the hidden state vector for the current state and the current action we choose, and then it outputs the approximated Q function and the hidden state vector for the next state.


% \begin{itemize}
%     \item Commonsense Question Answering: 
%     \item Recommendation Systems: 
% \end{itemize}

==> backup/backup_Nov15/3_heuristic.tex <==
% !TEX root = main.tex

\vspace{-0.1cm}
\section{Heuristic-Based KG Perturbation}\label{sec: pilotexpts}
\vspace{-0.2cm}
We aim to study how a KG's \textit{semantics} (i.e., semantic meaning of relations between entities) and \textit{connectivity} (i.e., structure of connections between entities) contribute to the downstream performance of NSKG models. To achieve this, we can measure a model's downstream performance in response to perturbing the KG in various ways. While the KG's semantics can be perturbed by altering its relation types, the KG's connectivity can be perturbed by changing its edge connections. To this end, we design four graph perturbation heuristics as described below, each involving perturbation of relation types, edge connections, or both.
%To perturb the KG, $\mathcal{G}$, we first consider four heuristics, each involving random reassignment of relation types or edge connections. These heuristics are described below:

\textbf{Relation Swapping (RS) \hspace{1mm}}
For RS, we randomly select two edges, $\{(e_1, r_1, e_2), (e_1', r_2, e_2')\}$, from $\mathcal{T}$ and swap their relations, yielding $\{(e_1, r_2, e_2), (e_1', r_1, e_2')\}$. It is possible for the two edges to share entities, such that $e_1=e_1'$, $e_1=e_2'$, $e_2=e_1'$, and/or $e_2=e_2'$. This heuristic changes the semantics of the two edges, while leaving the KG's connectivity structure unchanged.

\textbf{Relation Replacement (RR) \hspace{1mm}}
Let $s_\mathcal{G}$ be an edge scoring function trained on $\mathcal{G}$, such that $s_{\mathcal{G}}(e_1, r, e_2)$ measures how likely edge $(e_1, r, e_2)$ is valid. For RR, we randomly select an edge $(e_1, r_1, e_2)$ in $\mathcal{T}$ and replace its relation with relation $r_2$, where $r_2=\argminB_{r \in \mathcal{R}}{s_\mathcal{G}(e_1,r,e_2)}$. Like RS, this heuristic changes the KG's relation distribution, but not its structure. Note that, prior to perturbing $\mathcal{G}$, we assume $s_\mathcal{G}$ has been trained on the link prediction task for $\mathcal{G}$. More details about calculating $s_\mathcal{G}$ can be found in Section~\ref{sec:exp}.  
% used in the paper are \citep{li-etal-2016-commonsense} for Question Answering task and \citep{yang2015embedding} for recommendation tasks. 

\textbf{Edge Rewiring (ER) \hspace{1mm}} 
For ER, we first randomly select an edge $(e_1,r,e_2)$ in $\mathcal{T}$. Let $\mathcal{E}' \subset \mathcal{E}$ be the set of entities that have an edge with $r$ but are not $1$-hop neighbors of $h$. After that, we randomly select an entity $e_2'$ from $\mathcal{E}'$, remove edge $(e_1,r,e_2)$ from $\mathcal{T}$, and add edge $(e_1,r,e_2')$ to $\mathcal{T}$. Unlike RS and RS, this heuristic alters the KG's connectivity structure, while keeping its relation distribution the same. 

\textbf{Edge Deletion (ED) \hspace{1mm}} 
For ED, we randomly select an edge in $\mathcal{T}$ and remove it from $\mathcal{T}$. This heuristic changes both the KG's connectivity structure and relation distribution.

%\mrigank{Using heuristics we want to perturb two different aspects of a KG namely the relation distribution and the edge connectivity of the KG. We select these 4 heuristics as they capture all the 4 possible scenarios of perturbation that we wish to inspect.}
%\aaron{Maybe add an explanation for why these heuristics were chosen and how we might expect them to affect downstream performance.}

% Note that the ATS metric will fail to recognize these perturbations to the KG by design, since after deletion the remaining edges are still valid triples.

==> backup/backup_Nov15/4_rl.tex <==
% !TEX root = main.tex

\vspace{-0.1cm}
% \section{Policy Learning for Targeted KG Perturbation}
\section{RL-Based KG Perturbation}
\vspace{-0.1cm}

Here, we introduce our RL-based KG perturbation approach. Given a KG, $\mathcal{G}$, this approach involves training a policy to output a perturbed KG, $\mathcal{G}'$, such that both original-to-perturbed semantic distance, $f(\mathcal{G},\mathcal{G}^{'})$, and downstream performance, $g(\mathcal{G}^{'})$, are maximized. We consider two variants of this approach: \textbf{RL-Based Relation Replacement (RL-RR)} and \textbf{RL-Based Edge Rewiring (RL-ER)}. RL-RR and RL-ER have the same basic perturbation mechanisms as the RR and ER heuristics do, respectively, but are also able to adapt their perturbations to the given downstream dataset. Thus, we expect RL-RR and RL-ER to output perturbed KGs that yield higher downstream performance than their heuristic-based counterparts.

The perturbation procedure is modeled as a finite horizon Markov decision process $(S, A, P, R, \gamma)$, where $S$ is the state space, $A$ is the action space, $P$ is the transition probability, $R$ is the reward function, and $\gamma$ is the discount factor. In the rest of this section, we introduce a metric for measuring semantic distance (i.e., $f$), define $(S, A, R)$, and explain how RL-RR and RL-ER are implemented.


% \xiang{Need update to only talk about the relation perturbation policy and reward design.}

% In this section we introduce our targeted perturbation policy which learns to maximally perturb the graph while maintaining the performance on the downstream task. The policy can be trained to perform either relation perturbations i.e. changing the relations of edges in the knowledge graph, or edge perturbations i.e. changing the target node of an edge in the graph.
% %Another is structure perturbation, i.e., replacing the edges. %We try to perturb the semantics and the structure of the graph separately to see the effect of different attributes of the graph on the downstream tasks.
% To achieve this goal, we adopt Deep Q-networks (DQN)~\citep{mnih2015human}, a deep RL algorithm to learn the target policy. We model the perturbation procedure as a Finite Horizon Markov Decision Process $(S, A, P, R, \gamma)$, where $S$ is the state space,  $A$ is the action space, $P$ is the transition probability, $R$ is the reward function and $\gamma$ is the discount factor. With this setting, DQN aims at learning an approximated Q function $Q(s_t, a_t) $ for state $s_t$ and action $a_t$ at step $t$. The detailed definitions are as follows. 

\begin{figure}
%{0.5\textwidth}
    %\vspace{-0.6cm}
    \centering
\includegraphics[width=1.0\textwidth]{figures/dqn.pdf}
%\vspace{-0.5cm}
    \caption{\textbf{RL-Based KG Perturbation.} (Left) To obtain a computationally feasible action space for each RL perturbation method, we decouple each action into a sequence of three subactions. (Right) At each time step, a subaction sequence is predicted according to the given RL perturbation method (RL-RR or RL-ER). The schematic depicts the LSTM-based DQN architecture used for RL-RR and RL-ER.}
    \label{fig:model_figure}
    \vspace{-0.2cm}
\end{figure}


\textbf{Aggregated Triple Score (ATS) \hspace{1mm}}
To measure pairwise semantic distance between KGs, we propose the Aggregated Triple Score (ATS). Recall that $s_\mathcal{G}$ is an edge (triple) scoring function, such that $s_{\mathcal{G}}(e_1, r, e_2)$ measures how likely edge $(e_1, r, e_2)$ is valid. We assume $s_\mathcal{G}$ has been trained on the link prediction task for $\mathcal{G}$. Hence, ATS is defined as $f^{ATS}(\mathcal{G},\mathcal{G}^{'}) = \frac{1}{|\mathcal{T}^{'}|}\sum_{(e_1,r,e_2)\in\mathcal{T}^{'}}s_\mathcal{G}(e_1,r,e_2)$, which denotes the mean $s_\mathcal{G}$ score across all edges in $\mathcal{G'}$. Intuitively, if a high percentage of edges in $\mathcal{G'}$ are also likely to exist in $\mathcal{G}$ (i.e., high ATS), then we say that $\mathcal{G'}$ has high semantic similarity with $\mathcal{G}$. More details about $s_\mathcal{G}$ can be found in Section \ref{sec:exp}. 
% The KG scoring functions used in the paper are \citep{li-etal-2016-commonsense} for Question Answering task and \citep{yang2015embedding} for recommendation tasks. 
%This validation score is derived from the Knowledge Base Completion model mentioned above. 
%trained on Conceptnet. We train the embedding based Knowledge base completion architecture as specified in \citep{li-etal-2016-commonsense} on the Knowledge Graph. Given a triple $ t = (e1,r,e2)$, this model outputs the score $f(t)$ of the triple. Larger the score of the triple, more semantically correct the triple should be. 

\textbf{State Space \hspace{1mm}}
The state space $S$ consists of all possible perturbed configurations of $\mathcal{G}$, with respect to the given perturbation algorithm. For RL-RR, $\mathcal{G}$'s connectivity structure does not change, so the corresponding state space is all graphs with the same structure as $\mathcal{G}$. For RL-ER, $\mathcal{G}$'s connectivity structure does change, while its relation distribution stays constant, so the corresponding state space is all graphs with the same relation distribution as $\mathcal{G}$. 

\textbf{Action Space \hspace{1mm}}
For RL-RR and RL-ER, the action space consists of all possible relation replacements and edge rewirings, respectively. Since having such a large action space poses computational issues, we reduce the action space by decoupling each action into a sequence of three subactions and operate instead in this smaller subaction space. Therefore, an action at time step $t$ would be denoted as \begin{small}$a_t = (a_t^{(0)}, a_t^{(1)}, a_t^{(2)})$\end{small}. Additionally, to make the policy choose low-ATS perturbations, we further restrict the \begin{small}$a_t^{(2)}$\end{small} subaction space to be the $K$ actions resulting in the lowest ATS.

For RL-RR, \begin{small}$a_t^{(0)}$\end{small} is sampling an entity $e_{1} \in \mathcal{E}$; \begin{small}$a_t^{(1)}$\end{small} is selecting an edge $(e_{1}, r, e_{2}) \in \mathcal{T}$; and \begin{small}$a_t^{(2)}$\end{small} is selecting a relation $r' \in \mathcal{R}$ to replace $r$ in $(e_{1}, r, e_{2})$. After \begin{small}$a_t^{(2)}$\end{small}, we complete \begin{small}$a_t$\end{small} by deleting \begin{small}$(e_{1}, r, e_{2})$\end{small} from $\mathcal{T}$ and adding \begin{small}$(e_{1}, r', e_{2})$\end{small} to $\mathcal{T}$. 
For RL-ER, \begin{small}$a_t^{(0)}$\end{small} is sampling an entity $e_{1} \in \mathcal{E}$; \begin{small}$a_t^{(1)}$\end{small} is selecting an edge $(e_{1}, r, e_{2}) \in \mathcal{T}$; and \begin{small}$a_t^{(2)}$\end{small} is selecting an entity $e_{2}' \in \mathcal{N}_1(e_{1})$, which is a $1$-hop neighbor of $e_{1}$. After \begin{small}$a_t^{(2)}$\end{small}, we complete \begin{small}$a_t$\end{small} by deleting \begin{small}$(e_{1}, r, e_{2})$\end{small} from $\mathcal{T}$ and adding \begin{small}$(e_{1}, r, e_{2}')$\end{small} to $\mathcal{T}$.

%For semantic perturbation, the action $a_t$ is to choose a triple from KG and substitute its relation type with another one. We can assign \begin{small}$a_t^{(0)}$\end{small} as the head entity, \begin{small}$a_t^{(1)}$\end{small} as its neighbour and finally \begin{small}$a_t^{(2)}$\end{small} as the relation type that substitutes the given relation.
%For structure perturbation, the action can also be decomposed to choosing a head entity, its neighbour and another tail entity. So the edge between the head and its neighbour is transferred to the tail entity.



% \textbf{Actions. }
% For both perturbations, the action space is very large and impractical to model. Thus to shrink the action space, we decompose an action $a_t$ into three subactions $a_t^{(0)}, a_t^{(1)}, a_t^{(2)}$, and the action space $A$ is decomposed into 
% \begin{small}$A= A_0\times_{a_0} A_1 \times_{(a_0,a_1)} A_2$\end{small}.
% For semantic perturbation, the action $a_t$ is to choose a triple from KG and substitute its relation type with another one. It can be decomposed to, first choosing a head entity ($a_t^{(0)}\in A_0=\mathcal{E}$), then a tail entity $a_t^{(1)}\in A_1(a_0)=\text{Neighbor}(a_0)$, and finally the relation type to substitute $a_t^{(2)}\in A_2=\mathcal{R}$.
% For edge perturbation, the action can also be decomposed to choosing a head entity ($a_t^{(0)}\in A_0=\mathcal{E}$), then a tail entity $a_t^{(1)}\in A_1(a_0)=\text{Neighbor}(a_0)$, and finally another tail entity for substitute $a_t^{(2)}\in A_2=\mathcal{E}$.

% In this way, we've unified the two types of perturbations in one framework. To accommodate the actions, we also decompose the DQN into 2 sub DQNs {$Q_1, Q_2$}. Note we choose $a_t^{(0)}$ randomly at each steps without DQN, because we are going to perturb a large percentage of the graph and nearly all actions in A_0 will be chosen, and thus the choice of $a_t^{(0)}$ is not decisive.

\textbf{Reward Function \hspace{1mm}}
The reward function encourages the policy to maximize downstream performance. This optimization of downstream performance is the key difference between the heuristic-based perturbations and the RL-based perturbations. For the commonsense QA task, we implement this by minimizing the KL divergence between the predicted answer distribution and the true answer distribution. For the recommender system task, we directly use dev AUC as the reward.
% The reward may be at very small scale, so we record the average of the absolute value of rewards and scale it to a pre-set value.

% \textbf{Reward.}
% The reward is designed to reflect the change of downstream task performance. 
% For QA, the straightforward design is to use the change of test set accuracy as rewards. However, the accuracy change is discrete and is not aware of probability drop, e.g., from 0.9 to 0.5 as long as the correct answer has the highest predicted probability. Therefore, we adopt KL-divergence between predicted answer distribution and the uniform wrong distribution as the extent of the predicted distribution to be wrong, and use the drop of it as reward. $Reward=\sum_{(q,a)} Reward(q,a)$, where $
%     Reward(q,a)=- \Delta (D_{KL}(p_{predict}||p_{wrong}))\text{  ,  }  p_{wrong}(a)=\begin{cases}0, &a \text{ is correct} \cr \frac{1}{num\_answers-1} , & a \text{ is wrong} \end{cases} $
% The reward may be at very small scale, so we record the average of the absolute value of rewards and scale it to a pre-set value.

% While trying to preserve the downstream task performance, we also need to ensure we are perturbing KG to a large scale by dropping validation score dramatically. Such multi-task problem is hard to solve if we simply integrate the two tasks into rewards, as it's hard to decide the weight of each task. Therefore, we restrict the action space $A^\prime_2$ to the K actions with lowest validation scores in the original action space $A_2$. In this way we can ensure that the validation score drops dramatically.


% \begin{figure}[H] 
% \centering 
% \includegraphics[width=0.5\textwidth]{figures/model_arch.JPG} 
% \caption{Model Architecture \xiang{@Hansen, pls update this figure and beautify it more.}} 
% \label{model_figure} 
% \end{figure}

% \begin{figure}
%  \hfill\begin{minipage}{.5\textwidth}\centering
%   \includegraphics[width=0.7\textwidth]{figures/model_arch.JPG} 
%   \caption{\texttt{minipage}}
%  \end{minipage}
% \end{figure}
% \begin{tabular}{cc}
% \raisebox{.1cm}
% {
% \begin{minipage}{.5\textwidth}
% \begin{figure}[H] 
% \begin{flushright}
% \includegraphics[width=0.7\textwidth]{figures/model_arch.JPG} 
% \caption{Model Architecture
% \xiang{@Hansen, pls update this figure and beautify it more.}} 
%  \end{flushright}
% \label{model_figure} 
% \end{figure}




% \begin{algorithm}[H]
% \SetAlgoLined
% % \KwResult{Write here the result }
%  Parameters: $S, T, T_1, T_2, T_3 \;$
%  initialization:$\mathcal{B}$,$h_0\;$
%  \For{n=1,2,...,S }{

%   \For{t=1,2,...,T}{
%     Randomly select $a_t^{(0)}$\;
%     Calculate $Q_{1,\theta}$ by \eqref{cal_Q1}\;
%     With $\epsilon$ probability, randomly select $a_t^{(1)}$, otherwise $a_t^{(1)}=\text{argmax}Q_{1,\theta}(a|s_t,a_t^{(0)}) $\;
%     Calculate $Q_{2,\phi}$ by \eqref{cal_Q2}\;
%     With $\epsilon$ probability, randomly select $a_t^{(2)}$, otherwise $a_t^{(2)}=\text{argmax}Q_{2,\phi}(a|s_t,a_t^{(0)},a_t^{(1)}) $\;
%     Calculate $s_{t+1}$ \text{through LSTM Cell} \;
%     \If{t==T}{
%     Evaluate KG on downstream tasks and get $r$ by \eqref{reward}}
%     \Else{r=0}
%     Store ($s_t$,$a_t$,$s_{t+1}$,r) in $\mathcal{B}$
%     \If{t mod $T_1==0$}{
%         sample a batch from $\mathcal{B}$ \;
%         update through \eqref{bellman} \;
%     }
%     \If{t mod $T_2==0$}{
%         $\theta_1^\prime = \theta_1$, $\phi_1^\prime = \phi_1$
%     }
    
%   }
%  }
%  \For{t=1,2,...,$T_3$}{
%       \text{ sample a batch from} $\mathcal{B}$ \;
%         \text{update through} \eqref{bellman} \;
%  }
 
%  \caption{Training process of our DQN}
% \end{algorithm}
% \end{minipage}}
% &
% \begin{minipage}{.5\textwidth}

% \end{minipage}
% \end{tabular}


% \begin{algorithm}[H]
% \SetAlgoLined
% % \KwResult{Write here the result }
%  Parameters: $S, T, T_1, T_2, T_3 \;$
%  initialization:$\mathcal{B}$,$h_0\;$
%  \For{n=1,2,...,S }{

%   \For{t=1,2,...,T}{
%     Randomly select $a_t^{(0)}$\;
%     Calculate $Q_{1,\theta}$ by \eqref{cal_Q1}\;
%     With $\epsilon$ probability, randomly select $a_t^{(1)}$, otherwise $a_t^{(1)}=\text{argmax}Q_{1,\theta}(a|s_t,a_t^{(0)}) $\;
%     Calculate $Q_{2,\phi}$ by \eqref{cal_Q2}\;
%     With $\epsilon$ probability, randomly select $a_t^{(2)}$ \;
%     otherwise $a_t^{(2)}=\text{argmax}Q_{2,\phi}(a|s_t,a_t^{(0)},a_t^{(1)}) $\;
%     Calculate $s_{t+1}$ \text{through LSTM Cell} \;
%     \If{t==T}{
%     Evaluate KG on downstream tasks and get $r$ by \eqref{reward}}
%     \Else{r=0}
%     Store ($s_t$,$a_t$,$s_{t+1}$,r) in $\mathcal{B}$
%     \If{t mod $T_1==0$}{
%         sample a batch from $\mathcal{B}$ \;
%         update through \eqref{Bellman1} \eqref{Bellman2} \;
%     }
%     \If{t mod $T_2==0$}{
%         $\theta_1^\prime = \theta_1$, $\phi_1^\prime = \phi_1$
%     }
    
%   }
%  }
%  \For{t=1,2,...,$T_3$}{
%       \text{ sample a batch from} $\mathcal{B}$ \;
%         \text{update through} \eqref{bellman} \;
%  }
 
%  \caption{Training process of our DQN}
% \end{algorithm}



% \begin{figure}[htbp]
% \centering
% \begin{minipage}[c]{0.4\textwidth}
% \centering
% \includegraphics[width=0.7\textwidth]{figures/model_arch.JPG}
% \caption{Model Architecture} 
% \label{model_figure} 
% \end{minipage}

% \noindent
% \begin{minipage}[c]{0.4\textwidth}
% \centering




% \end{minipage}
% \end{figure}

\textbf{DQN Architecture and Training \hspace{1mm}}
To train RL-RR and RL-ER, we use the Deep Q-Networks (DQN) algorithm ~\citep{mnih2015human}. With DQN, our goal is to learn a Q-function $Q(s_t, a_t)$, which outputs the expected reward for taking action $a_t$ in state $s_t$ at time step $t$. 

The DQN requires the embeddings $s_t$ of the current state \begin{small}$\mathcal{G}_t$\end{small} as input. A common approach to represent the current state is by GNN-based graph encoder \begin{small}$s_t=\text{GNN}(\mathcal{G}_t)$\end{small}. However, such method is not suitable for our task, since one of our goal is to examine whether these graph encoders have captured the information of KG. Thus it will conflict with our goal if we use our questioned object in our examining method. Therefore, we alternatively leverage a LSTM \citep{hochreiter1997long} for the state embedding. At each step, we feed the embedding of the chosen action $a_t$ into LSTM, and then the perturbed graph is represented by the output hidden vector of LSTM, \textit{i.e.}, \begin{small}$h_t=\text{LSTM}(s_0, [a_1, a_2,...,a_t])$\end{small}. However, the perturbed actions \begin{small}$a_1, a_2,...,a_t$\end{small} are fed sequentially to LSTM, and thus the state embedding $s_t$ will not preserve the order-invariant property. It would mean that a given state would depend on the order of perturbations performed which is not what we desire. To alleviate this issue, we randomly shuffle the order of actions while training and re-calculate the state embeddings of the DQN for the random ordering. Thus the model is forced to learn order invariant embeddings.


% At each time step $t$, we predict a perturbation action, \begin{small}$a_t = (a_t^{(0)}, a_t^{(1)}, a_t^{(2)})$\end{small}. 
% As shown in Figure \ref{fig:model_figure}, this involves two stages, which are parameterized by an LSTM \citep{hochreiter1997long} encoder and two MLP Q-functions. In the first stage, we randomly select 
The subaction \begin{small}$a_t^{(1)}$\end{small} depends on \begin{small}$a_t^{(0)}$\end{small} and similarly  \begin{small}$a_t^{(2)}$\end{small} depends on \begin{small}$a_t^{(1)}$\end{small}, \begin{small}$a_t^{(0)}$\end{small}. To solve for such action spaces, 
we use a hierarchical system of two DQNs to choose these. \begin{small}$a_t^{(0)}$\end{small} is chosen randomly. The first DQN takes the state and \begin{small}$a_t^{(0)}$\end{small} to sample \begin{small}$a_t^{(1)}$\end{small} and the second DQN follows similar procedure to sample \begin{small}$a_t^{(2)}$\end{small}. The actions for both the perturbations are kept similar to ensure that the same hierarchical framework works for both of them.

% At time step $t$, state \begin{small}$\mathcal{G}_t$\end{small} is encoded into an embedding $s_t$. At each step, we feed the embedding of the chosen action $a_t$ into LSTM, and then the perturbed graph is represented by the output hidden vector of LSTM, \textit{i.e.}, \begin{small}$h_t=\text{LSTM}(s_0, [a_1, a_2,...,a_t])$\end{small}. 

% A common approach to represent the current state is by GNN-based graph encoder \begin{small}$s_t=\text{GNN}(\mathcal{G}_t)$\end{small}. However, such method is not suitable for our task, since one of our goal is to examine whether these graph encoders have captured the information of KG. Thus it will conflict with our goal if we use our questioned object in our examining method. 

% However, the perturbed actions \begin{small}$a_1, a_2,...,a_t$\end{small} are fed sequentially to LSTM, and thus the state embedding $s_t$ will not preserve the order-invariant property. It would mean that a given state would depend on the order of perturbations performed which is not what we desire. To alleviate this issue, we randomly shuffle the order of actions while training and re-calculate the state embeddings of the DQN for the random ordering. Thus the model is forced to learn order invariant embeddings.


% The DQN requires the embeddings $s_t$ of the current state \begin{small}$\mathcal{G}_t$\end{small} as input. A common approach to represent the current state is by GNN-based graph encoder \begin{small}$s_t=\text{GNN}(\mathcal{G}_t)$\end{small}. However, such method is not suitable for our task, since one of our goal is to examine whether these graph encoders have captured the information of KG. Thus it will conflict with our goal if we use our questioned object in our examining method. Therefore, we alternatively leverage a LSTM \citep{hochreiter1997long} for the state embedding. At each step, we feed the embedding of the chosen action $a_t$ into LSTM, and then the perturbed graph is represented by the output hidden vector of LSTM, \textit{i.e.}, \begin{small}$h_t=\text{LSTM}(s_0, [a_1, a_2,...,a_t])$\end{small}. However, the perturbed actions \begin{small}$a_1, a_2,...,a_t$\end{small} are fed sequentially to LSTM, and thus the state embedding $s_t$ will not preserve the order-invariant property. It would mean that a given state would depend on the order of perturbations performed which is not what we desire. To alleviate this issue, we randomly shuffle the order of actions while training and re-calculate the state embeddings of the DQN for the random ordering. Thus the model is forced to learn order invariant embeddings.

The proposed DQN architecture is illustrated in Figure \ref{fig:model_figure}. At the step $t$ of perturbing triples in the KG, the state embedding $s_t$ together with the chosen actions are fed into the LSTM Cell to form the Q functions $Q_1$ and $Q_2$ as follows:
% $$ Q_1(a_t^{(1)}|s_t,a_t^{(0)})=\text{Dot}(MLP(a_t^{(1)}),MLP(h_t^{(1)})) $$
% $$ Q_2(a_t^{(2)}|s_t,a_t^{(0)},a_t^{(1)})=\text{Dot}(MLP(a_t^{(2)}),MLP(h_t^{(2)})) $$
% \vspace{-0.05cm}
\begin{small}
\begin{equation}
Q_1(a_t^{(1)}|s_t,a_t^{(0)})= \langle MLP(a_t^{(1)}),MLP(h_t^{(1)})\rangle; \label{cal_Q1} 
\end{equation}
\vspace{-0.3cm}
\begin{equation}
 Q_2(a_t^{(2)}|s_t,a_t^{(0)},a_t^{(1)})=\langle MLP(a_t^{(2)}),MLP(h_t^{(2)}) \rangle; \label{cal_Q2} \end{equation}
 \end{small}
where $h_t^{(1)}=\text{LSTMCell}_1(s_t,a_t^{(0)})$ and $h_t^{(2)}=\text{LSTMCell}_2(s_t,[a_t^{(1)},a_t^{(0)}])$ are the immediate hidden representation of current state. 
Actions $a_t^{(1)}$ and $a_t^{(2)}$ are chosen via Q function $\epsilon$-greedily during training and greedily during evaluation.

Evaluating the KG on downstream task is heavily time-consuming, and our task also requires a large number of perturbations. Therefore, we only get rewards every $T$ steps. $T$ can be as large as hundreds. In this way, the Q function $Q(s_t,a_t)$ is to predict the expectation of reward at step $T$ if we choose action $a_t$ at current state $s_t$. 

The training of DQN follows the common approach. Q functions are updated through Q-iterations minimizing the Bellman Error as follows.
\begin{small}
\begin{equation}
\theta \leftarrow \theta - \alpha \nabla_\theta (\gamma \max_{a_t^{(2)}} Q_{2,\phi^\prime}(a_t^{(2)}|s_t,a_t^{(0)},a_t^{(1)})-Q_{1,\theta}(a_t^{(1)}|s_t,a_t^{(0)}))^2; \label{Bellman1}
\end{equation}
\vspace{-0.3cm}
\begin{equation}
\phi \leftarrow \phi - \alpha \nabla_\phi ((r + \gamma \max_{a_{t+1}^{(1)}} Q_{1,\theta^\prime}(a_{t+1}^{(1)}|s_{t+1},a_{t+1}^{(0)}))-Q_{2,\phi}(a_{t}^{(2)}|s_t))^2.  \label{Bellman2}
\end{equation}
\end{small}
In this way, we are able to train the DQN and learn our targeted perturbation policy.
% The overall training framework is summarized in Algorithm 1.


% \xiang{where is the algorithm box??}


    
% \subsection{Validation Score}
% Since our aim is to perturb the Knowledge Graph we require a metric to judge the extent to which the graph has been corrupted. To this end we suggest the use of the following two different types of validation scores:
% \begin{itemize}
%     \item Embedding Based Validation Score: This validation score is derived from a Knowledge Base Completion model trained on Conceptnet. We train the embedding based Knowledge base completion architecture as specified in \citep{li-etal-2016-commonsense} on Conceptnet. This model take a triple as input and outputs the probability of the triple being semantically correct. We define the score of a triple to be this probability. We define the validation score of a graph to be the mean of scores of each triple in the graph. A thing to note is that this validation score will fail to capture the structure changes in the graph as will be evident in the experiments section. To alleviate this problem we use another validation score.
%     \item Structure Based Validation Score: This validation score is based on the observable properties of a Graph such as clustering coefficient. To incorporate relational information we first extract subgraphs from the complete graph that contain only a given relation. Then we find the mean of the clustering coefficient distributions of all such subgraphs. Then we use the reciprocal of the L2 distance between the mean distributions of the perturbed graph and the original graph. Note that unlike the Embedding based validation score this validation score does whether a triple makes semantic sense. Thus for our work it is of prime importance we use both these validation scores. 
% \end{itemize}

% \subsection{Semantic Based Perturbation}
% This is the first type of perturbation that we aim to achieve on a KG. Using this type of perturbations we try to corrupt the graph without changing the structure of the KG. 
% For this type of perturbations, we will choose a triple and substitute its relation type with another relation type at each step. We will do a large amount of steps to make sure the graph is largely perturbed. We decompose a single step into three sub-actions: action0 is to choose a head entity from the KG, action1 is to choose a tail entity from the neighborhood of head entity, and action2 is to choose the relation type to substitute for the original one. 
% In order to maintain high performance on downstream tasks with the largely perturbed KG, we leverage the Deep Q-networks(DQN), a reinforcement learning algorithm for this task. We view the downstream task performance as environment, and our perturbation policy as the agent. Thus the DQN is to learn a Q-function for the actions, and use rewards from downstream task performance to update its parameters. 
% Since we will perturb a large percentage of KG, the choice of action0 is not decisive. Therefore, we randomly choose action0 at each step. We use 2 DQNs for selecting action1 and action2, respectively. In order to ensure we are really perturbing the graph heavily, action2 (the relation type) is selected from the K actions with lowest validation score. In experiments, we set K=5.



% \subsection{Structure Based Perturbation}
% For this type of perturbation, we will choose a triple and substitute its tail entity with another tail entity at each step. We will do a large amount of steps to make sure the graph is largely perturbed. Similar to semantic based perturbation, we decompose a single step into three sub-actions: action0 is to choose a head entity from the KG, action1 is to choose a tail entity from the neighborhood of head entity, and action2 is to choose another tail entity to substitute for the original one. 
% %%

==> backup/backup_Nov15/5_experiments.tex <==
% !TEX root = main.tex

\section{Experiments}
\label{sec:exp}
\vspace{-0.1cm}


% \begin{figure}[tb!]
% \vspace{-0.6cm}
% \centering
% \subfloat[][Test Accuracy on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Rel_Acc_MHGRN.png}}
% \subfloat[][ATS on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Rel_Val_Score_MHGRN.png}}
% \subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_AUC_Music.png}}
% \subfloat[][ATS on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_Val_score_music.png}}
% \vspace{-0.1cm}
% \caption{Variation of Performance and Evaluation Metrics with scale of perturbation on KGCN with Last.FM and MHGRN with CSQA.  The horizontal axis
%  shows the scale of perturbation, i.e., the percentage of edges being perturbed.}
% \vspace{-0.1cm}
% \label{fig:heur_curves}
% \end{figure}

% \begin{figure}[tb!]
% \vspace{-0.6cm}
% \centering
% \subfloat[][Test Accuracy on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Rel_Acc_MHGRN.png}}
% \subfloat[][ATS on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Rel_Val_Score_MHGRN.png}}
% \subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_AUC_Music.png}}
% \subfloat[][ATS on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_Val_score_music.png}}
% \vspace{-0.1cm}
% \caption{Variation of Performance and Evaluation Metrics with scale of perturbation on KGCN with Last.FM and MHGRN with CSQA.  The horizontal axis
%  shows the scale of perturbation, i.e., the percentage of edges being perturbed.}
% \vspace{-0.1cm}
% \label{fig:heur_curves}
% \end{figure}
% \textbf{Observations and Discussion.}
% We show curves of how the performance and the ATS metric change across different percentages(of total number of edges in the KG) of relation-based perturbations in Figure~\ref{fig:heur_curves}. We observe that simple heuristics are able to perturb the KG to a large extent (Figure~\ref{fig:heur_curves}-b) while maintaining the performance in the recommendation task (Figure~\ref{fig:heur_curves}-a). This casts doubt on the faithfulness of the symbolic knowledge for KGCN and motivates us to investigate other neural-symbolic models as well. 

% On the contrary, for MHGRN with CSQA we observe that indeed randomization of relations of the KG leads to a clear drop in performance (test accuracy), as shown in Figure~\ref{fig:heur_curves}-c. To further examine whether random noise could yield similar performance drop as simple heuristics do, we design three controlled noisy baselines where we replace the subgraph embeddings for each instance from MHGRN with (1) zero vectors, (2) random vectors or replace the entities and relation embeddings with random vectors. By doing so, the model achieves $53.99\%$, $52.48\%$ and $54.03\%$ in accuracy respectively, indicating that the simple heuristics just yield some meaningless knowledge embeddings.
% Since this is due to the fact that simple heuristics perturb KG blindly, we ask the question whether we can maintain the performance while corrupting a KG with some sophisticated perturbation policies. To this end in the next section we propose a RL based perturbation policy.


% \aaron{will organize above later}

In this section, we evaluate our proposed KG perturbation methods on their ability to increase the perturbed KG's semantic distance from the original KG, while maintaining downstream performance and the ability to facilitate faithful explanations. For both of our heuristic-based and RL-based perturbation methods, we test on the commonsense QA and recommender system downstream tasks. In addition, we conduct a user study where humans subjects are asked to rate original and perturbed KGs with respect to readability and usability for solving downstream tasks. 

% A frozen downstream model is used to ensure that the model does not have a chance to overfit to the perturbed graph. \aaron{figure out how to integrate this part}

%In this section we introduce our experimental setup. With the help of these experiments, we challenge the faifulness of the symbolic knowledge in the current models. 
%try to validate our hypothesis that current models on many tasks do not model the KG effectively.
%We use different types of perturbation techniques to show even if the KG is completely perturbed we can maintain the downstream performance. We also perform some analysis on the paths that the models deem important for a prediction which pose questions on the interpretability of such models.

% \vspace{-0.2cm}
% \subsection{Experiment Setup}
% \vspace{-0.2cm}

% \vspace{-0.2cm}
% \subsection{Baselines for Graph Perturbation}
% \vspace{-0.2cm}

% In addition to the Relation Swapping(RS) and Relation Replacement(RR) perturbation heuristics (\textsection~\ref{sec: pilotexpts}), we further introduce two other perturbation methods as baselines in our experiments.

% \textbf{Edge Rewiring (ER): } We first randomly select an edge $(h,r,t)$ in the KG. 
% %We denote by $\mathcal{N}(h)$ the set of neighbors for the entity $h$. 
% Let $k \in \mathcal{E} \setminus \mathcal{N}_1(h)$. 
% Then we rewire the edge to another one with the same relation, i.e.,
% $
%     \mathcal{T} \leftarrow (\mathcal{T} \setminus \{(h,r,t)\}) \cup \{(h,r,k)\}
% $.
% It alters the structure of the graph but keep the relation distribution across the KG constant. 

% \textbf{Edge Deletion (ED):} We randomly select an edge and delete it.
% % \begin{align}\label{eq:deletion-heuristic}
% %   &i \sim \text{UniformDiscrete}\{1,2,\ldots,|\mathcal{T}|\} \\
% % %   ,\quad \text{for } j=1,2,\ldots\\
% %     &\mathcal{T} \leftarrow \mathcal{T} \setminus \{e_i=(h,r,t)\} \nonumber
% % \end{align}\noindent
% %This heuristic clearly changes both the structure of the graph as well as the distribution of relations across the KG.
% This heuristic changes both the structure of the graph as well as the relation distribution across the KG. 
% Note that the ATS metric will fail to recognize these perturbations to the KG by design, since after deletion the remaining edges are still valid triples .

% In the next subsection we denote Relation Swapping Heuristic and Greedy Heuristic as Semantic Heuristic 1 and Semantic Heuristic 2 respectively. We denote Deletion Heuristic and Rewiring Heuristic as Structure Heuristic 1 and Structure Heuristic 2 respectively. Next we introduce the tasks on which we perform our experiments.


\vspace{-0.2cm}
\subsection{Evaluation Protocol and Metrics}
\vspace{-0.2cm}

% \xiang{touch on ACC and AUC metrics.}

To measure downstream performance, we use the standard evaluation metric for the given task. For commonsense QA, we measure performance using accuracy \citep{lin2019kagnet, feng2020scalable}, whereas, for recommender systems, we measure performance using AUC ~\citep{wang2019knowledge, wang2018ripplenet}. Also, the choice of edge scoring function $s_{\mathcal{G}}$ is task-specific, since KGs from different tasks may differ greatly with respect to semantics or connectivity. For commonsense QA, we use the scoring function from \citet{li-etal-2016-commonsense}, and, for recommender systems, we use the scoring function from \citet{yang2015embedding}.

In order to measure how much the perturbed KG has deviated from the original KG, we need metrics that capture both semantic and structural distance. Although the ATS metric does capture KG semantic distance to some extent, it is not sensitive to structural differences between KGs. To address this shortcoming of ATS, we consider two additional complementary metrics (SC2D and SD2) which do capture KG connectivity information. In the later experiments, we validate ATS, SC2D and SD2 by measuring how well they correlate with humans' perception of KG readability and usefulness.

\textbf{Similarity on Clustering Coefficient Distribution (SC2D) \hspace{1mm}} 
Given a KG \begin{small}$\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$\end{small}, we define \begin{small}$\mathcal{G}^r$\end{small} as the subgraph containing all the triples with a particular relation $r$, i.e., \begin{small}$\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
    where $\mathcal{T}^{'}=\{(e_1,r',e_2) \hspace{1mm} | \hspace{1mm} e_1,e_2\in\mathcal{E},r'=r\}$.\end{small}
% \ryan{This strategy looks at triangles that are all homogeneous in terms of their relation $r$, what about triangles that are not all of the same relation $r$, but mixed relations? There are typically far more of these, just by chance. But in any case, its unclear why they were ignored. It was probably done since the above way just makes it simple to apply standard algorithms, but hopefully we have a more solid reason and justification for this.}
We then compute the relation specific clustering coefficient vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective} of the $i^{th}$ entity and compute the average clustering vector $\mathbf{c}$ for the whole graph as the average of $\mathbf{c^r}$ over all $r \in \mathcal{R}$, i.e., $\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$.
We denote the average clustering vector for the unperturbed KG and the perturbed KG by $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ respectively. Therefore, the SC2D metric is defined as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$, i.e.,
$f^{SC2D}(\mathcal{G},\mathcal{G}^{'}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$
with $b$ as a constant for avoiding zero division.

\textbf{Similarity on Degree Distribution (SD2) \hspace{1mm}}
SC2D is not effective for cases where the KG has a very small local clustering coefficient. For example, the KG used for recommender systems is almost bipartite, such that the local clustering coefficient tends to be close to zero. Thus, we also use the SD2 metric, which captures structural changes even for KGs that are not compatible with SC2D. To compute SD2, we first create a set of graphs $\mathcal{G}^{r}$ for each relation $r \in \mathcal{R}$. We then calculate the relation specific degree vector $\mathbf{d^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{d^r}$ represents the degree of the $i^{th}$ node and calculate the average degree vector $\mathbf{d}$ for the whole graph as the mean of $\mathbf{d^r}$ over all $r \in \mathcal{R}$, i.e., $\mathbf{d} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{d^r}$.
We denote the average degree vector of the unperturbed KG and the perturbed KG by $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$ respectively. Therefore, the SD2 metric is defined as the reciprocal of the L2 distance between $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$, i.e.,
$
f^{SD2}(\mathcal{G},\mathcal{G}^{'}) = \frac{1}{\lVert \mathbf{d_{o}} - \mathbf{d_{p}} \rVert_2 + b}.
$

  



\begin{table*}[t]
\vspace{-0.1cm}
\centering
\caption{\textbf{CSQA Performance Across Perturbation Methods.} We report test accuracy using the in-house data split from \citet{lin2019kagnet} on CSQA. The results here are from perturbing all facts in the original KG. 
% \xiang{@Mrigank: 1. Use full names for the baselines? 2. go to 3 decimal places for the validation metrics; 3. Let's still show all the three metrics for both task; and explain the issues in writing.}
}
\label{tab:results:csqa}
\hspace{-0.3cm}
\vspace{-0.1cm}
\scalebox{0.80}{
\begin{tabular}{lcccccccc}
    \toprule 
    %\multirow{2}{*}{\textbf{Methods}}
    &
    \multicolumn{8}{c}{ \textbf{CSQA}}\\
    \cmidrule(lr){2-9} 
    & \multicolumn{4}{c}{ \textbf{RN}}&\multicolumn{4}{c}{ \textbf{MHGRN}} \\
    \cmidrule(lr){2-5}
    \cmidrule(lr){6-9}
    \textbf{Method}& Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) &  Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) \\
    \midrule
    {w/o KG} & 53.41 & - & - &- & 53.41 & - &- & -  \\
    {w/ KG} & 56.87 & 0.940&-&- & 57.21 & 0.940&-&- \\
    \midrule
    {Relation Swapping} & 53.42 & 0.831&0.168&6.20E-3 & 53.42 & 0.831& 0.168 & 6.20E-3  \\
    {Relation Replacement} & 53.42 & 0.329& 0.100&1.70E-3 & 52.22 & 0.329& 0.100&\textbf{1.70E-3}  \\
    {Edge Rewiring} & 53.42 & 0.505&0.131&2.31E-3 & 52.22 & 0.505&0.131&2.31E-3  \\
    {Edge Deletion} & 52.21 & 0.933&0.144&2.00E-3 & 51.00 & 0.933&0.144&2.00E-3  \\
    \midrule
    {RL-ER} & 54.89 & 0.346&\textbf{0.081}&1.76E-3 & 55.05 & 0.325&\textbf{0.073}&1.78E-3  \\
    {RL-RR} & \textbf{55.21} & \textbf{0.322}&0.102 & \textbf{1.66E-3}& \textbf{55.52} & \textbf{0.314}&0.101&1.78E-3 \\
    % {RL Edge} & 54.75 & 0.505&\textbf{0.082} & \textbf{55.15} & 0.542&\textbf{0.070} & 66.60 & 0.411&0.163 & 67.20 & 0.341&0.095 \\
    % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
    % \midrule
    % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
    % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
    % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    \bottomrule 
\end{tabular}
}
\vspace{-0.0cm}
\end{table*} 



\begin{table*}[t]
\vspace{-0.1cm}
\centering
\caption{\textbf{OBQA Performance Across Perturbation Methods.} We report the test accuracy on OBQA using the official data split. The results here are from perturbing all facts in the original KG.
% \xiang{@Mrigank: 1. Use full names for the baselines? 2. go to 3 decimal places for the validation metrics; 3. Let's still show all the three metrics for both task; and explain the issues in writing.}
}
\label{tab:results:obqa}
\hspace{-0.3cm}
\vspace{-0.1cm}
\scalebox{0.80}{
\begin{tabular}{lcccccccc}
    \toprule 
    %\multirow{2}{*}{\textbf{Methods}}
    &
    \multicolumn{8}{c}{ \textbf{OBQA}}\\
    \cmidrule(lr){2-9} 
    & \multicolumn{4}{c}{ \textbf{RN}} &\multicolumn{4}{c}{ \textbf{MHGRN}}\\
    \cmidrule(lr){2-5}
    \cmidrule(lr){6-9}
    % \cmidrule(lr){10-13}
    % \cmidrule(lr){14-17}
    \textbf{Method}& Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) & Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$)& SD2 ($\downarrow$) \\
    \midrule
    {w/o KG} &  62.00 & - & - &- & 62.00 & - &-&- \\
    {w/ KG}  & 66.80 & 0.934&-&- & 68.00 & 0.934&-&- \\
    \midrule
    {Relation Swapping}  & 67.00 & 0.857&0.189& 7.79E-3& 67.30& 0.857&0.189&7.79E-3 \\
    {Relation Replacement} & 66.80 & 0.269&0.105&1.84E-3 & 67.60 & 0.269&0.105&1.84E-3 \\
    {Edge Rewiring} & 66.60 & 0.620&0.172&7.31E-3 & 67.00 & 0.620&0.172&7.31E-3 \\
    {Edge Deletion} & 66.80 & 0.923&0.155& 2.19E-3&67.60 & 0.923&0.155&2.19E-3 \\
    \midrule
    {RL-ER} & 67.00 & 0.518&\textbf{0.100}& 5.55E-4&\textbf{67.80} & 0.584&\textbf{0.104}&6.49E-4 \\
    {RL-RR} & \textbf{67.30} & \textbf{0.255}&0.108 & \textbf{1.79E-4}& 67.70 & \textbf{0.248}&\textbf{0.104}&\textbf{1.75E-4} \\
    % {RL Edge} & 54.75 & 0.505&\textbf{0.082} & \textbf{55.15} & 0.542&\textbf{0.070} & 66.60 & 0.411&0.163 & 67.20 & 0.341&0.095 \\
    % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
    % \midrule
    % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
    % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
    % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    \bottomrule 
\end{tabular}
}
\vspace{-0.0cm}
\end{table*} 
\subsection{ Commonsense QA Experiments}
\vspace{-0.1cm}

%Given a dataset and a neuro symbolic QA model, we try to deceive the model into learning corrupt graph structures and giving invalid explanations using a perturbed KG. 
%We first introduce our experimental setup for the commonsense question answering task.

% \xiang{what is the task/problem setting (input and output, goal)? Should introduce before going into models..}

% \textbf{Setup.}
For commonsense QA, we conduct experiments on the CommonsenseQA (CSQA) and OpenBookQA (OBQA) datasets, both of which require external commonsense knowledge to answer the question. %In addition to CommonsenseQA dataset that we introduced in section\ref{sec: pilotexpts}, we also exhibit our experiments on OpenBookQA which is a question answering dataset that consists of science questions and shows improvement in performance after augmenting a Language Model with a KG. The labels for the official test set are available and we report our results on the official test set. We run our experiments MHGRN \citep{feng2020scalable}, RelationNet \citep{santoro2017simple} and Graph Networks \citep{battaglia2018relational}.
%\textbf{KG-augmented Models for QA.} 
% \xiang{1-2 sentences to summarize how these models are like (summarizing from previous section is okay).}
The NSKG QA models we experiment with are Relation Networks (RN)~\citep{santoro2017simple} and MHGRN ~\citep{feng2020scalable}. On commonsense QA, RN and MHGRN both significantly outperform non-KG models as well as many other NSKG models ~\citep{feng2020scalable}. For both RN and MHGRN, we use BERT-Base ~\citep{devlin2018bert} as the text encoder. Following the high-level procedure described in Section \ref{sec: problem_setting}, we first train both QA models on the original KG to obtain their original downstream performance, then keep the models frozen throughout the KG perturbation. As our KG, we use ConceptNet~\citep{speer2016conceptnet}, which has been commonly used by NSKG models on commonsense QA.
% and Graph Networks~\citep{battaglia2018relational} 
 
%For each instance in the dataset these models encode the subgraph containing the concepts from this instance and use these encodings for predicting the correct answer for a given question. Relation Net encodes the relational paths between concepts whereas MHGRN uses a Graph Neural Network to encode the subgraphs for each instance.

% \textbf{Evaluation Protocol and Metrics.}
% As discussed above, the ATS metric is not sensitive to structure perturbation in the KG. Thus, we adopt the \textbf{Similarity on Clustering Coefficient (SC2D)} as a complementary metric. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$, we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$, i.e., $\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
%     where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$.
% % \ryan{This strategy looks at triangles that are all homogeneous in terms of their relation $r$, what about triangles that are not all of the same relation $r$, but mixed relations? There are typically far more of these, just by chance. But in any case, its unclear why they were ignored. It was probably done since the above way just makes it simple to apply standard algorithms, but hopefully we have a more solid reason and justification for this.}
% We then compute the relation specific clustering coefficient vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective} of the $i^{th}$ node and compute the average clustering vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e., $\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$.
% We denote the average clustering vector for the unperturbed KG and the perturbed KG by $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ respectively. We then define the SC2D metric as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$, i.e.,
% $V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$
% with $b$ as a constant for avoiding zero division.





\textbf{Main Results \hspace{1mm}}
%For experiments on Question Answering, we take the complete conceptnet graph and prune it first such that it only contains edges that are relevant for the given dataset i.e for each edge either the head entity or the tail entity is a part of the given dataset. 
Table~\ref{tab:results:csqa} shows the results for RN and MHGRN on the CSQA dataset and Table~\ref{tab:results:obqa} shows the same for the OBQA dataset when perturbing all facts in the KG. In most cases, we find that our perturbation methods are able to maintain downstream performance. First, when using heuristic-based perturbation, RN and MHGRN perform on par with the ``w/o KG" baseline on CSQA, but manage to achieve similar test accuracy to that of the ``w/ KG" baseline on OBQA. Second, when using RL-based perturbation, both models get slightly worse test accuracy than the ``w/ KG" baseline does on CSQA. Meanwhile, for RL-based perturbation on OBQA, RN performs noticeably better than ``w/ KG", while MHGRN performs about the same as ``w/ KG". Plus, using a T-test with three runs for both models, we show that RL-based perturbation achieves a statistically significant improvement over their heuristic-based counterparts. Since the KG can be perturbed completely while preserving -- or even improving -- performance, it is likely that both RN and MHGRN are relying on unfaithful symbolic knowledge for making predictions. Later, we present a KG human evaluation which further supports this hypothesis.

Note that perturbing a fact is not guaranteed to yield invalid or novel facts in the resulting KG. Thus, different perturbation methods may result in perturbed KGs that differ in their respective degrees of deviation from the original KG. This is shown by the ATS, SC2D, and SD2 scores in Table~\ref{tab:results:csqa} and Table~\ref{tab:results:obqa}, which demonstrate that the RL-based perturbation methods generally yield more highly perturbed KGs than the heuristic-based perturbation methods do. However, these perturbed KGs do not necessarily contain meaningless noise, as Table~\ref{tab:randomized_baseline} shows that noisy KG perturbation baselines (\textsection~\ref{sec: pilotexpts}) lead to significant performance drop.

\textbf{Varying Perturbation Level \hspace{1mm}}
We also evaluate various perturbation methods with respect to level of perturbation. For MHGRN on CSQA, Figure~\ref{fig:final_curves}a-b illustrates downstream test accuracy and ATS as a function of the percentage of facts perturbed in the KG. We observe that RR and RL-RR are more effective than RS, for both test accuracy and ATS. Furthermore, for higher levels of perturbations, the RR and RL-RR maintain downstream performance better than RS does.  
%It indicates that the RL policy is able to perturb the KG to the same extent if not more as is evident from the drastic drop in evaluation metrics.

\begin{wraptable}{h}{0.38\textwidth}
% \vspace{-0.6cm}
\centering
\scalebox{0.8}{
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{CSQA}} & \multicolumn{2}{c}{\textbf{OBQA}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} & Read & Use & Read & Use \\
\midrule
Orig. KG & 0.580&0.420&0.711&0.232  \\
%\midrule
%RL1 &0.4178&0.2444&0.4200&0.1550\\
RL-RR &0.452&0.268&0.418&0.156\\
RL-ER&0.429&0.285&0.410&0.179\\
\bottomrule
    \end{tabular}
}
    \caption{\small \textbf{Human Evaluation.} Human ratings of the readability (Read) and usefulness (Use) of top-scoring KG paths from MHGRN.}
    \label{tab:user_study}
\end{wraptable}


\textbf{Noisy Baselines \hspace{1mm}}
To see whether the perturbed KGs using our proposed perturbation methods are really capturing more than just random noise, we compare them to three noisy baselines: (1) replace subgraph embedding with zero vector, (2) replace subgraph embedding with random vector, and (3) replace entity/relation embeddings with random vectors. We evaluate these noisy baselines with MHGRN on CSQA. As shown in Tables \ref{tab:randomized_baseline}, when using these noisy baselines, the model performs about the same as ``w/o KG" and much worse than ``w/ KG" or our proposed methods (Table \ref{tab:results:csqa}). This indicates that the perturbed KGs from our proposed methods are capturing more than just random noise, like the noisy baselines do, although the information they capture may not be readable or usable by humans.
% \xiang{loose end}


\textbf{Human Evaluation \hspace{1mm}}
% \xiang{@Peifeng: let’s write out the human evaluation paragraph and talk about the scores, inter-annotator agreement metric, and correlation metric}
To measure KGs' ability to provide faithful explanations, we conduct a human evaluation on high-scoring KG paths from MHGRN. In this user study, we consider the original KG as well as the KGs from RL-RR and RL-ER. First, for each KG method, we randomly select 10 questions from the CSQA and OBQA test sets which are answered correctly by the model. Next, for each of the 10 questions, we retrieve the top-scoring path for each answer choice, as determined by MHGRN's path decoder attention. After that, we ask five human annotators to rate each path along two dimensions: readability and usefulness.  Readability is defined as whether the facts within the path are understandable; it is rated on a scale of $[0, 1]$. Usefulness is defined as whether the paths are useful for predicting the correct answer; it is rated on a scale of $[0, 1, 2]$. For each dimension of a given question, the final rating is chosen via majority voting. In Table~\ref{tab:user_study}, for each method, we report the average rating for each dimension. To measure inter-annotator agreement, we use Fleiss' $\kappa$ and obtain values of $0.312$ and $0.314$ for readability and usability, respectively -- this indicates fair agreement between annotators. Compared to paths from the original KG, we find that paths from RL-RR and RL-ER are considerably less readable and less usable. This suggests that our proposed RL-based perturbation methods are effective, but also that NSKG models may not necessarily provide faithful explanations for their predictions. 




\begin{figure}[tb!]
\vspace{-0.4cm}
\centering
\subfloat[][Test Acc on CSQA]{\includegraphics[width=0.25\textwidth]{figures/final_MHGRN_Acc.png}}
\subfloat[][ATS on CSQA]{\includegraphics[width=0.25\textwidth]{figures/final_MHGRN_Val.png}}
\subfloat[][AUC on MovieLens]{\includegraphics[width=0.25\textwidth]{figures/final_reco_AUC.png}}
\subfloat[][ATS on MovieLens]{\includegraphics[width=0.25\textwidth]{figures/Final_reco_Val.png}}
\vspace{-0.1cm}
\caption{\textbf{Varying Perturbation Level.} Performance and KG distance with respect to perturbation level, for MHGRN on CSQA and RippleNet on MovieLens-20M. The horizontal axis denotes the percentage of perturbed edge in the KG.}
\label{fig:final_curves}
% \caption{Variation of Performance and Validation Scores with scale of perturbation on MHGRN with CSQA.
% \xiang{add two flat curves for w/ and w/o KG accuracy.}
% \xiang{enlarge font size; remove top/leftmost boundary; remove vertical grey lines.}
%\vspace{-1cm}
\vspace{-0.1cm}
\end{figure}


\begin{table}[t!]
\vspace{0.1cm}
% \quad
% \parbox{0.3\linewidth}{
% \vspace{-0.4cm}
% %\centering
% \scalebox{0.65}{
% \begin{tabular}{lcccc}
% \toprule
%         Model & Test Acc & ATS & SC2D & SD2  \\
%         \midrule
%          Edge Rewiring& 56 & 0.46\\
%          RL-ER& 56 & 0.46\\
%          RL-RR& 56 & 0.46\\
% \bottomrule
%     \end{tabular}
%     }
%     \caption{\small Ablation Study of study different perturbation techniques on MHGRN with OBQA}
%     \label{tab:ablation}
% }
% \quad
\parbox{0.47\linewidth}{
\centering
\small\scalebox{0.75}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{CSQA}} & \multicolumn{2}{c}{\textbf{OBQA}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} & \textbf{RN}&\textbf{MHGRN}& \textbf{RN}&\textbf{MHGRN}\\
\midrule
w/o KG &53.41&53.41&62.00&62.00\\
w/ KG &56.87&57.21&66.80&68.00\\
w/ zero graph emb. &53.10&53.99&64.80&66.40\\
w/ rand. graph emb. &52.60&52.48&64.75&65.90\\
w/ rand. KG emb. &53.02&54.03&64.45&64.85\\
\bottomrule
\end{tabular}
}
\caption{\small \textbf{Noisy Baselines for Commonsense QA.} Test accuracy of noisy baselines on CSQA and OBQA. The noisy baselines are: replace subgraph embedding with zero vector (w/ zero graph emb.), replace subgraph embedding with random vector (w/ rand. graph emb.), and replace entity/relation embeddings with random vectors (w/ rand. KG emb.).}
\label{tab:randomized_baseline}
}
\hfill
\parbox{0.475\linewidth}{
\small
\centering
\vspace{-0.7cm}
\scalebox{0.75}{\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Last.FM}} & \multicolumn{2}{c}{\textbf{MovieLens-20M}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} & \textbf{KGCN}&\textbf{RippleNet}& \textbf{KGCN}&\textbf{RippleNet}\\
\midrule
w/o KG &50.75&50.75&91.30&91.30\\
w/ KG &55.99&56.23&96.62&97.46\\
w/ rand. ngbd. &55.91&51.04&96.21&92.11\\
% w/ rand. KG emb. &53.02&54.03&53.01&56.85\\
\bottomrule
\end{tabular}}
\caption{\small \textbf{Noisy Baselines for Recommender Systems.} Test AUC of noisy baselines on Last.FM and MovieLens-20M. For KGCN, we randomize the neighborhood of each entity; for RippleNet, we randomize the ripple set of each user (w/ rand. ngbd.). 
% \footnote{need to explain what happen to the SC2D metric for rec dataset in footnote.}
}
\label{tab:randomized_reco}
}
\vspace{-0.0cm}
\end{table}



\textbf{Quality of Evaluation Metrics \hspace{1mm}}
Using the results of our human evaluation, we validate the effectiveness of our three proposed KG distance metrics: ATS, SC2D and SD2. We find that the Pearson correlation coefficient between the human evaluation scores in Table~\ref{tab:user_study} and the three KG distance scores in Table~\ref{tab:results:csqa} and Table~\ref{tab:results:obqa} are $0.845$, $0.932$ and $0.932$, respectively. This indicates high correlation and demonstrates that the KG distance metrics well capture the semantic faithfulness of KGs.


% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on CommonsenseQA and OBQA perturbation experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA and on the official set of OBQA. We perturb all the triples in the KG
% % \xiang{@Mrigank: 1. Use full names for the baselines? 2. go to 3 decimal places for the validation metrics; 3. Let's still show all the three metrics for both task; and explain the issues in writing.}
% }
% \label{tab:results:csqa}
% \scalebox{0.65}{
% \begin{tabular}{lcccccccccccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{8}{c}{ \textbf{CSQA}}&\multicolumn{8}{c}{ \textbf{OBQA}}\\
%     \cmidrule(lr){2-9} \cmidrule(lr){10-17}
%     & \multicolumn{4}{c}{ \textbf{RN}}&\multicolumn{4}{c}{ \textbf{MHGRN}} &\multicolumn{4}{c}{ \textbf{RN}} &\multicolumn{4}{c}{ \textbf{MHGRN}}\\
%     \cmidrule(lr){2-5}
%     \cmidrule(lr){6-9}
%     \cmidrule(lr){10-13}
%     \cmidrule(lr){14-17}
%     & Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) &  Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) & Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$)  & Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) \\
%     \midrule
%     {w/o KG $^{\dagger}$} & ~53.71 & - & - & ~53.71 & - & - & ~62.00 & - & - & ~62.00 & -&- \\
%     {w/ KG} & 56.87 & 0.940&- & 57.21 & 0.940&- & 66.80 & 0.934&- & 68.00 & 0.934&- \\
%     \midrule
%     {Relation Swapping} & 53.42 & 0.831&0.168 & 53.42 & 0.831& 0.168 & 67.00 & 0.857&0.189& 67.80& 0.857&0.189 \\
%     {Relation Replacement} & 53.42 & 0.329&0.100 & 52.22 & 0.329&0.100 & 66.80 & 0.269&0.105 & 67.60 & 0.269&0.105 \\
%     {Edge Rewiring} & 53.42 & 0.505&0.131 & 52.22 & 0.505&0.131 & 66.60 & 0.620&0.172 & 67.00 & 0.620&0.172 \\
%     {Edge Deletion} & 52.21 & 0.933&0.144 & 51.00 & 0.933&0.144 & 66.80 & 0.923&0.155& 67.60 & 0.923&0.155 \\
%     \midrule
%     {RL Relation} & \textbf{55.12} & \textbf{0.312}&0.108 & 54.63 & \textbf{0.314}&0.101 & 66.40 & 0.273&0.104 & 67.20 & 0.278&0.104 \\
%     {RL Edge} & 54.75 & 0.505&\textbf{0.082} & \textbf{55.15} & 0.542&\textbf{0.070} & 66.60 & 0.411&0.163 & 67.20 & 0.341&0.095 \\
%     % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
%     % \midrule
%     % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
%     % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
%     % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*} 



% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on CommonsenseQA and OBQA perturbation experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA and on the official set of OBQA. We perturb all the triples in the KG
% % \xiang{@Mrigank: 1. Use full names for the baselines? 2. go to 3 decimal places for the validation metrics; 3. Let's still show all the three metrics for both task; and explain the issues in writing.}
% }
% \label{tab:results:csqa}
% \scalebox{0.65}{
% \begin{tabular}{lcccccccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{6}{c}{ \textbf{CSQA}}&\multicolumn{6}{c}{ \textbf{OBQA}}\\
%     \cmidrule(lr){2-7} \cmidrule(lr){8-13}
%     & \multicolumn{3}{c}{ \textbf{RN}}&\multicolumn{3}{c}{ \textbf{MHGRN}} &\multicolumn{3}{c}{ \textbf{RN}} &\multicolumn{3}{c}{ \textbf{MHGRN}}\\
%     \cmidrule(lr){2-4}
%     \cmidrule(lr){5-7}
%     \cmidrule(lr){8-10}
%     \cmidrule(lr){11-13}
%     & Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) &  Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) & Acc & ATS ($\downarrow$) & SC2D ($\downarrow$)  & Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) \\
%     \midrule
%     {w/o KG $^{\dagger}$} & ~53.71 & - & - & ~53.71 & - & - & ~62.00 & - & - & ~62.00 & -&- \\
%     {w/ KG} & 56.87 & 0.940&- & 57.21 & 0.940&- & 66.80 & 0.934&- & 68.00 & 0.934&- \\
%     \midrule
%     {Relation Swapping} & 53.42 & 0.831&0.168 & 53.42 & 0.831& 0.168 & 67.00 & 0.857&0.189& 67.80& 0.857&0.189 \\
%     {Relation Replacement} & 53.42 & 0.329&0.100 & 52.22 & 0.329&0.100 & 66.80 & 0.269&0.105 & 67.60 & 0.269&0.105 \\
%     {Edge Rewiring} & 53.42 & 0.505&0.131 & 52.22 & 0.505&0.131 & 66.60 & 0.620&0.172 & 67.00 & 0.620&0.172 \\
%     {Edge Deletion} & 52.21 & 0.933&0.144 & 51.00 & 0.933&0.144 & 66.80 & 0.923&0.155& 67.60 & 0.923&0.155 \\
%     \midrule
%     {RL Relation} & \textbf{55.12} & \textbf{0.312}&0.108 & 54.63 & \textbf{0.314}&0.101 & 66.40 & 0.273&0.104 & 67.20 & 0.278&0.104 \\
%     {RL Edge} & 54.75 & 0.505&\textbf{0.082} & \textbf{55.15} & 0.542&\textbf{0.070} & 66.60 & 0.411&0.163 & 67.20 & 0.341&0.095 \\
%     % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
%     % \midrule
%     % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
%     % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
%     % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*} 


\vspace{-0.1cm}
\subsection{Recommender System Experiments}
% \vspace{-0.2cm}
%Given a dataset and a KG augmented recommendation model, we try to perturb the KG using different methods and analyze the performance of the model. This task uses a subgraph sampled from the Microsoft Satori Knowledge Base.
% \xiang{what is the task/problem setting (input and output, goal)? Should introduce before going into models..}

% \textbf{Setup.} 
We consider two recommender system benchmarks: Last.FM~\citep{rendle2012libfm} and MovieLens-20M ~\citep{harper2016movielens}. KGs have been shown to benefit recommender systems in cold start scenarios ~\citep{wang2018ripplenet}. Following ~\citet{wang2018ripplenet}, we simulate a cold start scenario by using 20\% of the train set for Last.FM and 40\% of the train set for Movie Lens-20M.
%\textbf{KG-augmented Models for Recommender Systems.}
% \xiang{similarly, 2 sentences to overview these methods.}
We experiment with KGCN ~\citep{wang2019knowledge} and RippleNet ~\citep{wang2018ripplenet} as the NSKG models for our recommender systems. Like with commonsense QA, both models are first trained on the recommender system datasets with the original KG, then frozen throughout the KG perturbation. For both Last.FM and MovieLens-20M, we use the item KG from ~\cite{wang2019aknowledge}. Since the item KG is almost bipartite, the local clustering coefficient of each node is extremely small, which makes the SC2D metric meaningless in this case. Therefore, for recommender system experiments, we do not report SC2D results.

% \textbf{Evaluation Protocol and Metrics.}
% The KG used for recommendation tasks has a very low clustering coefficient. Therefore, we introduce another evaluation metric, Similarity on Degree Distribution (SD2), which can also capture structural changes. Similar to the SC2D metric, we first create a set of graphs $\mathcal{G}^{r}$ for each relation $r \in \mathcal{R}$. We then calculate the relation specific degree vector $\mathbf{d^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{d^r}$ represents the degree of the $i^{th}$ node and calculate the average degree vector $\mathbf{d}$ for the whole graph as the mean of $\mathbf{d^r}$ over all $r \in \mathcal{R}$, i.e., $\mathbf{d} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{d^r}$.
% We denote the average degree vector of the unperturbed KG and the perturbed KG by $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$ respectively. We then define the SD2 metric of the KG as the reciprocal of the L2 distance between $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$, i.e.,
% $
% V_{dc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{d_{o}} - \mathbf{d_{p}} \rVert_2 + b}.
% $


\begin{table*}[tb!]
\vspace{0.1cm}
\centering
\caption{\textbf{Recommender System Performance Across Perturbation Methods.} We report the test AUC for KGCN and RippleNet on Last.FM and MovieLens-20M. The results here are from perturbing facts in the original KG. Note that the SD2C metric is not included here, since the local clustering coefficient is too small to be meaningful.}
% \footnote{need to explain what happen to the SC2D metric for rec dataset in footnote.}
\scalebox{0.60}{
\begin{tabular}{lcccccccccccc}
    \toprule  
    \multirow{2}{*}{\textbf{Method}}&
    \multicolumn{6}{c}{ \textbf{Last.FM}}&\multicolumn{6}{c}{ \textbf{MovieLens 20M}}\\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13}
    & \multicolumn{3}{c}{ \textbf{KGCN}}&\multicolumn{3}{c}{ \textbf{RippleNet}} &\multicolumn{3}{c}{ \textbf{KGCN}} &\multicolumn{3}{c}{ \textbf{RippleNet}}\\
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    \cmidrule(lr){11-13}
    & AUC ($\uparrow$) & ATS ($\downarrow$) & SD2 ($\downarrow$) &  AUC ($\uparrow$)& ATS ($\downarrow$)  & SD2 ($\downarrow$)& AUC ($\uparrow$)& ATS ($\downarrow$)  & SD2 ($\downarrow$) & AUC ($\uparrow$)& ATS ($\downarrow$) & SD2 ($\downarrow$) \\
    \midrule
    {w/o KG} & ~50.75 & -&- & ~50.75 & -&- & ~91.30 & -&- & ~91.30 & -&- \\
    {w/ KG} & 55.99 & 0.972&- & 56.23 & 0.972&- & 96.62 & 0.960&- & 97.46 & 0.960&- \\
    \midrule
    {Relation Swapping} & 55.98 & 0.681&3.05E-2 & 56.23 & 0.681&3.05E-2 & \textbf{96.62} & 0.678&6.14E-4 & \textbf{97.46} & 0.678&6.14E-4 \\
    {Relation Replacement} & 55.98 & 0.415&0.339 & 56.22 & 0.415&0.339 & 96.50 & 0.413&\textbf{7.74E-5} & 97.45 & 0.413&\textbf{7.74E-5} \\
    {Edge Rewiring} & 55.98 & 0.437&1.89E-2 & 53.74& 0.320&6.28E-3 & 96.24 & 0.679&4.44E-4 & 93.42 & 0.739&3.16E-4 \\
    {Edge Deletion} & 50.96 & 0.941& 3.38E-3 & 45.98 & 0.941& 3.38E-3 & 90.36 & 0.982&1.02E-4 & 90.22 & 0.982&1.02E-4 \\
    \midrule
    {RL-ER}  & 55.49 & 0.345&5.45E-3 & 54.97 & 0.343&5.44E-3 & 95.79 & 0.454& 3.50E-4&95.08 & 0.791&5.51E-4 \\
    {RL-RR} & \textbf{56.04} & \textbf{0.320}&\textbf{1.3E-3} & \textbf{56.28} & \textbf{0.310}&\textbf{1.2E-3} & 96.53 & \textbf{0.401}&2.23E-4 & 97.25 & \textbf{0.268}&2.21E-4 \\
%     {RL Edge} & 56.23 & 7.8E-1&9.6E-1 & 56.21 & 9.4E-1&3.6E-1 & 97.46 & 6.1E-1&1.7E-1 & 97.43 & 9.3E-1&3.1E-2 \\
    % {RL Edge} & 54.75 & 0.505&\textbf{0.082} & \textbf{55.15} & 0.542&\textbf{0.070} & 66.60 & 0.411&0.163 & 67.20 & 0.341&0.095 \\
    % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
    % \midrule
    % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
    % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
    % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    \bottomrule 
\end{tabular}
}\label{tab:results:reco}
\vspace{-0.0cm}
\end{table*} 


\textbf{Main Results \hspace{1mm}} 
In Table~\ref{tab:results:reco}, we report performance with respect to downstream test AUC, ATS, and SD2. For each perturbation method, we report performance for when all facts in the KG have been perturbed. 
%Since clustering coefficient based evaluation metric is not very suitable for this task, we report the degree evaluation metric along with the embedding based evaluation metric. The key takeaway from Table~\ref{tab:results:reco} is that a
%We use the official split of 6:2:2 for train, dev and test set as specified in \citep{wang2019knowledge} for our experiments.
% We observe that despite a completely perturbed graph, the change in performance is statistically insignificant according to the T test with 3 independent runs regardless of what type of perturbation we do. This strongly suggests that it is the (false) connection between entities instead of the semantic stored in the KG that leads to the improvement over non-KG baseline. Thus, the neural-symbolic recommender system built on top of these false connection could hardly provide any faithful explanation.
We observe that, for KGCN, all perturbation methods (except ED) achieve roughly the same AUC as ``w/ KG" does. Meanwhile, for RippleNet, all perturbation methods (except ER and ED) achieve roughly the same AUC as ``w/ KG" does. Using the T-test with three independent runs, for almost all perturbation methods, we find a statistically insignificant difference between AUC from the perturbed KG and AUC from the original KG. Unlike QA systems (which also have a text encoder), recommender systems depend solely on the KG for their predictions. Thus, ED performs about the same as ``w/o KG", since almost all edges are being deleted. However, other perturbation methods produce KGs that are completely perturbed yet somehow still contain enough information to provide improved performance over the ``w/o KG" baselines. This suggests that NSKG recommender systems using these perturbed graphs are making correct predictions while being unable to faithfully explain them.

\textbf{Varying Perturbation Level \hspace{1mm}}
For RippleNet on MovieLens-20M, Figure~\ref{fig:final_curves}c-d shows how downstream performance and KG distance change as a function of the number of perturbation steps. Across different perturbation methods, as the number of perturbation steps increases, we observe negligible change in performance (i.e., flat curve). Meanwhile, ATS drops drastically, indicating that the KG's semantics are being significantly perturbed. This suggests that RippleNet is not using the KG in a faithful manner for making predictions.  %Note that the drop in performance is insignificant for all scales of perturbation but the KG changes considerably as can be seen from the drastic drop in the evaluation metrics.


\textbf{Noisy Baseline \hspace{1mm}}
In Table \ref{tab:randomized_reco}, we consider the additional noisy baseline of randomizing each entity's neighborhood. For RippleNet, this means randomizing the ripple set. On this baseline, we find that KGCN performs about the same as ``w/ KG", while RippleNet performs significantly worse. Since Ripplenet considers directed edges, it may use edge information in a finer-grained way, relying on the precise order of entities in the edge. The opposite may be true for KGCN, which only considers undirected edges. This may explain why RippleNet is more sensitive than KGCN to entity neighbor randomization. This hypothesis is also supported by Table \ref{tab:results:reco}, since RippleNet's performance drops when we perturb edge connections. Based on this evidence, we may conclude that RippleNet relies considerably on the KG's specific edge connectivity structure.

%These results provide a strong evidence to us for validating our claims that current neuro symbolic models do not capture the KG semantics and structure faithfully.


% \xiang{too short for this subsection; need to expand on the result discussion.}


% \begin{table*}[t]
% \centering
% \vspace{-0.2cm}
% \caption{\textbf{Performance comparison on recommendation based perturbation experiments} We report the test AUC on Last.FM and MovieLens-20M}
% \label{tab:results:reco}
% \scalebox{0.55}{
% \begin{tabular}{lcccccccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%   \multicolumn{6}{c}{ \textbf{Last.FM}}&\multicolumn{6}{c}{ \textbf{MovieLens 20M}}\\
%     \cmidrule(lr){2-7} \cmidrule(lr){8-13}
%     & \multicolumn{3}{c}{ \textbf{KGCN}}&\multicolumn{3}{c}{ \textbf{RippleNet}} &\multicolumn{3}{c}{ \textbf{KGCN}} &\multicolumn{3}{c}{ \textbf{Ripplenet}}\\
%     \cmidrule(lr){2-4}
%     \cmidrule(lr){5-7}
%     \cmidrule(lr){8-10}
%     \cmidrule(lr){11-13}
%     & Acc ($\uparrow$) & ATS ($\downarrow$) & SD2 ($\downarrow$) &  Acc & ATS ($\downarrow$) &  SD2 ($\downarrow$)& Acc & ATS ($\downarrow$) & SD2 ($\downarrow$) & Acc & ATS ($\downarrow$) &  SD2 ($\downarrow$)//
%     \midrule
%     {w/o KG $^{\dagger}$} & ~50.75 & -&- & ~50.75 & -&- & ~91.30 & -&- & ~91.30 & -&- \\
%     {w/ KG} & 55.99 & 0.972&- & 56.23 & 0.951&- & 96.62 & 0.962&- & 96.62 & 0.962&- \\
%     \midrule
%     {Relation Swapping} & 55.98 & 0.681&0.967 & 56.23 & 0.779&0.967 & 96.62 & 0.678&0.176 & 97.46 & 0.612&0.172 \\
%     {Greedy Relation Replacement} & 55.98 & 0.415&0.339 & 56.22 & 0.495&0.339 & 96.50 & 0.413&0.121 & 97.45 & 0.458&0.132 \\
%     {Edge Rewiring} & 56.04 & 0.437&0.417 & 56.22& 0.437&0.427 & 96.24 & 0.679&0.073 & 96.62 & 0.679&0.073 \\
%     {Edge Deletion} & 55.96 & 0.941&0.362 & 56.21 & 0.941&0.362 & 96.36 & 0.982&0.031 & 97.22 & 0.982&0.031 \\
%     \midrule
%     {RL Relation} & 56.23 & 0.95&- & 56.23 & 0.95&- & 97.46 & 0.96&- & 97.46 & 0.96&- \\
%     % {RL Edge} & 56.23 & 7.8E-1&9.6E-1 & 56.21 & 9.4E-1&3.6E-1 & 97.46 & 6.1E-1&1.7E-1 & 97.43 & 9.3E-1&3.1E-2 \\
%     % {RippleNet- Heuristic2} & 56.22 & 4.9E-1/-/3.4E-1 & 52.22 & 7.8E-1/-/4.2E-1 & 97.45 & 4.5E-1/-/1.3E-1 & 93.62 & 7.9E-1/-/7.6E-2 \\
%     % {RippleNet- RL} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*}

% \begin{figure}[tb!]
% \vspace{-0.2cm}
% \centering
% \subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_AUC_Music.png}}
% \subfloat[][Emb Val Score]{\includegraphics[width=0.25\textwidth]{figures/Relation_Val_score_music.png}}
% \subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Edge_AUC_Music.png}}
% \subfloat[][Degree Val Score]{\includegraphics[width=0.25\textwidth]{figures/Edge_Val_score_music.png}}
% \vspace{-0.2cm}
% \caption{Variation of Performance and Validation Scores with scale of perturbation on KGCN with Last.FM. \xiang{enlarge font size; remove top/leftmost boundary; remove vertical grey lines.}}
% \label{fig:heur_curvesKGCN}
% \end{figure}


% % In addition to MHGRN which we introduced in \ref{sec: pilotexpts} we also experiment on the following models for Commonsense Question Answering. 

% \textbf{Relation Net \citep{santoro2017simple}}: This is a path based model that has been adapted by \citep{feng2020scalable} for commonsense question answering. We use this model as it is simple yet powerful for the Commonsense Question Answering task. We augment this model with bert-base and use it on the CSQA \citep{talmor-etal-2019-commonsenseqa} and with roberta-large to use it on OBQA \citep{mihaylov-etal-2018-suit}. 

% \textbf{Graph Networks \citep{battaglia2018relational}}: Graph Networks is a general framework of encoding relational graphs such as a KG which we adapt to perform Commonsense Question Answering. As for Relation Net we augment this model with bert-base on CSQA and with roberta-large on OBQA.

% Since we will also perturb the structure of the KG, we need some evaluation metric that is more robust to structural changes than the ones introduced \ref{sec: pilotexpts}. To this end we introduce the following evaluation metric:

% \textbf{Clustering Coefficient based evaluation metric}: We design this evaluation metric in a way that it is robust to structural perturbation to the KG as well as perturbation to the edge types. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$ we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$ i.e $\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
%     where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$
% % \ryan{This strategy looks at triangles that are all homogeneous in terms of their relation $r$, what about triangles that are not all of the same relation $r$, but mixed relations? There are typically far more of these, just by chance. But in any case, its unclear why they were ignored. It was probably done since the above way just makes it simple to apply standard algorithms, but hopefully we have a more solid reason and justification for this.}
% We then calculate the relation specific clustering coefficient vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective} of the $i^{th}$ node and calculate the average clustering vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e $\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$
% We denote by $\mathbf{c_{o}}$, the average clustering vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{c_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ i.e
% $$V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$$
% with $b$ as a constant for avoiding zero division.

% \subsection{Recommendation}
% We introduce KGCN in \ref{sec: pilotexpts} for showcasing our pilot experiments. For this task we also work on the following model

% \textbf{Ripplenet \citep{wang2018ripplenet}} This is a KG based recommendation model that combines path based encoding and embedding based encoding of a KG. We use this model on the Last.FM and the Movie-Lens 20M datasets.

% One thing to note here is that we have a different KG for each dataset. The local clustering coefficients for the KG in this task are very small and do not provide much information. Thus for this task we introduce another evaluation metric which is quite similar to the clustering coefficient based evaluation metric.

%  \textbf{Degree Coefficient based evaluation metric: } Similar to the clustering coefficient based evaluation we first create a set of graphs $\mathcal{G}^{r}$ for each relation $r \in \mathcal{R}$. We then calculate the relation specific degree vector $\mathbf{d^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{d^r}$ represents the degree of the $i^{th}$ node and calculate the average degree vector $\mathbf{d}$ for the whole graph as the mean of $\mathbf{d^r}$ over all $r \in \mathcal{R}$ i.e $$\mathbf{d} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{d^r}$$
% We denote by $\mathbf{d_{o}}$, the average degree vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{d_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$ i.e
% \begin{equation}
% V_{dc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{d_{o}} - \mathbf{d_{p}} \rVert_2 + b}.
% \end{equation}

% To perturb the KG to a much lower evaluation metric while preserving the accuracy, we use DQNs to model the process.To ensure we only perturb relevant facts in the KG, we extract the subgraph containing only those concepts that appear in the Question Answer statements.

% We decompose the perturbation of a relation edge into three sub-actions: choosing a subject, choosing a object connected with the chosen subject, and substituting the relation edge between the chosen subject and object with another one. We choose the first sub-action randomly at each step, and use two DQNs to predict the reward after a fixed number of steps for the other two sub-actions.
% After a fixed number of steps, we use the change of accuracy on downstream tasks as the rewards.

% We've also tried 2 variants of DQN.

% For DQN Variant 1,
% we use the difference in probabilities of the correct answer in place of accuracy as the reward. We feel this can be a more informative reward.

% For DQN Variant 2, in order to make evaluation metric as low as possible,
% we use only 1 DQN to select the tail entity and use the relation that has the lowest evaluation metric as the action. Here we only use the probability change as reward and use the greedy strategy to decrease the evaluation metric.

% In comparison, we use two random methods for perturbation.  The heuristic 1 is that we select two edges at random and swap relations and heuristic 2 is we choose tail relation randomly and select the relation which minimizes the val metric of the triple.

% Results show that our RL method does work.

% Currently our DQN method does not contain previous actions as states, but only gives predictions based on current actions. Therefore, at evaluation, if we choose the same first sub-action, the second and third sub-action will be the same, which will limit the total number of changes. 
% Therefore, we'll next try to contain previous actions as states, and use it to make more changes. This will make evaluation metric much lower.
% In addition to the models, introduced in \ref{sec: pilotexpts} we also experiment on the following models.
% % \subsection{Heuristics}
% % We consider the following heuristics as a baseline for comparison of the experiments.

% % \textbf{Heuristic1}: Choose two edges at random and swap relations. (Write it more formally)

% % \textbf{Heuristic2}: Choose an edge at random and select the relation that minimizes the embedding based evaluation metric.(Write it more formally)

% % \textbf{Edge Heuristic1}: Select an edge at random and delete it. (Write it more formally)

% % \textbf{Edge Heuristic2}: Choose an edge at random and a third node at random. Remove the original edge and add it to the third node.

% % \subsection{Question Answering}
% % We experiment on the following Question Answering datasets. We also mention the Graph Encoder used in each of them. For this set of experiments we take the complete conceptnet graph and prune it first such that it only contains edges that are relevant for the given dataset i.e for each edge either the head entity or the tail entity is a part of the given dataset.

% % \textbf{CommonsenseQA}: CommonsenseQA is a commonsense question answering benchmark dataset that is derived from conceptnet and is one of those tasks which requires external knowledge in the form of a KG to perform well. Since the labels for the official test are not available we report our results on the inhouse test split of \citep{lin2019kagnet}. We exhibit our experiments on this dataset using MHGRN \citep{feng2020scalable}, RelationNet \citep{santoro2017simple} and Graph Networks \citep{velivckovic2018graph}. 

% % \textbf{OpenBookQA}: OpenBookQA is question answering dataset that consists of science questions which shows improvement in performance after augmenting a Language Model with a KG. The labels for the official test set are available and we report our results on the official test set. As in the case of CSQA we run our experiments on MHGRN, RelationNet and Graph Networks. 

% % \subsection{Recommendation}
% % We experiment on the following Recommendation datasets. We also mention the Graph Encoder used in each of them.

% % \textbf{Last.FM}: Last.FM contains user rating information on musicians and music from a set of 2 thousand users from Last.fm online music system. We demonstrate our experiments on this dataset on KGCN and Ripplenet

% % \textbf{MovieLens 20M}: MovieLens 20M is a widely used benchmark dataset in movie recommendations, which consists of approximately 20 million explicit ratings (ranging from 1 to 5) on the MovieLens website. We showcase our experiments on this dataset using KGCN and Ripplenet.
% \textbf{Relation Net \citep{santoro2017simple}}: This is a path based model that has been adapted by \citep{feng2020scalable} for commonsense question answering. We use this model as it is simple yet powerful for the COmmonsense Question Answering task. We augment this model with bert-base and use it on the CSQA \citep{talmor-etal-2019-commonsenseqa} and with roberta-large to use it on OBQA \citep{mihaylov-etal-2018-suit}. 

% \textbf{Graph Networks \citep{battaglia2018relational}}: Graph Networks is a general framework of encoding relational graphs such as a KG which we adapt to perform Commonsense Question Answering. As for Relation Net we augment this model with bert-base on CSQA and with roberta-large on OBQA.

% \textbf{Ripplenet \citep{wang2018ripplenet}} This is a KG based recommendation model that combines path based encoding and embedding based encoding of a KG. We use this model on the Last.FM and the Movie-Lens 20M datasets.

% In the next subsection we introduce some baseline methods for the perturbation of KG.
% \subsection{Baseline Methods}
% We introduced some heuristic perturbation methods in section \ref{sec: pilotexpts}. Now we introduce some other baselines to compare our perturbation policy in addition to those introduced in \ref{sec: pilotexpts}.

% \textbf{Rewiring Heuristic: } This is a heuristic that we design to alter the structure of the graph but keep the relation distribution across the KG constant. In this heuristic we first select an edge $(h,r,t)$ randomly. We denote by $\mathcal{N}(v)$, the set of neighbors of the node v. Let $k \in \mathcal{E} \setminus \mathcal{N}(h)$. 
% Then:
% \begin{align}\label{rewiring-heuristic}
%     \mathcal{T} \leftarrow \mathcal{T} \setminus \{(h,r,t)\} \cup \{(h,r,k)\}
% \end{align}
 

% \textbf{Deletion Heuristic:} In this heuristic we randomly select an edge and delete it.
% \begin{align}\label{eq:deletion-heuristic}
%   &i \sim \text{UniformDiscrete}\{1,2,\ldots,|\mathcal{T}|\} \\
% %   ,\quad \text{for } j=1,2,\ldots\\
%     &\mathcal{T} \leftarrow \mathcal{T} \setminus \{e_i=(h,r,t)\} \nonumber
% \end{align}\noindent
% This heuristic clearly changes both the structure of the graph as well as the distribution of relations across the KG.
% This is a heuristic that clearly changes both the structure of the graph as well as the relation distribution across the KG. 
% A very interesting observation should be that the embedding based evaluation metric will fail to recognize these perturbations to the KG by design. Since even if we delete edges the remaining edges are still valid triples of the KG which in turn keeps this evaluation metric almost unchanged. 
% For the next section we denote Relation Swapping Heuristic and Greedy Heuristic as Semantic Heuristic 1 and Semantic Heuristic 2 respectively. We denote Deletion Heuristic and Rewiring Heuristic as Structure Heuristic 1 and Structure Heuristic 2 respectively

% We also introduce two more evaluation metrics in this section that are more robust to structure of the KG than the embedding based evaluation metric.

% \textbf{Clustring Coefficient/Degree based evaluation metrics} We design this evaluation metric in a way that it is robust to structural perturbation to the KG as well as perturbation to the edge types. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$ we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$ i.e $\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
%   where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$
% We then calculate the relation specific clustering coefficient vector/ degee vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective}/ degree of the $i^{th}$ node and calculate the average clustering vector/ degree vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e $$\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$$
% We denote by $\mathbf{c_{o}}$, the average clustering/degree vector of the unperturbed KG and denote the average clustering/degree vector of the perturbed KG with $\mathbf{c_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ i.e
% $$V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$$
% with $b$ as a constant for avoiding zero division.

% In the next section we report our results and analysis of our experiments.

% \begin{table}[t]
% \parbox{0.45\linewidth}{
%     \begin{tabular}{lrrrr}
% \toprule
% \multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c}{CSQA} & \multicolumn{2}{c}{OBQA} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} & Val. & Int. & Val. & Int. \\
% \midrule
% Ori.& 3.03&2.17&3.48&2.17  \\
% \midrule
% RL1 &2.68&2.19&2.82&1.90\\
% RL2 &2.99&2.29&2.79&2.09\\
% \bottomrule
%     \end{tabular}
%     \caption{User Study on Paths}
%     \label{tab:user_study}
% }
% \quad
% \parbox{0.55\linewidth}{
% \begin{tabular}{c|c}
% \toprule
%          &  \\
%          & 
%     \end{tabular}
%     \caption{Abalation Study}
%     \label{tab:ablation}
% }
% \end{table}

==> backup/backup_Nov15/6_result.tex <==
% !TEX root = main.tex
\section{Results and Discussions}
Details about the results and the plots.

% \begin{table}[h]
% \centering
% \label{result-table-QA}
% \begin{center}
% \begin{tabular}{llllll}
% \multicolumn{1}{c}{\bf Model}& \multicolumn{1}{c}{\bf Perturb}  &\multicolumn{2}{c}{\bf QA1}  &\multicolumn{2}{c}{\bf QA2} 
% \\ & & Acc. &Val. & Acc. &Val.

% \\\hline \\
% Bert & - & 57.13 & 0.94& & \\
% Bert+RN & - & 59.50 &0.94 & & \\
% Bert+RN & Heuristic1 &58.10  &0.90 & & \\
% Bert+RN & Heuristic2 &58.60  &0.87 & & \\
% Bert+RN & DQN(Vanilla) &\textbf{59.45}  &\textbf{0.87} & & \\
% Bert+RN & DQN(Variant1) &59.00  &0.87 & & \\
% Bert+RN & DQN(Variant2) &59.30  &0.87 & & \\
% % \hline
% % AlBert+RN & - &  & & & \\
% % AlBert+RN & Random &  & & & \\
% % AlBert+RN & DQN &  & & & \\
% \hline
% \end{tabular}
% \caption{Accuracy of downstream tasks and validation score of the original or perturbed KG}
% \end{center}
% \end{table}

% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on CommonsenseQA and OBQA perturbation experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA and on the official set of OBQA}
% \label{tab:results:csqa}
% \scalebox{0.62}{
% \begin{tabular}{lcccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{4}{c}{ \textbf{CSQA}}&\multicolumn{4}{c}{ \textbf{OBQA}}\\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%     & \multicolumn{2}{c}{ \textbf{Semantic Perturbation}}&\multicolumn{2}{c}{ \textbf{Structure Perturbation}} &\multicolumn{2}{c}{ \textbf{Semantic Perturbation}} &\multicolumn{2}{c}{ \textbf{Structure Perturbation}}\\
%     \cmidrule(lr){2-3}
%     \cmidrule(lr){4-5}
%     \cmidrule(lr){6-7}
%     \cmidrule(lr){8-9}
%     & Acc & Emb/CC/DC &  Acc & Emb/CC/DC & Acc & Emb/CC/DC  & Acc & Emb/CC/DC \\
%     \midrule
%     {w/o KG $^{\dagger}$} & ~53.71 & -/-/- & ~53.71 & -/-/- & ~62.00 & -/-/- & ~62.00 & -/-/- \\
%     \midrule
%     {RN w KG} & 56.87 & 9.4E-1/-/- & 56.87 & 9.4E-1/-/- & 58.97 & 9.3E-1/-/- & 58.97 & 9.3E-1/-/- \\
%     {RN- Heuristic1} & 53.42 & 8.3E-1/1.6E-1/6.2E-3 & 52.21 & 9.3E-1/1.4E-1/2.0E-3 & 66.80 & 8.5E-1/1.8E-1/7.8E-3 & 66.80 & 9.2E-1/1.5E-1/2.2E-3 \\
%     {RN- Heuristic2} & 53.42 & 3.3E-1/1.0E-1/1.7E-3 & 52.53 & 5.6E-1/1.3E-1/5.4E-4 & 66.80 & 2.7E-1/1.1E-1/1.8E-3 & 66.60 & 6.2E-1/1.7E-1/7.3E-3 \\
%      {RN- RL} & 55.12 & 3.1E-1/1.1E-1/1.1E-2 & 54.15 & 5.1E-1/8.2E-2/5.2E-4 & 66.40 & 2.7E-1/1.0E-1/1.8E-3 & 66.60 & 6.5E-1/1.6E-1/8.8E-3 \\
%     \midrule
%     {MHGRN w KG} & 57.21 & 9.4E-1/-/- & 57.21 & 9.4E-1/-/- & 68 & 9.3E-1/-/- & 68 & 9.3E-1/-/- \\
%     {MHGRN- Heuristic1} & 53.42 & 8.3E-1/1.6E-1/6.2E-3 & 51.00 & 9.3E-1/1.4E-1/2.0E-3 & 67.80 & 8.5E-1/1.8E-1/7.8E-3 & 67.60 & 9.2E-1/1.5E-1/2.2E-3 \\
%     {MHGRN- Heuristic2} & 53.74 & 3.3E-1/1.0E-1/1.7E-3 & 53.02 & 6.4E-1/1.6E-1/6.1E-3 & 67.60 & 2.7E-1/1.1E-1/1.8E-3 & 67.00 & 6.5E-1/1.6E-1/8.8E-3 \\
%     {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
%     \midrule
%     {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
%     {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
%     {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on CommonsenseQA in-house split for semantic based experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA.}
% \label{tab:results:csqa}
% \scalebox{0.62}{
% \hskip-6.5cm
% \begin{tabular}{lcccccccccccccccccccccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{13}{c}{ \textbf{CSQA}}&\multicolumn{13}{c}{ \textbf{OBQA}}\\
%     \cmidrule(lr){2-14} \cmidrule(lr){15-27} 
%     & \multicolumn{1}{c}{\textbf{Original}}& \multicolumn{2}{c}{ \textbf{Relation Swapping}}&\multicolumn{2}{c}{ \textbf{Greedy}}&\multicolumn{2}{c}{ \textbf{RL}} &\multicolumn{2}{c}{ \textbf{Rewiring}} &\multicolumn{2}{c}{ \textbf{Deletion}}&\multicolumn{2}{c}{ \textbf{RL}}&\multicolumn{1}{c}{\textbf{Original}}&\multicolumn{2}{c}{ \textbf{Relation Swapping}}&\multicolumn{2}{c}{ \textbf{Greedy}} &\multicolumn{2}{c}{ \textbf{RL}} &\multicolumn{2}{c}{ \textbf{Rewiring}} &\multicolumn{2}{c}{ \textbf{Deletion}}&\multicolumn{2}{c}{ \textbf{RL}}\\
%     \cmidrule(lr){3-4}
%     \cmidrule(lr){5-6}
%     \cmidrule(lr){7-8}
%     \cmidrule(lr){9-10}
%     \cmidrule(lr){11-12}
%     \cmidrule(lr){13-14}
%     \cmidrule(lr){16-17}
%     \cmidrule(lr){18-19}
%     \cmidrule(lr){20-21}
%     \cmidrule(lr){22-23}
%     \cmidrule(lr){24-25}
%     \cmidrule(lr){26-27}
%     & Acc & Acc & Emb &  Acc & Emb&  Acc & Emb & Acc & CC  & Acc & CC & Acc & CC & Acc & Acc & Emb &  Acc & Emb & Acc & CC  & Acc & CC & Acc & CC & Acc & CC \\
%     \midrule
%      {w/o KG}& ~53.47 & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~62.00 & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & - \\
%      \midrule
%      RN & ~56.87 & ~53.42 & 0.831 & ~53.42 & 0.329 & ~55.12 & 0.313 & ~53.42 & 0.131 & ~52.21 &  & ~62.00 & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & -  & ~62.00 & - \\
    
%      MHGRN & ~53.47 & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~62.00 & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & -  & ~62.00 & - \\
%      GN & ~53.47 & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~62.00 & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & -  & ~62.00 & - \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*}



% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on recommendation based perturbation experiments} We report the test AUC on Last.FM and MovieLens-20M}
% \label{tab:results:reco}
% \scalebox{0.65}{
% \begin{tabular}{lcccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{4}{c}{ \textbf{Last.FM}}&\multicolumn{4}{c}{ \textbf{MovieLens 20M}}\\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%     & \multicolumn{2}{c}{ \textbf{Semantic Perturbation}}&\multicolumn{2}{c}{ \textbf{Structure Perturbation}} &\multicolumn{2}{c}{ \textbf{Semantic Perturbation}} &\multicolumn{2}{c}{ \textbf{Structure Perturbation}}\\
%     \cmidrule(lr){2-3}
%     \cmidrule(lr){4-5}
%     \cmidrule(lr){6-7}
%     \cmidrule(lr){8-9}
%     & AUC & Emb/CC/DC &  AUC & Emb/CC/DC & AUC & Emb/CC/DC  & AUC & Emb/CC/DC \\
%     \midrule
%     {w/o KG $^{\dagger}$} & ~50.75 & -/-/- & ~50.75 & -/-/- & ~91.30 & -/-/- & ~91.30 & -/-/- \\
%     \midrule
%     {KGCN w KG} & 55.99 & 0.97/-/- & 55.97 & 0.97/-/- & 96.62 & 0.96/-/- & 96.62 & 0.96/-/- \\
%     {KGCN- Heuristic1} & 55.98 & 6.8E-1/-/9.7E-1 & 55.96 & 9.4E-1/-/3.6E-1 & 96.62 & 6.8E-1/-/1.8E-1 & 90.36 & 9.3E-1/-/3.1E-2 \\
%     {KGCN- Heuristic2} & 55.98 & 4.2E-1/-/3.4E-1 & 56.04 & 4.4E-1/-/4.2E-1 & 96.50 & 4.1E-1/-/1.2E-1 & 96.24 & 6.8E-1/-/7.3E-2 \\
%     {KGCN- RL} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \midrule
%     {RippleNet w KG} & 56.23 & 0.95/-/- & 56.23 & 0.95/-/- & 97.46 & 0.96/-/- & 97.46 & 0.96/-/- \\
%     {RippleNet- Heuristic1} & 56.23 & 7.8E-1/-/9.6E-1 & 56.21 & 9.4E-1/-/3.6E-1 & 97.46 & 6.1E-1/-/1.7E-1 & 97.43 & 9.3E-1/-/3.1E-2 \\
%     {RippleNet- Heuristic2} & 56.22 & 4.9E-1/-/3.4E-1 & 52.22 & 7.8E-1/-/4.2E-1 & 97.45 & 4.5E-1/-/1.3E-1 & 93.62 & 7.9E-1/-/7.6E-2 \\
%     {RippleNet- RL} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*}



% \begin{table*}[t]
% \centering
% \scalebox{0.70}{
% \begin{tabular}{lcccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{3}{c}{ \textbf{RN with Bert-base}}&\multicolumn{3}{c}{ \textbf{GN with Bert-base}}\\
%     \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%      & Heuristic1 & Heuristic2  & RL & Heuristic1 & Heuristic2 & RL \\
%     % \midrule  
%     % {w/o KG}  & ~($\pm$)  &  .~($\pm$.)  &  52.30~($\pm$0.16) & 55.39~($\pm$0.40) & 65.56~($\pm$0.76) & 68.69($\pm$0.56) \\
%     \midrule
%     {Embedding based Val Score}  &  0.891 &  0.678  &  0.6842 & 0.891 & 0.6785 & .~($\pm$.) \\
%     {Structure based Val Score} & 18e-05  &  12e-05  &  9.54e-05 & 18e-05 & 12e-05 & .~($\pm$.) \\
%     {Dev Acc}  & 57.8 & 56.18 & 56.92 &  57.65 & 56.1 & .~($\pm$.) \\
%     {Test Acc}  & 56 & 54.15 & 55.84 &  57.05 & 57.05 & .~($\pm$.)\\
%     % {RN + Link Prediction}  & .~($\pm$.) & .~($\pm$.) & 53.96~($\pm$0.56) &  56.02~($\pm$0.55) & 66.29($~\pm$0.29) & 69.33~($\pm$0.98)\\
%     % {KagNet$^{\dagger}$~\citep{lin2019kagnet}}  &  .  &  56.19  &  . & 57.16 & - & - \\
%     % {GN}  & .~($\pm$.) & .~($\pm$.) & .~($\pm$.) &  .~($\pm$.) & 69.24($~\pm$0.56) &
%     % 72.12~($\pm$0.45)\\
%     % \midrule
%     % {Hybrid GN without edge weights} & .~($\pm$.) & \textbf{.}~($\pm$.) & .($\pm$.) &  \textbf{.}~($\pm$.)  & 70.46~($\pm$0.81)   & 72.76~($\pm$1.02)  \\
%     % {Hybrid GN with Pruning} & .~($\pm$.) & \textbf{.}~($\pm$.) & .($\pm$.) &  \textbf{.}~($\pm$.)  & 70.13~($\pm$0.82)   & 72.82~($\pm$0.89)  \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \caption{\textbf{Performance comparison on OpenBookQA official split for semantic based perturbation.} We report test accuracy using the official data split on OpenBookQA.}
% \label{tab:results:csqa}
% \end{table*}
% \begin{figure}[h]
% \subfigure[Val score during eval]{
% \includegraphics[width=0.45\textwidth]{val_score.JPG}
% %\caption{val score during eval}
% }
% \subfigure[Loss during training of DQN(Vanilla)]{
% \includegraphics[width=0.45\textwidth]{loss_DQN.JPG}
% %\caption{loss during training of DQN(Vanilla)}
% }

% \subfigure[Accuracy on 400-size dev set during evaluation]{
% \includegraphics[width=0.45\textwidth]{acc.JPG}
% %\caption{loss during training of DQN(Vanilla)}
% }
% \caption{Plot of results.}
% \end{figure}

\begin{figure}[ht!]\label{fig:heur_curvesKGCN}
\centering
\subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_AUC_Music.png}}
\subfloat[][Emb Val Score]{\includegraphics[width=0.25\textwidth]{figures/Relation_Val_score_music.png}}
\subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Edge_AUC_Music.png}}
\subfloat[][Degree Val Score]{\includegraphics[width=0.25\textwidth]{figures/Edge_Val_score_music.png}}
\caption{Variation of Performance and Validation Scores with scale of perturbation on KGCN with Last.FM}
\end{figure}

\begin{figure}[ht!]\label{fig:final_curves}
\centering
\subfloat[][Test Acc on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Rel_Acc_MHGRN.png}}
\subfloat[][Emb Val Score]{\includegraphics[width=0.25\textwidth]{figures/Rel_Val_Score_MHGRN.png}}
\subfloat[][Test Acc on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Edge_Acc_MHGRN.png}}
\subfloat[][Degree Val Score]{\includegraphics[width=0.25\textwidth]{figures/EDGE_val_MHGRN.png}}
\caption{Variation of Performance and Validation Scores with scale of perturbation on MHGRN with CSQA}
\end{figure}

==> backup/backup_Nov15/7_related_work.tex <==
% !TEX root = main.tex

\vspace{-0.1cm}
\section{Related Work}
\label{sec:related-work}
\vspace{-0.1cm}


\textbf{KG-Augmented Models \hspace{1mm}} For various downstream tasks, KGs are commonly used to improve performance by augmenting machine learning models with external knowledge. In fact, the successes of pretrained language models (LMs) in natural language processing (NLP) have been hypothesized to stem from such LMs' ability to probe a latent knowledge base \citep{petroni2019language}. In the past, KGs have been used in various tasks such as commonsense QA \citep{lin2019kagnet,Shen2020ExploitingSK,Lv2020GraphBasedRO,musa2019answering}, recommender systems \citep{wang2019knowledge,Wang2020ReinforcedNS,Song2019ExplainableKG,cao2019unifying}, NLI, \citep{wang2019improving} and many others \citep{Chen2019KnowledgeawareTE,kapanipathi2020infusing}, greatly boosting KG-augmented model performance compared to non-KG methods. KGs have also been regarded as an important way to make the model more interpretable and generate explanations \citep{lin2019kagnet,Zhang2019InteractionEF,Song2019ExplainableKG,cao2019unifying,gao2019explainable,ai2018learning}.

\textbf{Adversarial Perturbation of Graphs \hspace{1mm}}
% \xiang{@Mrigank, include more related work and refs on this line and summarize them at very high level.}
Inspired by adversarial learning in computer vision and NLP, there have been many recent works investigating adversarial perturbations in the graph learning framework \citep{chen2020survey}. Like our work, these works also involve perturbing a graph, although their purpose for doing so is different. Whereas existing works primarily aim to adversarially perturb the graph minimally while having maximum impact on performance, our goal is to use graph perturbations to analyze the faithfulness of NSKG models in using KG information. A variety of paradigms have been proposed for perturb the graph, including gradient-based methods \citep{chen2018fast, bojchevski2019adversarial, wu2019adversarial}, RL-based methods \citep{ma2019attacking, dai2018adversarial}, and autoencoder-based methods \citep{chen2018fast}. Moreover, few existing works on graph perturbations have considered heterogeneous graphs like KGs. \citet{ma2019attacking} use an RL-based adversarial perturbation policy, but they only consider homogeneous graphs in their framework. Meanwhile, our work considers a KG, which is naturally heterogeneous. To the best of our knowledge, this is the first work to use graph perturbations for analyzing the faithfulness of NSKG models in using KG information and providing explanations.

==> backup/backup_Nov15/8_conclusion.tex <==
% !TEX root = main.tex
\vspace{-0.1cm}
\section{Conclusion}
\vspace{-0.1cm}
In this paper, we analyze the effects of strategically perturbed KGs on the predictions of NSKG models. With both simple heuristics and learned RL policies, we show that KGs can be perturbed in way that drastically changes their semantics and structure, while still preserving the model's downstream performance. Furthermore, we conduct a user study to demonstrate that these high-performing perturbed KGs simultaneously provide unfaithful explanations of the model's predictions.
%Further research can be done on coming up with neuro symbolic models that capture the semantics of the KG more faithfully and also can generate faithful explanations for a prediction. 

==> backup/backup_Oct22/1_introduction.tex <==
% !TEX root = main.tex
\section{Introduction}
\vspace{-0.1cm}

%%% 1st paragraph: neural-symbolic models which incorporate symbolic structures from external knowledge graph are gaining growing popularity. 
% --> what are these models like in general?
% --> they are gaining popularity because: 1) improved accuracy on downstream tasks (e.g., overcoming data sparsity in recommendation; augmenting with commonsense knowledge in QA); and 2) these structures, in conjunction with the learn attention weights, are claimed to help provide explanation of model predictions. [Cite papers that claiming the above points].
%%

% Aaron
Recently, neural reasoning over symbolic knowledge graphs (KGs) has emerged as a popular paradigm for various machine learning tasks, such as question answering (QA) ~\citep{lin2019kagnet, feng2020scalable, Lv2020GraphBasedRO}, recommender systems~\citep{wang2018ripplenet, wang2019aknowledge, wang2019knowledge}, and natural language inference~\citep{kapanipathi2020infusing, wang2019improving}. 
For a given data instance, such neural-symbolic KG (NSKG) methods extract a relevant subgraph from the KG, use a neural network to encode the subgraph -- either via message passing ~\citep{wang2018ripplenet,wang2019aknowledge} or path pooling~\citep{lin2019kagnet,feng2020scalable} -- then use the subgraph encoding to make a prediction. 
This incorporation of KG information has been shown to improve performance on a number of downstream tasks: for QA, the KG provides additional context about how a given answer choice is related to the question~\citep{talmor2018commonsenseqa}; for recommender systems, the KG mitigates data sparsity and cold start issues~\citep{wang2018shine}.
Besides improving performance, the KG can also be used to help explain the model's predictions, through inspection of high-scoring reasoning paths~\citep{feng2020scalable, lin2019kagnet, cao2019unifying, gao2019explainable}.

% Recently the neural-symbolic models which  incorporate symbolic structures from external knowledge graphs (KGs) are gaining growing popularity in machine learning tasks such as recommender systems~\citep{wang2018ripplenet, wang2019aknowledge, wang2019knowledge}, question answering~\citep{lin2019kagnet, feng2020scalable, Lv2020GraphBasedRO}, and natural language inference~\citep{kapanipathi2020infusing, wang2019improving}. 
% A typical KG-augmented (neural-symbolic) model either leverages the encoding of the grounded relational structures as additional input features~\citep{lin2019kagnet,feng2020scalable}, or models the relational connections in KG to propagate information among the entities (\textit{i.e.}, message passing)~\citep{wang2018ripplenet,wang2019aknowledge}. 
% By doing so, these methods successfully improve the performance on downstream tasks by bringing symbolic knowledge which is essential yet absent in the input as in commonsense reasoning tasks~\citep{talmor2018commonsenseqa}, or help to address data sparsity and cold start issues as in recommender systems~\citep{wang2018shine}.
% In addition to enhancing model performance, such symbolic knowledge, together with its learned (attention) weights, are used as explanations for the model predictions~\citep{feng2020scalable, lin2019kagnet, cao2019unifying, gao2019explainable}, providing ``insights" to practitioners for understanding the reasoning process.



%%% 2nd paragraph: 
% 1) should start the paragraph with "we question whether the symbolic structures from KG (together with the associated weights) necessarily indicate the model's predictions and enhance the performance." 
% 2） and then bring out the pilot study with these simple heuristics. The main focus should be on faithfulness of the explanation (we also will include human evaluation and those are direct proof; pls stress on that).
% 3) the performance drop is a secondary claim. Please follow the abstract narrative.

% Aaron
Despite the vast KG literature and increasing prevalence of NSKG models, the process in which NSKG models reason about KG information is still not well understood. When solving a reasoning task with a KG, a human might intuitively base their predictions on semantically faithful chains of entities and relations in the KG \citep{feng2020scalable, lin2019kagnet,Song2019ExplainableKG,gao2019explainable}. Meanwhile, it is assumed that NSKG models perform a similar reasoning process and that this process is responsible for the KG-associated performance gains. In this paper, we challenge this assumption and question whether existing NSKG models actually use KGs in a faithful manner. We study this question primarily by measuring model performance with respect to increasing amounts of KG perturbation. To perturb the KG, we propose several simple perturbation heuristics as well as a more powerful reinforcement learning (RL) perturbation model, which is trained to maximize the semantic distance between the original and perturbed KGs as well as the downstream performance when using the perturbed KG. Whereas the heuristic-based perturbations are the same for every model and dataset, the RL-based perturbations are tailored to the given model-dataset setting. Surprisingly, we find that the KG can be extensively perturbed with little effect on model performance, thus yielding unfaithful explanations and raising doubts about the role of the KG in current NSKG models.


% Our pilot study applies simple heuristics to perturb all the edges and relations in the KG.
% % and see whether a well-trained KG-augmented model would have significant performance drop. 
% In some cases, despite a deceptive symbolic structure, which completely deviates from the original KG, we observe that existing models still manage to maintain their performance on downstream tasks. For cases where model performance has noticeable drops, our human evaluation on the model explanation shows that the perturbed structure does not provide faithful explanations. 


% Due to the increased usage of neuro-symbolic models for various tasks, it is of paramount importance  to analyze the structures  learned by these models. In this paper, we question whether the KG structures associated with the data instances provide faithful explanation for the model's predictions and information carried by these structures--\textit{i.e.}, relations and connections between entities--necessarily contribute to the performance improvement on the models.
% Through a series of experiments on diverse tasks and KG-augmented models, we show that one can manipulate the KG structures without significant impact on the performance of the model, yielding deceptive model explanation and raising doubts on what information from the KG are actually captured.
% %
% Our pilot study applies simple heuristics to perturb all the edges and relations in the KG.
% % and see whether a well-trained KG-augmented model would have significant performance drop. 
% In some cases, despite a deceptive symbolic structure, which completely deviates from the original KG, we observe that existing models still manage to maintain their performance on downstream tasks. For cases where model performance has noticeable drops, our human evaluation on the model explanation shows that the perturbed structure does not provide faithful explanations. 


% On other cases, however, we observe noticeable performance drop for the models, indicating that a more targeted perturbation is necessary.
%Using these heuristics we try to challenge the faithfulness of the interpretations generated by the models. We also perform a user study to show the unfaithful explanations generated for a prediction by the models. There are some models that have a drastic performance drop with simple heuristic perturbations.



%%% 3rd paragraph: We need a paragraph to talk about:
% 1）what is our proposed method for solving the remaining issue in previous paragraph, and thus motivate the RL policy learning. 
% 2) And briefly introduce the solution idea of the proposed method

%In our pilot studies we observe a drastic performance drop of a recent KG-augmented model, MHGRN~\citep{feng2020scalable} on the commonsense QA task. 
% \xiang{1. this paragraph needs expansion and polishing; 2. we need leading sentence to make transition from the prior paragraph --- to give motivation on why we need such learning-based approach.}
% For these cases, we question whether a more sophisticated policy can be applied to deceive such specific KG models and maintain the performance on downstream tasks with large perturbations. To this end, we propose a reinforcement learning (RL) based perturbation algorithm and show the existence of such policies. 


% The preliminary results indicate that KG can be easily manipulated and lost its benefit. It brings more worrisome scenario that KG is perturbed in a more systematic way so that even advanced KG-augmented models can be deceived by such a perturbed KG without noticeable performance drop. To show the feasibility of such perturbation policies, we conduct a more sophisticated study where we propose a reinforcement learning (RL) based perturbation algorithm. We leverage the Deep Q-network (DQN) to model the change of downstream task performance given specific perturbation actions, and restrict the agent's action space to ensure nearly maximal perturbation. In this way, the agent learns a perturbation policy with a dual objective of maximally perturbing the graph but maintaining the original accuracy. We show that the agent learns to identify which edges or relations in the KG to perturb while preserving the competitive performance of these KG-augmented models. %compared with non-KG baselines.
% Unlike the heuristic methods, the RL agent can be tailored to a certain KG-augmented model by making use of its performance change as the training signal, and thus yield a perturbed graph with less structural and semantic information and a better performance compared with heuristic methods. %manage to learn deceptive symbolic structures which enable it to perform better than non KG baselines. 
%Both studies indicate that KG is not being leveraged appropriately, and the interpretations generated by the models cannot be relied upon.



%%% 4th paragraph: 1) summary of our exps and findings; 2) discuss about the implications/insights we could give to the community.

% Aaron
Our contributions can be summarized as follows: \textbf{(1)} We introduce four KG perturbation heuristics, which entail different ways to reassign relation types and edge connections in the KG. \textbf{(2)} We propose two RL-based KG perturbation models, which are trained to reassign relation types and edge connections such that both original-to-perturbed semantic distance and downstream performance are maximized. \textbf{(3)} Across two downstream tasks (commonsense QA, recommender systems), four datasets (CSQA, OBQA, Last.FM, MovieLens-20M), and four NSKG models (RN, MHGRN, KGCN, RippleNet), we demonstrate that NSKG models are largely able to maintain their original performance even when the KG has been significantly perturbed to the point that humans struggle to read or use it. To the best of our knowledge, this is the first work to analyze the effects of targeted KG perturbations on NSKG model performance.         


% \xiang{this paragraph needs more revision.}
% In summary, our main findings and contributions are as follows: (1) \textbf{Knowledge Graph Perturbation Framework:} 
% We study perturbations to the knowledge graph along two dimensions, \emph{semantically} by randomization of the relation types while holding the distribution of those types to be the same (and therefore controlling for the different factors), and \emph{structure-based perturbations} that changes the connections in the knowledge graph.
% (2) \textbf{RL-based Targeted Perturbation:} We demonstrate that on some tasks it is non-trivial to achieve our goal of perturbing a KG while maintaining downstream performance with simple perturbations. Therefore we present RL-based perturbation policy learning to maximally perturb the graph while trying to maintain the downstream performance.
% % summarize the main finding maybe?
% (3) We find via our experiments that even with a KG that is corrupted by a sizeable amount, we are able to maintain the downstream performance on most tasks. Through our different types of perturbations and human evaluation, we demonstrate how faithful are the explanations generated by  KG-augmented models and how much are the models sensitive to changes in the KG. 
% To the best of our knowledge this is the first work that deals with the analysis of graph augmented models using targeted perturbations. 


==> backup/backup_Oct22/2_background.tex <==
% !TEX root = main.tex

% \xiang{Need an illustrative figure in 2nd/3rd page for the problem setup and proposed approach @Mrigank.}

% \section{Deceiving KG-Augmented Models by Graph Perturbation}
\section{Problem Setting}
\vspace{-0.2cm}
% \xiang{I envision this section to given overview of our work by defining the problem and laying out some background context. Regarding this, in current writing we're missing: 

% 1) more formal problem definition (after introducing the necessary concepts and notations); should be in the first paragraph. @Mrigank, I recall that you had some formulation in your slides earlier.

% 2) in current writing there is no mention of ``explanation" or ``interpretability" by the KG structures used in these models. This is a critical point and should be well introduced, with notations.

% 3) an overview of the rest of the paper after this section (should be a short paragraph at the end of this section.)}

% Aaron
Our goal is to investigate: \textbf{(A)} whether NSKG models faithfully use KGs for making predictions and \textbf{(B)} whether KGs facilitate sensible explanations of model predictions. For \textbf{(A)}, across various perturbation techniques, we measure model performance as a function of the number of KG perturbations applied. If a KG has been perturbed to the point where even humans have difficulty understanding it, then a faithful NSGK model should not be able to use this perturbed KG to achieve high performance on downstream tasks. For \textbf{(B)}, we ask human subjects to rate original and perturbed KGs with respect to readability and usability for solving downstream tasks. If a KG receives higher ratings, then it is more likely to provide sensible explanations.      

\paragraph{Notation} Let $\mathcal{F}_{\theta}$ be an NSKG model, and let $(X_{train}, X_{dev}, X_{test})$ be a dataset for some downstream task. We denote a KG as $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$, where $\mathcal{E}$ is the set of entities (nodes), $\mathcal{R}$ is the set of relation types, and $\mathcal{T}=\{(h,r,t) \hspace{1.5mm} | \hspace{1.5mm} h,t \hspace{-0.5mm} \in \hspace{-0.5mm} \mathcal{E}, \hspace{1mm} r \hspace{-0.5mm} \in \hspace{-0.5mm} \mathcal{R}\}$ is the set of facts (edges) composed from existing entities and relations. Let $\mathcal{G}^{'}=(\mathcal{E},\mathcal{R},\mathcal{T}^{'}), \hspace{1mm} \mathcal{T}^{'} \hspace{-1mm} \neq\mathcal{T}$ be the KG obtained after perturbing the edges in $\mathcal{G}$. Let $f(\mathcal{G},\mathcal{G}^{'})$ be some function that measures the semantic distance between $\mathcal{G}$ and $\mathcal{G}^{'}$. Let $g(\mathcal{G})$ be the downstream performance when evaluating $\mathcal{F}_{\theta}$ on $X_{test}$ and $\mathcal{G}$. Furthermore, let $\oplus$ denote the concatenation operation and $\mathcal{N}_L(e)$ denote the set of $L$-hop neighbors for entity $e\in\mathcal{E}$.

\paragraph{High-Level Procedure} First, we train $\mathcal{F}_{\theta}$ on $X_{train}$ and $\mathcal{G}$, then evaluate $\mathcal{F}_{\theta}$ on $X_{test}$ and $\mathcal{G}$ to get the original performance $g(\mathcal{G})$. Second, we freeze $\mathcal{F}_{\theta}$, then perturb $\mathcal{G}$ to obtain $\mathcal{G}^{'}$. Third, we evaluate $\mathcal{F}_{\theta}$ on $X_{test}$ and $\mathcal{G}^{'}$ to get the perturbation performance $g(\mathcal{G}^{'})$. Therefore, our perturbation objective can be formalized as: 
\vspace{-3mm}
\begin{equation}
\mathcal{G}^{*}=\argmax_{\mathcal{G}^{'}} \hspace{1mm} f(\mathcal{G},\mathcal{G}^{'}) + g(\mathcal{G}^{'}).
\end{equation}
\vspace{-3mm}

In this paper, we consider two downstream tasks: commonsense QA and recommender systems. Each task has its own specific settings and models, which are described in the rest of this section.

%%%
% We aim to investigate whether KGs are being leveraged appropriately by the KG-augmented models. A KG is denoted as $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$, where $\mathcal{E}$ and $\mathcal{R}$ are the entity set and relation set respectively. It consists of a set of relational edges $\mathcal{T}=\{(h,r,t)|h,t\in\mathcal{E},r\in\mathcal{R}\}$. Let $\mathcal{N}_L(e)$ denote the set of L-hop neighbors for the entity $e\in\mathcal{E}$. Let $\mathcal{G}^{'}=(\mathcal{E},\mathcal{R},\mathcal{T}^{'}),\mathcal{T}^{'}\neq\mathcal{T}$ be a perturbed version of $\mathcal{G}$.
% We define a KG evaluation metric function $f(\mathcal{G},\mathcal{G}^{'})$ which quantifies how much relational information in the KG is \textit{preserved} after perturbation. We further define a performance measurement function $g(\mathcal{G},\mathcal{G}^{'})$ which quantifies the difference in a model's performance, \textit{e.g.}, accuracy on the downstream task. 
% Our goal (\textit{i.e.}, deceiving KG-augmented models) is to identify a \textit{perturbed} KG, $\mathcal{G}^{'}$, which maximally deviates from the original KG, $\mathcal{G}$; while minimally affecting the downstream performance of the KG-augmented model. This perturbation can be formalized into the following objective. 
% \vspace{-0.2cm}
% \begin{equation}
% \mathcal{G}^{*}=\argmin_{\mathcal{G}^{'}} f(\mathcal{G},\mathcal{G}^{'})+g(\mathcal{G},\mathcal{G}^{'}).
% \end{equation}
% In specific, the KG-augmented model is well-trained on $\mathcal{G}$ to get the original performance and fixed. Later the model is tested on $\mathcal{G}^{'}$ to get its performance after perturbation.
%We aim to investigate whether KGs are being leveraged appropriately by the KG-augmented models. 
%We conduct such an investigation through perturbing the underlying KGs of these models to a large extent while still preserving their competitive performance. Formally, a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$, where $\mathcal{E}$ and $\mathcal{R}$ are the entity set and relation set respectively, consists of a set of relational edges $\mathcal{T}=\{(h,r,t)|h,t\in\mathcal{E},r\in\mathcal{R}\}$. We perturb the \textbf{semantic} of KG by revising the relation type (\textsection\ref{}) as well as the graph \textbf{structure} by deleting/rerouting the edges (\textsection\ref{}) for a subset of $\mathcal{T}$  under the guidance of our proposed RL algorithm (\textsection\ref{}). By doing so, we cast doubt on whether the KGs truly contribute to the improvement brought by the models in a way we expect them to and thus raise the researchers' awareness in this field that KGs are not fully utilized. 
% In this work, we look into two different tasks across different domains, \textit{e.g.}, commonsense question answering (QA) and recommender system, as introduced in the rest of this section. %since KGs are shown to be helpful empirically for both tasks by recent works~\cite{}. For each task, we introduce respectively their problem setting and how KGs are leveraged to solve the tasks in the following.
%as well how knowledge is encoded by different kinds of graph encoder respectively in \textsection\ref{sec:task}. We then depict two typical graph encoders that the KG-augmented models adopt to encode the knowledge from a KG in \textsection\ref{}.

% \textbf{Commonsense Question Answering.}
\paragraph{Commonsense QA}
% \label{sec:csqa}
% \vspace{-0.3cm}
% Aaron
Given a question $q$ and a set of $k$ possible answers $\mathcal{A} = \{a_{1}, ... , a_{k}\}$, the task is to predict a plausibility score for each answer, such that the highest score is predicted for the correct answer. In commonsense QA, the questions are designed to require commonsense knowledge which is typically unstated in natural language, but more likely to be found in KGs. 

Given KG $\mathcal{G}$, let $\mathcal{E}_{(q,a)}\subset\mathcal{E}$ be the set of all entities mentioned in the text sequence $q \oplus a$, and let $\mathcal{T}_{(q,a)} \subset \mathcal{T}$ be the set of all edges connecting the entities in $\mathcal{E}_{(q,a)}$. Following \citet{lin2019kagnet} and \cite{feng2020scalable}, for each question-answer pair $(q, a)$, we first use off-the-shelf string matching tools to extract $\mathcal{E}_{(q,a)}$ from $q \oplus a$. Next, from $\mathcal{G}$, we construct a subgraph $\mathcal{G}_{(q,a)}$, which consists of $\mathcal{E}_{(q,a)}$ and $\mathcal{T}_{(q,a)}$.

Recall that the NSKG model is denoted as $\mathcal{F}_{\theta}$. For this task, let $\mathcal{F}_{\phi}^{text}$ be a text encoder, $\mathcal{F}_{\psi}^{graph}$ be a graph encoder, and $\mathcal{F}_{\xi}^{cls}$ be a classifier, where $\phi, \psi, \xi \subset \theta$. We then compute a text embedding $\mathbf{h}_{text} = \mathcal{F}_{\phi}^{text}(q \oplus a)$ and a graph embedding $\mathbf{h}_{graph} = \mathcal{F}_{\phi}^{graph}(\mathcal{G}_{(q,a)})$. After that, we compute the score for $(q,a)$ as $y_{(q,a)} = \mathcal{F}_{\xi}^{cls}(\mathbf{h}_{text} \oplus \mathbf{h}_{graph})$. Finally, we select the highest scoring answer: $a^{*} = \argmax_{a \in A} \hspace{1mm} y_{(q,a)}$ 

Since the graph encoder $\mathcal{F}_{\psi}^{graph}$ plays the critical role of leveraging information from the KG, significant research effort has been devoted to designing better graph encoders. Two common types of graph encoders are graph neural networks (GNNs) and path-based models. GNNs iteratively update each node's embedding by aggregating its neighbor nodes' embeddings, then obtain the graph embedding by pooling the final node embeddings ~\citep{kipf2016semi, schlichtkrull2018modeling}. Path-based models treat the graph as a set of paths, encode each path separately, then obtain the graph embedding by aggregating the path embeddings ~\citep{lin2019kagnet, santoro2017simple}. More recently, MHGRN ~\citep{feng2020scalable} was proposed as a hybrid of GNNs and path-based models, achieving better interpretability, scalability, and performance on commonsense QA benchmarks. In these graph encoders, the aggregation weights computed for $\mathcal{G}_{(q,a)}$ can serve as an explanation for the model prediction.


%\textbf{Problem Setting}. We focus on multi-choice commonsense QA which is the general format for most of the benchmarks in this field. Given a question $q$, a system is required to select one of the choices $\{a\}$ as the answer. The task is on-purposely designed to omit the key background knowledge that leads to the answer, so as to test the system for its understanding of commonsense. 
% Given a question $q$ and a set of choices $\mathcal{C}$, the task requires a system to select one of the choices $a\in\mathcal{A}$ as the answer.
% To tackle the task, the KG-augmented QA systems such as KagNet~\citep{lin2019kagnet} and MHGRN~\citep{feng2020scalable}
% %In response, systems solving these tasks usually resort to some external KG for obtaining knowledge necessary for answering the question. They 
% first extract the set of entities $\mathcal{E}_{(q,a)}\subset\mathcal{E}$ mentioned in the pair of $(q,a)$ with existing entity recognition tools and later construct a sub-graph $\mathcal{G}_{(q,a)}$ containing $\mathcal{E}_{(q,a)}$ and their multi-hop relations in the KG. Then the system encodes the $(q,a)$ pair to a context embedding $\mathbf{c}$ and encodes $\mathcal{G}_{(q,a)}$ to a knowledge embedding $\mathbf{k}$. Finally, both $\mathbf{c}$ and $\mathbf{k}$ are concatenated for calculating the plausibility score. 
% %a general QA framework consisting one context encoder and one graph encoder is adopted to solve the task. The context encoder, which is usually a pre-trained LM~\cite{}, takes as input the QA pair $(q,a)$ and outputs a context embedding $\mathbf{c}$. The graph encoder takes as input the sub-graph and outputs the knowledge embedding $\mathbf{k}$. Both output embeddings are concatenated together as the input to the final classifier that gives a score for a choice: $f(q,a)=\mathbf{w}\cdot[\mathbf{c};\mathbf{k}]+b$.
% The choice with the highest score is selected as the answer.
% %\textbf{Graph Encoders for QA-KG}. 
% Two types of graph encoders are generally adopted to encode $\mathcal{G}_{(q,a)}$ to $\mathbf{k}$ as described below. 

% (1) Graph Neural Networks ~\citep{kipf2016semi,schlichtkrull2018modeling} firstly represent each node by its feature embedding $\{\mathbf{h}^0_i\},i\in\mathcal{G}_{(q,a)}$ and then iteratively update a node's representation  by aggregating its neighbors' embedding, i.e., $\mathbf{h}^l_i=\text{Aggregation}(\{\mathbf{h}^{l-1}_j|j\in \mathcal{N}_1(i)\})$. Finally, a pooling over all the node embeddings is used as the graph representation: $\mathbf{k}=\text{Pooling}(\{\mathbf{h}^{L}_i\})$ with $L$ indicating each node receives information from its neighbors up to $L$ hops. 

% (2) Path-Based Models~\citep{lin2019kagnet,santoro2017simple} treat an input graph as a set of relational paths $\mathcal{P}$ connecting the entities. Then each path $p_i\in\mathcal{P}$ is encoded as an embedding $\mathbf{p}_i$  and further aggregated to obtain the knowledge embedding: $\mathbf{k}=\text{Aggregation}(\{\mathbf{p}_i\})$.

% In both graph encoders, the subgraph $\mathcal{G}_{(q,a)}$ together with the aggregation weights serve as the explanation for the prediction.

\paragraph{Recommender Systems} 
% \vspace{-0.3cm}
%\textbf{Problem Setting}. 

% Aaron
We consider a set of users $\mathcal{U}=\{u_1,u_2,...,u_M\}$, a set of items $\mathcal{V}=\{v_1,v_2,...,v_N\}$, and a user-item interaction matrix $\mathbf{Y}\in\mathcal{R}^{M\times N}$. If user $u$ has engaged with item $v$ before, then $y_{uv}=1$ in the user-item interaction matrix; otherwise, $y_{uv}=0$. Additionally, we consider a KG $\mathcal{G}$, in which $\mathcal{R}$ is the set of relation types in $\mathcal{G}$. In $\mathcal{G}$, nodes are items $v \in \mathcal{V}$, and edges are facts of the form $(v_{i}, r, v_{j})$, where $r \in \mathcal{R}$ is a relation. For the zero entries in $\mathbf{Y}$ (i.e., $y_{uv}=0$), our task is to predict a compatibility score for user-item pair $(u, v)$, indicating how likely user $u$ is to want to engage with item $v$. We represent each user $u$, item $v$, and relation $r$ as embeddings $\mathbf{u}$, $\mathbf{v}$, and $\mathbf{r}$, respectively. Given a pair $(u, v)$, its compatibility score is computed as $\langle \mathbf{u}, \mathbf{v} \rangle$, the inner product between $\mathbf{u}$ and $\mathbf{v}$. 

Two prominent examples of NSKG recommender systems are KGCN ~\citep{wang2019knowledge} and RippleNet ~\citep{wang2018ripplenet}. In KGCN, we first retrieve $\mathbf{u}$ and $\mathbf{v}$ from $\mathcal{G}$'s embedding table, which is learned. Next, a neural network iteratively updates $\mathbf{v}$ by aggregating its subgraph of $L$-hop neighbor embeddings, the corresponding relation embeddings, and $\mathbf{u}$. After $\mathbf{v}$ is done updating, we compute $\langle \mathbf{u}, \mathbf{v} \rangle$. In RippleNet, we retrieve $\mathbf{v}$ from $\mathcal{G}$'s embedding table, which is learned, and set the items $u$ has interacted with as seed nodes. Next, a neural network computes $\mathbf{u}$ via iterative aggregating its subgraph of seed node embeddings, their $L$-hop neighbor embeddings, and the corresponding relation embeddings. After obtaining $\mathbf{u}$, we again compute $\langle \mathbf{u}, \mathbf{v} \rangle$. In both KGCN and RippleNet, the aggregation weights from the subgraph can be used to explain the model prediction.           

% In this task, we consider a set of users $\mathcal{U}=\{u_1,u_2,...,u_M\}$ and a set of items $\mathcal{V}=\{v_1,v_2,...,v_N\}$, as well as their interaction matrix $\mathbf{Y}\in\mathcal{R}^{M\times N}$. An observed interaction ($y_{uv}=1$) indicates that the user $u$ engages with the item $v$ before while
% the task is to predict the unobserved interaction ($y_{uv}=0$).
% The KG-augmented recommender systems assume there exists 
% an item KG which provides bountiful relational connections between the items. They further represent each user and item as embeddings $\mathbf{u}$ and $\mathbf{v}$ and then use their interaction, e.g., inner product for recommending $v$ to $u$. Below we introduce two recent works we investigate in this paper which differ in how they leverage the item KG and represent the users and items.

%\textbf{KG-Augmented Recommendation System}.Recent work on Knowledge Graph augmented Recommendation Systems can be classified into 3 categories namely Embedding based, Path based and Hybrid Models. Embedding based models \citep{huang2018improving,wang2018dkn, wang2019multi} try to learn entity embeddings using a knowledge graph embedding (KGE) techniques and then use these learned embeddings for recommendation. Path based models \citep{hu2018leveraging,yu2014personalized,zhao2018learning} explore the connectivity between different items that can be leveraged for the recommendation task. Embedding based methods focus heavily on the relation types between two entities. In this way using path based models seems a more natural approach for recommendation but these models include finding meta paths/graphs which are not easy to tune in practice. Hybrid models \citep{wang2019knowledge, wang2018ripplenet} try to combine best of both worlds by learning embeddings of an entity based on its local neighbourhood and using these embeddings for the recommendation task. The two well known hybrid models for recommendation systems are described below.


% KGCN~\citep{wang2019knowledge} represents an item as each aggregation over its neighbors in the KG, i.e., $\mathbf{v}=\text{Aggregation}_u(\{\mathbf{v}^{'}|v^{'}\in\mathcal{N}_1(v)\})$, where the aggregation weights are personalized for $u$. This aggregation is repeated $L$ times to obtain information from $L$-hops neighbors (similar to GNN). The user embedding is initialized randomly and learned during training.
%tries to learn a user personalized embedding for the neighbourhood N(v) of a given entity v by weighting the features of the neighbouhood entities with learnable user personalized weights i.e $\mathbf{v_{N(v)}^u} = \sum_{e \in N(v)}^{}\pi_{r_{v,e}}^u\mathbf{e}$ where $r_{v,e}$ is the label of the edge connecting v and e and $\mathbf{e}$ is the embedding for entity e. Then this neighbourhood embedding is aggregated with the the embedding of v and passed thorough non linearities to get a personalized entity embedding $\mathbf{v^u}$ and then use this along with the user embedding $\mathbf{u}$ to get a score for a given user-entity pair.
% In contrast, RippleNet~\citep{wang2018ripplenet} represents each user $u$ as the aggregation over the $L$-hops neighbors of the items $\mathcal{V}_u$ which $u$ has been interacted with before, i.e., $\mathbf{u}=\text{Aggregation}(\{\mathbf{v}|v\in\mathcal{N}_L(v^{'}),\forall v^{'}\in\mathcal{V}_u\})$. The item embedding is initialized randomly and learned during training. In both KGCN and RippleNet, the aggregation weights on the items' neighbors are used to explain the recommendation results.
%tries to learn user embeddings using his/her preferred items. For a given user u, they construct a ripple set of triples that are k hop away from entities in which u is interested. Then they pass messages among the triples in this ripple set and set the embedding \textbf{u} of user u to be the aggregation of these messages. For a user-entity pair they use this learned user embeddings and the entity embeddings to estimate the probability that the given user engages in the given item.  

% \xiang{Need a short paragraph as an overview of the rest of the paper after this section}
% In the rest of the paper, we will first present the pilot study that motivates the work, and then describe the targeted RL perturbation policy that we propose for our analysis. Finally we detail our experimental setup and show our results and analysis that support the claim of the paper.


\begin{figure}[t]
%{0.57\textwidth}
    \centering
\vspace{-0.4cm}
    \includegraphics[width=1.0\textwidth]{figures/pert_kg.pdf}
    %\vspace{-0.4cm}
    \caption{\textbf{Proposed KG perturbation framework.} Given a original KG, we conduct relation/edge perturbation on the KG by either heuristics or our RL algorithm. Then the perturbed graph is fed to a well-trained neural-symbolic model for obtaining prediction and (unfaithful) explanation on the downstream task.}
    \label{fig:pert_framework}
\vspace{-0.4cm}
\end{figure}

% \subsection{Graph Encoders}
% Recently there has been a boom in the research of Graph Representation Learning Models \citep{velivckovic2018graph, hamilton2017representation, hamilton2017inductive,you2019position} but a very few of them can be adapted successfully to heterogeneous graphs such as Knowledge Graphs. To this end we introduce Graph Networks \citep{battaglia2018relational} and Relation Networks \citep{santoro2017simple} which aim to capture the relational information present in Knowledge Graphs.
% \begin{itemize}
%     \item Path Based Models: 
%     \item Message Passing based Models: Details about Graph Networks
% \end{itemize}
% \subsection{Deep Q Networks}
% In this paper we try to leverage Reinforcement Learning to come up with a targeted perturbation policy. We use Deep Q Networks (DQN) to learn the perturbation policy. DQN and its variants have been shown very powerful in playing games, where the policy of agents is trained through the feedback reward from the environment. 
% In this work, we view our perturbation policy as agent, and the downstream task performance as environment. Every time we use our policy to perturb KG for a fixed steps, we will get reward from the environment reflecting how well we maintain the downstream task performance. In this way, we have our policy trained and the DQN will learn a good policy suiting for our purpose.

% In a typical DQN, at each step we will have to feed the embeddings of state to get the approximated Q function. However, in our work, if we directly use a GNN-based model to embed the current KG as state, it will conflict with the purpose of our work, which is to examine the effect of the GNN-based model of KG. Therefore, we alternatively apply a LSTM to represent the state as hidden state, and at the same time form the DQN. The initialized embedding of LSTM is randomized and trainable. At each time step, the LSTM cell takes in the hidden state vector for the current state and the current action we choose, and then it outputs the approximated Q function and the hidden state vector for the next state.


% \begin{itemize}
%     \item Commonsense Question Answering: 
%     \item Recommendation Systems: 
% \end{itemize}

==> backup/backup_Oct22/3_pilot_study.tex <==
% !TEX root = main.tex

\vspace{-0.1cm}
\section{Pilot Study with Simple Perturbation Heuristics}\label{sec: pilotexpts}
\vspace{-0.2cm}

% We conduct our investigation through perturbing the underlying KGs of these models to a large extent and see whther the models can still preserve their competitive performance. We perturb the \textit{semantic} of KG by revising the relation types as well as the graph \textit{structure} by deleting/rerouting the edges for a subset of $\mathcal{T}$. 
As a pilot study to motivate our work, we first consider two simple strategies to perturb the KG: (1) \textbf{Relation Swapping (RS)}: We randomly choose two triples (edges) in the KG and swap their relations. This heuristic changes the semantic of the triples while leaving the underlying connectivity structure unchanged.
%is designed in a way that after perturbing the KG the relation distribution across the KG remains unchanged. It is very important to note here that this heuristic does not change the structure of the graph. It only affects the semantics of the triples in the KG. 
(2) \textbf{Relation Replacement (RR)}: We randomly choose a triple $(h,r_1,t)$ and then replace its relation with another one $r_2$ that yields the most invalid triples, i.e., $r_2=\argminB_{r \in \mathcal{R}}{s_\mathcal{G}(h,r,t)}$ where $s_\mathcal{G}(\cdot)$ is a KG scoring function trained on $\mathcal{G}$.
%we delete the edge $(h,r,t)$ and add $(h,r',t)$  where $r' = \argminB_{r'' \in \mathcal{R}}{f(h,r'',t)}$ and $f(.)$ is a KG completion model. 
%Given a triple, the KG completion model outputs a score to measure how plausible the triple is valid.
This heuristic also does not perturb KG's structure but its semantics. 
%or the connectivity of the graph in any way but it affects the relation distribution across the KG.
% whether the dowtrying to maintain the downstream performance. 





%\subsection{Validation Score}
%Since our aim is to perturb the Knowledge Graph we require a metric to judge the extent to which the graph has been corrupted. Due to the size of the Knowledge Graph it is impractical for humans to evaluate the amount of knowledge in the KG or how much has the KG changed after perturbations on structure as well as semantics.
%To this end we suggest the use of the following two different types of validation scores:

% \ryan{It's unclear why these validation scores are needed. Seems like they are only used to determine how much the graph is corrupted, but don't we already know by definition? 
% For instance, if we perform the relation swapping to 100\% of the edges, then we know that we have completely changed the relations of the graph, while holding the structure the same, and thus controlling for it.
% I sort of understand the use of validation metrics, but wonder if its really needed, it just adds another level of abstraction that we need to somehow explain.
% The fact that we change 100\% of the relations, and measure accuracy should be enough.
% I guess these may be able to help explain the change in accuracy, but in the end, these "validation scores" are heuristics in themselves, and their importance is unclear.
% see some drop performance drop should be enough.
% For instance, if we randomize the relations via the swapping heuristic (applying it enough to fully randomize the relations in the graph).
% then we know for a fact we c 
% }
    % \item Embedding Based Validation Score: This validation score is derived from a Knowledge Base Completion model trained on Conceptnet. We train the embedding based Knowledge base completion architecture as specified in \citep{li-etal-2016-commonsense} on Conceptnet. This model take a triple as input and outputs the probability of the triple being semantically correct. We define the score of a triple to be this probability. We define the validation score of a graph to be the mean of scores of each triple in the graph. A thing to note is that this validation score will fail to capture the structure changes in the graph as will be evident in the experiments section. To alleviate this problem we use another validation score.
    
To quantify to what extent we perturb the KG, we propose an automatic measurement called \textbf{Aggregated Triple Score (ATS)}. 
%This validation score is derived from the Knowledge Base Completion model mentioned above. 
%trained on Conceptnet. We train the embedding based Knowledge base completion architecture as specified in \citep{li-etal-2016-commonsense} on the Knowledge Graph. Given a triple $ t = (e1,r,e2)$, this model outputs the score $f(t)$ of the triple. Larger the score of the triple, more semantically correct the triple should be. 
It is defined as the average scores given by the KG scoring function mentioned above over all the triples present in the KG, i.e., $f^{ATS}(\mathcal{G},\mathcal{G}^{'}) = \frac{1}{|\mathcal{T}^{'}|}\sum_{(h,r,t)\in\mathcal{T}^{'}}s_\mathcal{G}(h,r,t)$. The KG scoring functions used in the paper are \citep{li-etal-2016-commonsense} for Question Answering task and \citep{yang2015embedding} for recommendation tasks. 
%where $\mathcal{G}$ represents the KG and $N$ represents the total number of triples in G. %One thing to note is that deleting edges also leads to a decrease of semantic knowledge in the KG, but it is not captured by this validation score. To alleviate this issue we come up with two more validation scores that we believe are more robust to different types of perturbations.
    
% \textbf{Clustering Coefficient based Validation Score}: We design this validation score in a way that it is robust to structural perturbation to the KG as well as perturbation to the edge types. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$ we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$ i.e $$\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$$
%     where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$
% \ryan{This strategy looks at triangles that are all homogeneous in terms of their relation $r$, what about triangles that are not all of the same relation $r$, but mixed relations? There are typically far more of these, just by chance. But in any case, its unclear why they were ignored. It was probably done since the above way just makes it simple to apply standard algorithms, but hopefully we have a more solid reason and justification for this.}
   
%  We then calculate the relation specific clustering coefficient vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective} of the $i^{th}$ node and calculate the average clustering vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e $$\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$$
% We denote by $\mathbf{c_{o}}$, the average clustering vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{c_{p}}$. We then define the validation score of the KG as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ i.e
% $$V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$$
% with $b$ as a constant for avoiding zero division.
% It is important to note that this validation score is more based on a physical property of the KG namely the clustering coefficient and not some neural embeddings which are hard to interpret. This validation score also robustly captures both changes in relations and the structure of the graph. Another observation is when the KG is very sparse the clustering coefficient values can be very small and may not give us a good idea how much perturbed the graph is. Therefore we define another validation score for our experiments.

% \textbf{Degree Coefficient based Validation Score: } Similar to the clustering coefficient based validation we first create a set of graphs $\mathcal{G}^{r}$ for each relation $r \in \mathcal{R}$. We then calculate the relation specific degree vector $\mathbf{d^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{d^r}$ represents the degree of the $i^{th}$ node and calculate the average degree vector $\mathbf{d}$ for the whole graph as the mean of $\mathbf{d^r}$ over all $r \in \mathcal{R}$ i.e $$\mathbf{d} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{d^r}$$
% We denote by $\mathbf{d_{o}}$, the average degree vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{d_{p}}$. We then define the validation score of the KG as the reciprocal of the L2 distance between $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$ i.e
% \begin{equation}
% V_{dc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{d_{o}} - \mathbf{d_{p}} \rVert_2 + b}.
% \end{equation}
% Similar to the clustering coefficient based validation score, this score is also based on a physical property of the graph namely degree coefficient. Even if the KG is sparse we expect this validation score to gives us a good idea of the extent of perturbation. 
    


% A better name might be "Relation Randomization", randomization is a common method in statistics, and experimental designs, not sure if I'd call it a heuristic.

% We consider one such swapping as two perturbations.


% \begin{align}\label{eq:relation-swapping}
%   &i \sim \text{UniformDiscrete}\{1,2,\ldots,|E|\} \\
%   & j \sim \text{UniformDiscrete}\{1,2,\ldots,|E|\} \\
% %   ,\quad \text{for } j=1,2,\ldots\\
%     &E \leftarrow E \setminus \{e_i=(h,r,t), e_j=(h,r^{\prime},t)\} \nonumber
%     &E \leftarrow E \cup \{e_i=(h,r^{\prime},t), e_j=(h,r,t)\} \nonumber
% \end{align}\noindent


% \ryan{Define formally with equation}

% \textbf{Rewiring Heuristic: } This is a heuristic that we design to alter the structure of the graph but keep the relation distribution across the KG constant. In this heuristic we first select an edge $(h,r,t)$ randomly. We denote by $\mathcal{N}(v)$, the set of neighbors of the node v. Let $k \in \mathcal{E} \setminus \mathcal{N}(h)$. 
% Then:
% \begin{align}\label{rewiring-heuristic}
%     \mathcal{T} \leftarrow \mathcal{T} \setminus \{(h,r,t)\} \cup \{(h,r,k)\}
% \end{align}
 

% \textbf{Deletion Heuristic:} In this heuristic we randomly select an edge and delete it.
% \begin{align}\label{eq:deletion-heuristic}
%   &i \sim \text{UniformDiscrete}\{1,2,\ldots,|\mathcal{T}|\} \\
% %   ,\quad \text{for } j=1,2,\ldots\\
%     &\mathcal{T} \leftarrow \mathcal{T} \setminus \{e_i=(h,r,t)\} \nonumber
% \end{align}\noindent
% This heuristic clearly changes both the structure of the graph as well as the distribution of relations across the KG.
% % This is a heuristic that clearly changes both the structure of the graph as well as the relation distribution across the KG. 
% A very interesting observation should be that the embedding based validation score will fail to recognize these perturbations to the KG by design. Since even if we delete edges the remaining edges are still valid triples of the KG which in turn keeps this validation score almost unchanged.
% \ryan{unclear why it should be.}

% \ryan{Would be easy and nice to show equations for all 4 of the heuristics. I did one above, which can be modified in various ways to appropriately define the other 3.}
% \ryan{
% It is also worth mentioning the connection of Relation Swapping and Rewiring Heuristic with Randomization techniques that are used in controlled experimental designs, e.g., relation swapping 
% Also, if we did relation swapping 100\%, then this would be equivalent to relation randomization, and in that case, it can be thought of as obtaining a random permutation of relations while fixing the graph structure.
% }

% \textbf{Downstream Tasks and Models.}
%To showcase our pilot experiments using simple heuristic methods we demonstrate our results on the following graph encoder:
We conduct our pilot study on both of commonsense QA and recommendation system tasks. For commonsense QA, we adopt MHGRN~\citep{feng2020scalable}, a hybrid of GNN and path-based model, on a commonsense benchmark dataset, CSQA~\citep{talmor2018commonsenseqa}. For recommendation system, we adopt KGCN~\citep{wang2019knowledge} on the Last.FM~\citep{rendle2012libfm} dataset.

%\textbf{MHGRN \citep{feng2020scalable}: } For this experiment we use MHGRN on the CSQA dataset. CSQA is a commonsense question answering benchmark dataset that is derived from conceptnet and is one of those tasks which requires external knowledge in the form of a KG. Since the labels for the official test are not available we report our results on the inhouse test split of \citep{lin2019kagnet}. MHGRN is a recently proposed strong baseline for commonsense question answering that uses multi hop message passing to model relational paths between concept pairs. For this study we use Bert-base as the language model accompanying the graph encoder.

%\textbf{KGCN \citep{wang2019knowledge}: }We also experiment on KGCN on the Last.FM dataset. Last.FM is a music reviews dataset that is used as a benchmark for many recommendation systems. KGCN is a recently proposed strong baseline for recommendation systems. This system uses the Microsoft Satori Knowledge base as the Knowledge Graph. We only use 20\% of the available training data as the use of KG in the recommendation task is justified more under the cold start scenario where we have limited training data. 

% For this experiment we take the complete conceptnet graph and prune it first such that it only contains edges that are relevant for the CSQA dataset i.e for each edge either the head entity or the tail entity is a part of the csqa dataset. We report our results after perturbing 40\% of the pruned KG in table \ref{tab:heur_table} and show curves of how the performance changes with different scales of perturbation in figure \ref{fig:heur_curves}.

% \begin{figure}[ht!]\label{fig:heur_curves_MHGRN}
% \centering
% \subfloat[][Test Acc on MHGRN]{\includegraphics[width=0.25\textwidth]{figures/Rel_Acc_MHGRN.png}}
% \subfloat[][Emb Val Score]{\includegraphics[width=0.25\textwidth]{figures/Rel_Acc_MHGRN.png}}
% \subfloat[][Test Accuracy on CSQA]{\includegraphics[width=0.25\textwidth]{figures/EDGE_val_MHGRN.png}}
% \subfloat[][Degree Val Score]{\includegraphics[width=0.25\textwidth]{figures/Edge_Val_score_music.png}}
% \caption{Variation of Test Accuracy and Validation Scores with scale of perturbation on MHGRN with CSQA}
% \label{fig:heur_curves_MHGRN}
% \end{figure}

% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on heuristics after perturbing 40\% of the KG.} We report test accuracy and the validation scores.}
% \label{tab:heur_table}
% \scalebox{0.80}{
% \begin{tabular}{lcccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \textbf{Test Acc} & $\mathbf{V_{emb}}$ & $\mathbf{V_{cc}}$ & $\mathbf{V_{dc}}$\\
%      &  & & & \\
%     \midrule  
%     {w/o KG}  & 53.47  &  - & - & - \\
%     \midrule
%     % {RN~\citep{santoro2017simple}}  & 65.20~($\pm$1.18)  &  75.35~($\pm$1.39) \\
%     % {RGCN~\citep{Schlichtkrull2017ModelingRD}}  & 62.45~($\pm$1.57) & 74.60~($\pm$2.53) \\
%     % {GconAttn~\citep{Wang2018ImprovingNL}}  & 64.75~($\pm$1.48)  &  71.80~($\pm$1.21) \\
%     {MHGRN w KG}  & 57.45  &  0.94 & - & - \\
%     {MHGRN Relation Swapping}  & 56.19  &  0.891 & 0.225 & 0.013 \\
%     {MHGRN Greedy}  & 54.31  & 0.677& 0.143 & 0.0043 \\
%     % {Hybrid RN}  & .~($\pm$.)  &  .~($\pm$.) \\
%     % {GN}  & .~($\pm$.)  &  .~($\pm$.) \\
%     % \midrule
%     % {MHGRN Greedy}  & .~($\pm$.)  &  .~($\pm$.) \\
%     {MHGRN Rewiring}  & 53.42  & 0.79 & 0.2 & 0.0113\\
%     {MHGRN Deletion}  & 53.5 & 0.934 & 0.179 & 0.0057 \\
%     \bottomrule
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*}
% \begin{multicols}{2}
%         \begin{figure*}[ht!]
%             \includegraphics[width=.3\textwidth]{figures/Emb_Val_Score_RN.png}\hfill
%             \includegraphics[width=.3\textwidth]{figures/test_acc_RN.png}\hfill
%             \includegraphics[width=.3\textwidth]{figures/New_val_RN.png}
%             \caption{Image A.}
%             \caption{Image B.}
%             \caption{Image C.}
%         \end{figure*}
%     \end{multicols}
\begin{figure}[tb!]
\vspace{-0.6cm}
\centering
\subfloat[][Test Accuracy on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Rel_Acc_MHGRN.png}}
\subfloat[][ATS on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Rel_Val_Score_MHGRN.png}}
\subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_AUC_Music.png}}
\subfloat[][ATS on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_Val_score_music.png}}
\vspace{-0.1cm}
\caption{Variation of Performance and Evaluation Metrics with scale of perturbation on KGCN with Last.FM and MHGRN with CSQA.  \xiang{polish and enrich caption.}}
\vspace{-0.1cm}
\label{fig:heur_curves}
\end{figure}
\textbf{Observations and Discussion.}
% We observe that the out of all the heuristics we suggested only the relation swapping heuristic was able to maintain the test accuracy of the downstream model somewhat. But when we look at the validation scores we notice that the relation swapping heuristic was unable to perturb the graph to a large extent and thus we cant conclude that relation swapping heuristic achieved our aim. For the rest of the heuristics, we notice that the KG is indeed perturbed to a large extent but there is $\approx 3\%$ drop in performance. Thus this set of experiments exhibit the fact that our aim of perturbing the KG to a large extent while preserving the performance cannot be accomplished with simple heuristic methods and motivate us to pursue a Reinforcement Learning strategy to learn a targeted perturbation policy.
We show curves of how the performance and the ATS metric change across different percentages(of total number of edges in the KG) of relation-based perturbations in Figure~\ref{fig:heur_curves}. We observe that simple heuristics are able to perturb the KG to a large extent (Figure~\ref{fig:heur_curves}-b) while maintaining the performance in the recommendation task (Figure~\ref{fig:heur_curves}-a). This casts doubt on the faithfulness of the symbolic knowledge for KGCN and motivates us to investigate other neural-symbolic models as well. %We know that if we do large number of unique relation swapping we will get a KG with random relations. The fact that in spite of having a KG with random relations the performance is not impacted motivates us to analyze more such models. 

On the contrary, for MHGRN with CSQA we observe that indeed randomization of relations of the KG leads to a clear drop in performance (test accuracy), as shown in Figure~\ref{fig:heur_curves}-c. To further examine whether random noise could yield similar performance drop as simple heuristics do, we design three controlled noisy baselines where we replace the subgraph embeddings for each instance from MHGRN with (1) zero vectors, (2) random vectors or replace the entities and relation embeddings with random vectors. By doing so, the model achieves $53.99\%$, $52.48\%$ and $54.03\%$ in accuracy respectively, indicating that the simple heuristics just yield some meaningless knowledge embeddings.
Since this is due to the fact that simple heuristics perturb KG blindly, we ask the question whether we can maintain the performance while corrupting a KG with some sophisticated perturbation policies. To this end in the next section we propose a RL based perturbation policy.
%to see whether we can maintain performance on MHGRN with CSQA even with a corrupted graph. We also do more analysis on other Recommendation and Commonsense Question Answering models. 

% \textbf{Human Evaluation on Model Explanation.} We manually evaluate the quality of the model explanation after the perturbations...
% \xiang{placeholder for the study on interpretability.}

==> backup/backup_Oct22/4_method.tex <==
% !TEX root = main.tex

\vspace{-0.1cm}
\section{Policy Learning for Targeted KG Perturbation}
\vspace{-0.3cm}

% \xiang{Need update to only talk about the relation perturbation policy and reward design.}

In this section we introduce our targeted perturbation policy which learns to maximally perturb the graph while maintaining the performance on the downstream task. The policy can be trained to perform either relation perturbations i.e. changing the relations of edges in the knowledge graph, or edge perturbations i.e. changing the target node of an edge in the graph.
%Another is structure perturbation, i.e., replacing the edges. %We try to perturb the semantics and the structure of the graph separately to see the effect of different attributes of the graph on the downstream tasks.
To achieve this goal, we adopt Deep Q-networks (DQN)~\citep{mnih2015human}, a deep RL algorithm to learn the target policy. We model the perturbation procedure as a Finite Horizon Markov Decision Process $(S, A, P, R, \gamma)$, where $S$ is the state space,  $A$ is the action space, $P$ is the transition probability, $R$ is the reward function and $\gamma$ is the discount factor. With this setting, DQN aims at learning an approximated Q function $Q(s_t, a_t) $ for state $s_t$ and action $a_t$ at step $t$. The detailed definitions are as follows. 

\begin{figure}
%{0.5\textwidth}
    %\vspace{-0.6cm}
    \centering
\includegraphics[width=0.95\textwidth]{figures/dqn.pdf}
%\vspace{-0.5cm}
    \caption{\textbf{The proposed DQN architecture for targeted KG perturbation.} The table in the left shows the corresponding subactions instantiated by relation/edge perturbation. The figure in the right shows the unified DQN framework for both relation and edge perturbations.  \xiang{further enrich caption.}}
    \label{fig:model_figure}
    \vspace{-0.5cm}
\end{figure}


\textbf{States. }
The state space $S$ consists of all the possible $\mathcal{G}$ that can be obtained via our perturbation. For relation perturbation, the structure of the graph remains unaltered, hence the state space is all the graphs with the same structure as the original graph. For edge perturbations, the structure of the graph is changed but the distribution of the relations remain the same. So the state space here would be the set of all possible graphs with the same relational distribution. 
%For structure perturbation, %the structure of the graph is changed, but the relation distribution is maintained, so 
%the state space is all the graphs whose outward edges for each entity are the same as the original graph. 

The DQN requires the embeddings $s_t$ of the current state \begin{small}$\mathcal{G}_t$\end{small} as input. A common approach to represent the current state is by GNN-based graph encoder \begin{small}$s_t=\text{GNN}(\mathcal{G}_t)$\end{small}. However, such method is not suitable for our task, since one of our goal is to examine whether these graph encoders have captured the information of KG. Thus it will conflict with our goal if we use our questioned object in our examining method. Therefore, we alternatively leverage a LSTM \citep{hochreiter1997long} for the state embedding. At each step, we feed the embedding of the chosen action $a_t$ into LSTM, and then the perturbed graph is represented by the output hidden vector of LSTM, \textit{i.e.}, \begin{small}$h_t=\text{LSTM}(s_0, [a_1, a_2,...,a_t])$\end{small}. However, the perturbed actions \begin{small}$a_1, a_2,...,a_t$\end{small} are fed sequentially to LSTM, and thus the state embedding $s_t$ will not preserve the order-invariant property. It would mean that a given state would depend on the order of perturbations performed which is not what we desire. To alleviate this issue, we randomly shuffle the order of actions while training and re-calculate the state embeddings of the DQN for the random ordering. Thus the model is forced to learn order invariant embeddings.

\textbf{Actions}.
Naturally the two types of perturbations will have different action spaces as well.
A simple action space for replacing relations can be defined as the set of all possible edges but it will make the action space very large and pose a huge scalability problem. Instead we break down the relation replacement action into a triple of subactions, \begin{small}$a_t = (a_t^{(0)}, a_t^{(1)}, a_t^{(2)})$\end{small}, where \begin{small}$a_t^{(0)}$\end{small} is to choose the head entity, \begin{small}$a_t^{(1)}$\end{small} is to choose a neighbour entity and finally \begin{small}$a_t^{(2)}$\end{small} is to choose a relation type that substitutes the relation between the chosen entities. We further restrict the action space to the top K actions with the lowest ATS in the original action space for \begin{small}$a_t^{(2)}$\end{small}. Thus we try to ensure a  drop in evaluation metrics with a reduced action space.

For edge perturbations, we break down the actions into a triple of subactions, \begin{small}$a_t = (a_t^{(0)}, a_t^{(1)}, a_t^{(2)})$\end{small}, where \begin{small}$a_t^{(0)}$\end{small} is to choose the head entity, \begin{small}$a_t^{(1)}$\end{small} is to choose a neighbour entity and \begin{small}$a_t^{(2)}$\end{small} is to choose an entity not in the direct neighbourhood of the head entity. So at every action, we remove the edge between the head and the tail entity (chosen by \begin{small}$a_t^{(0)}$\end{small} and \begin{small}$a_t^{(1)}$\end{small}) and add the edge with the same relation between the same head entity but the tail entity chosen by \begin{small}$a_t^{(2)}$\end{small}. 

Clearly for both the setups, the subaction \begin{small}$a_t^{(1)}$\end{small} depends on \begin{small}$a_t^{(0)}$\end{small} and similarly  \begin{small}$a_t^{(2)}$\end{small} depends on \begin{small}$a_t^{(1)}$\end{small}, \begin{small}$a_t^{(0)}$\end{small}. To solve for such action spaces, 
we use a hierarchical system of two DQNs to choose these. \begin{small}$a_t^{(0)}$\end{small} is chosen randomly. The first DQN takes the state and \begin{small}$a_t^{(0)}$\end{small} to sample \begin{small}$a_t^{(1)}$\end{small} and the second DQN follows similar procedure to sample \begin{small}$a_t^{(2)}$\end{small}. The actions for both the perturbations are kept similar to ensure that the same hierarchical framework works for both of them.

%For semantic perturbation, the action $a_t$ is to choose a triple from KG and substitute its relation type with another one. We can assign \begin{small}$a_t^{(0)}$\end{small} as the head entity, \begin{small}$a_t^{(1)}$\end{small} as its neighbour and finally \begin{small}$a_t^{(2)}$\end{small} as the relation type that substitutes the given relation.
%For structure perturbation, the action can also be decomposed to choosing a head entity, its neighbour and another tail entity. So the edge between the head and its neighbour is transferred to the tail entity.



% \textbf{Actions. }
% For both perturbations, the action space is very large and impractical to model. Thus to shrink the action space, we decompose an action $a_t$ into three subactions $a_t^{(0)}, a_t^{(1)}, a_t^{(2)}$, and the action space $A$ is decomposed into 
% \begin{small}$A= A_0\times_{a_0} A_1 \times_{(a_0,a_1)} A_2$\end{small}.
% For semantic perturbation, the action $a_t$ is to choose a triple from KG and substitute its relation type with another one. It can be decomposed to, first choosing a head entity ($a_t^{(0)}\in A_0=\mathcal{E}$), then a tail entity $a_t^{(1)}\in A_1(a_0)=\text{Neighbor}(a_0)$, and finally the relation type to substitute $a_t^{(2)}\in A_2=\mathcal{R}$.
% For edge perturbation, the action can also be decomposed to choosing a head entity ($a_t^{(0)}\in A_0=\mathcal{E}$), then a tail entity $a_t^{(1)}\in A_1(a_0)=\text{Neighbor}(a_0)$, and finally another tail entity for substitute $a_t^{(2)}\in A_2=\mathcal{E}$.

% In this way, we've unified the two types of perturbations in one framework. To accommodate the actions, we also decompose the DQN into 2 sub DQNs {$Q_1, Q_2$}. Note we choose $a_t^{(0)}$ randomly at each steps without DQN, because we are going to perturb a large percentage of the graph and nearly all actions in A_0 will be chosen, and thus the choice of $a_t^{(0)}$ is not decisive.

\textbf{Reward.}
The reward is designed to reflect the change of downstream task performance. 
For QA tasks, we minimize the KL divergence between the predicted distribution and the distribution over right answers. The distribution over right answers is a dirac distribution over the right answer. We set the reward as the decrease in KL-Divergence from the previous state. The reward may be at very small scale, so we record the average of the absolute value of rewards and scale it to a pre-set value.
For recommendation task, we directly use the development AUC metric as the reward.


% \textbf{Reward.}
% The reward is designed to reflect the change of downstream task performance. 
% For QA, the straightforward design is to use the change of test set accuracy as rewards. However, the accuracy change is discrete and is not aware of probability drop, e.g., from 0.9 to 0.5 as long as the correct answer has the highest predicted probability. Therefore, we adopt KL-divergence between predicted answer distribution and the uniform wrong distribution as the extent of the predicted distribution to be wrong, and use the drop of it as reward. $Reward=\sum_{(q,a)} Reward(q,a)$, where $
%     Reward(q,a)=- \Delta (D_{KL}(p_{predict}||p_{wrong}))\text{  ,  }  p_{wrong}(a)=\begin{cases}0, &a \text{ is correct} \cr \frac{1}{num\_answers-1} , & a \text{ is wrong} \end{cases} $
% The reward may be at very small scale, so we record the average of the absolute value of rewards and scale it to a pre-set value.

% While trying to preserve the downstream task performance, we also need to ensure we are perturbing KG to a large scale by dropping validation score dramatically. Such multi-task problem is hard to solve if we simply integrate the two tasks into rewards, as it's hard to decide the weight of each task. Therefore, we restrict the action space $A^\prime_2$ to the K actions with lowest validation scores in the original action space $A_2$. In this way we can ensure that the validation score drops dramatically.


% \begin{figure}[H] 
% \centering 
% \includegraphics[width=0.5\textwidth]{figures/model_arch.JPG} 
% \caption{Model Architecture \xiang{@Hansen, pls update this figure and beautify it more.}} 
% \label{model_figure} 
% \end{figure}

% \begin{figure}
%  \hfill\begin{minipage}{.5\textwidth}\centering
%   \includegraphics[width=0.7\textwidth]{figures/model_arch.JPG} 
%   \caption{\texttt{minipage}}
%  \end{minipage}
% \end{figure}
% \begin{tabular}{cc}
% \raisebox{.1cm}
% {
% \begin{minipage}{.5\textwidth}
% \begin{figure}[H] 
% \begin{flushright}
% \includegraphics[width=0.7\textwidth]{figures/model_arch.JPG} 
% \caption{Model Architecture
% \xiang{@Hansen, pls update this figure and beautify it more.}} 
%  \end{flushright}
% \label{model_figure} 
% \end{figure}

% \begin{algorithm}[H]
% \SetAlgoLined
% % \KwResult{Write here the result }
%  Parameters: $S, T, T_1, T_2, T_3 \;$
%  initialization:$\mathcal{B}$,$h_0\;$
%  \For{n=1,2,...,S }{

%   \For{t=1,2,...,T}{
%     Randomly select $a_t^{(0)}$\;
%     Calculate $Q_{1,\theta}$ by \eqref{cal_Q1}\;
%     With $\epsilon$ probability, randomly select $a_t^{(1)}$, otherwise $a_t^{(1)}=\text{argmax}Q_{1,\theta}(a|s_t,a_t^{(0)}) $\;
%     Calculate $Q_{2,\phi}$ by \eqref{cal_Q2}\;
%     With $\epsilon$ probability, randomly select $a_t^{(2)}$, otherwise $a_t^{(2)}=\text{argmax}Q_{2,\phi}(a|s_t,a_t^{(0)},a_t^{(1)}) $\;
%     Calculate $s_{t+1}$ \text{through LSTM Cell} \;
%     \If{t==T}{
%     Evaluate KG on downstream tasks and get $r$ by \eqref{reward}}
%     \Else{r=0}
%     Store ($s_t$,$a_t$,$s_{t+1}$,r) in $\mathcal{B}$
%     \If{t mod $T_1==0$}{
%         sample a batch from $\mathcal{B}$ \;
%         update through \eqref{bellman} \;
%     }
%     \If{t mod $T_2==0$}{
%         $\theta_1^\prime = \theta_1$, $\phi_1^\prime = \phi_1$
%     }
    
%   }
%  }
%  \For{t=1,2,...,$T_3$}{
%       \text{ sample a batch from} $\mathcal{B}$ \;
%         \text{update through} \eqref{bellman} \;
%  }
 
%  \caption{Training process of our DQN}
% \end{algorithm}
% \end{minipage}}
% &
% \begin{minipage}{.5\textwidth}

% \end{minipage}
% \end{tabular}


% \begin{algorithm}[H]
% \SetAlgoLined
% % \KwResult{Write here the result }
%  Parameters: $S, T, T_1, T_2, T_3 \;$
%  initialization:$\mathcal{B}$,$h_0\;$
%  \For{n=1,2,...,S }{

%   \For{t=1,2,...,T}{
%     Randomly select $a_t^{(0)}$\;
%     Calculate $Q_{1,\theta}$ by \eqref{cal_Q1}\;
%     With $\epsilon$ probability, randomly select $a_t^{(1)}$, otherwise $a_t^{(1)}=\text{argmax}Q_{1,\theta}(a|s_t,a_t^{(0)}) $\;
%     Calculate $Q_{2,\phi}$ by \eqref{cal_Q2}\;
%     With $\epsilon$ probability, randomly select $a_t^{(2)}$ \;
%    otherwise $a_t^{(2)}=\text{argmax}Q_{2,\phi}(a|s_t,a_t^{(0)},a_t^{(1)}) $\;
%     Calculate $s_{t+1}$ \text{through LSTM Cell} \;
%     \If{t==T}{
%     Evaluate KG on downstream tasks and get $r$ by \eqref{reward}}
%     \Else{r=0}
%     Store ($s_t$,$a_t$,$s_{t+1}$,r) in $\mathcal{B}$
%     \If{t mod $T_1==0$}{
%         sample a batch from $\mathcal{B}$ \;
%         update through \eqref{Bellman1} \eqref{Bellman2} \;
%     }
%     \If{t mod $T_2==0$}{
%         $\theta_1^\prime = \theta_1$, $\phi_1^\prime = \phi_1$
%     }
    
%   }
%  }
%  \For{t=1,2,...,$T_3$}{
%       \text{ sample a batch from} $\mathcal{B}$ \;
%         \text{update through} \eqref{bellman} \;
%  }
 
%  \caption{Training process of our DQN}
% \end{algorithm}



% \begin{figure}[htbp]
% \centering
% \begin{minipage}[c]{0.4\textwidth}
% \centering
% \includegraphics[width=0.7\textwidth]{figures/model_arch.JPG}
% \caption{Model Architecture} 
% \label{model_figure} 
% \end{minipage}

% \noindent
% \begin{minipage}[c]{0.4\textwidth}
% \centering




% \end{minipage}
% \end{figure}

\textbf{DQN Architecture and Training Process.}
The proposed DQN architecture is illustrated in Figure \ref{fig:model_figure}. At the step $t$ of perturbing triples in the KG, the state embedding $s_t$ together with the chosen actions are fed into the LSTM Cell to form the Q functions $Q_1$ and $Q_2$ as follows:
% $$ Q_1(a_t^{(1)}|s_t,a_t^{(0)})=\text{Dot}(MLP(a_t^{(1)}),MLP(h_t^{(1)})) $$
% $$ Q_2(a_t^{(2)}|s_t,a_t^{(0)},a_t^{(1)})=\text{Dot}(MLP(a_t^{(2)}),MLP(h_t^{(2)})) $$
% \vspace{-0.05cm}
\begin{small}
\begin{equation}
Q_1(a_t^{(1)}|s_t,a_t^{(0)})= \langle MLP(a_t^{(1)}),MLP(h_t^{(1)})\rangle; \label{cal_Q1} 
\end{equation}
\vspace{-0.3cm}
\begin{equation}
 Q_2(a_t^{(2)}|s_t,a_t^{(0)},a_t^{(1)})=\langle MLP(a_t^{(2)}),MLP(h_t^{(2)}) \rangle; \label{cal_Q2} \end{equation}
 \end{small}
where $h_t^{(1)}=\text{LSTMCell}_1(s_t,a_t^{(0)})$ and $h_t^{(2)}=\text{LSTMCell}_2(s_t,[a_t^{(1)},a_t^{(0)}])$ are the immediate hidden representation of current state. 
Actions $a_t^{(1)}$ and $a_t^{(2)}$ are chosen via Q function $\epsilon$-greedily during training and greedily during evaluation.

Evaluating the KG on downstream task is heavily time-consuming, and our task also requires a large number of perturbations. Therefore, we only get rewards every $T$ steps. $T$ can be as large as hundreds. In this way, the Q function $Q(s_t,a_t)$ is to predict the expectation of reward at step $T$ if we choose action $a_t$ at current state $s_t$. 

The training of DQN follows the common approach. Q functions are updated through Q-iterations minimizing the Bellman Error as follows.
\begin{small}
\begin{equation}
\theta \leftarrow \theta - \alpha \nabla_\theta (\gamma \max_{a_t^{(2)}} Q_{2,\phi^\prime}(a_t^{(2)}|s_t,a_t^{(0)},a_t^{(1)})-Q_{1,\theta}(a_t^{(1)}|s_t,a_t^{(0)}))^2; \label{Bellman1}
\end{equation}
\vspace{-0.3cm}
\begin{equation}
\phi \leftarrow \phi - \alpha \nabla_\phi ((r + \gamma \max_{a_{t+1}^{(1)}} Q_{1,\theta^\prime}(a_{t+1}^{(1)}|s_{t+1},a_{t+1}^{(0)}))-Q_{2,\phi}(a_{t}^{(2)}|s_t))^2.  \label{Bellman2}
\end{equation}
\end{small}
In this way, we are able to train the DQN and learn our targeted perturbation policy.
% The overall training framework is summarized in Algorithm 1.


% \xiang{where is the algorithm box??}


    
% \subsection{Validation Score}
% Since our aim is to perturb the Knowledge Graph we require a metric to judge the extent to which the graph has been corrupted. To this end we suggest the use of the following two different types of validation scores:
% \begin{itemize}
%     \item Embedding Based Validation Score: This validation score is derived from a Knowledge Base Completion model trained on Conceptnet. We train the embedding based Knowledge base completion architecture as specified in \citep{li-etal-2016-commonsense} on Conceptnet. This model take a triple as input and outputs the probability of the triple being semantically correct. We define the score of a triple to be this probability. We define the validation score of a graph to be the mean of scores of each triple in the graph. A thing to note is that this validation score will fail to capture the structure changes in the graph as will be evident in the experiments section. To alleviate this problem we use another validation score.
%     \item Structure Based Validation Score: This validation score is based on the observable properties of a Graph such as clustering coefficient. To incorporate relational information we first extract subgraphs from the complete graph that contain only a given relation. Then we find the mean of the clustering coefficient distributions of all such subgraphs. Then we use the reciprocal of the L2 distance between the mean distributions of the perturbed graph and the original graph. Note that unlike the Embedding based validation score this validation score does whether a triple makes semantic sense. Thus for our work it is of prime importance we use both these validation scores. 
% \end{itemize}

% \subsection{Semantic Based Perturbation}
% This is the first type of perturbation that we aim to achieve on a KG. Using this type of perturbations we try to corrupt the graph without changing the structure of the KG. 
% For this type of perturbations, we will choose a triple and substitute its relation type with another relation type at each step. We will do a large amount of steps to make sure the graph is largely perturbed. We decompose a single step into three sub-actions: action0 is to choose a head entity from the KG, action1 is to choose a tail entity from the neighborhood of head entity, and action2 is to choose the relation type to substitute for the original one. 
% In order to maintain high performance on downstream tasks with the largely perturbed KG, we leverage the Deep Q-networks(DQN), a reinforcement learning algorithm for this task. We view the downstream task performance as environment, and our perturbation policy as the agent. Thus the DQN is to learn a Q-function for the actions, and use rewards from downstream task performance to update its parameters. 
% Since we will perturb a large percentage of KG, the choice of action0 is not decisive. Therefore, we randomly choose action0 at each step. We use 2 DQNs for selecting action1 and action2, respectively. In order to ensure we are really perturbing the graph heavily, action2 (the relation type) is selected from the K actions with lowest validation score. In experiments, we set K=5.



% \subsection{Structure Based Perturbation}
% For this type of perturbation, we will choose a triple and substitute its tail entity with another tail entity at each step. We will do a large amount of steps to make sure the graph is largely perturbed. Similar to semantic based perturbation, we decompose a single step into three sub-actions: action0 is to choose a head entity from the KG, action1 is to choose a tail entity from the neighborhood of head entity, and action2 is to choose another tail entity to substitute for the original one. 
% %%

==> backup/backup_Oct22/5_experiment.tex <==
% !TEX root = main.tex

\section{Experiments}
\label{sec:exp}
\vspace{-0.2cm}

In this section, we evaluate the effectiveness of our heuristic and RL-based perturbation in perturbing KG as well as preserving performance of a fixed model on commonsense QA and recommender system tasks respectively. A frozen downstream model is used to ensure that the model does not have a chance to overfit to the perturbed graph. We denote our two RL based perturbation methods by \textbf{RL-Relation Replacement (RL-RR)} and \textbf{RL-Edge Rewiring (RL-ER)} respectively. We also conduct human evaluation on the explanation given by the symbolic knowledge from both unperturbed and perturbed KGs to cast doubt on their faithfulness.
%In this section we introduce our experimental setup. With the help of these experiments, we challenge the faifulness of the symbolic knowledge in the current models. 
%try to validate our hypothesis that current models on many tasks do not model the KG effectively.
%We use different types of perturbation techniques to show even if the KG is completely perturbed we can maintain the downstream performance. We also perform some analysis on the paths that the models deem important for a prediction which pose questions on the interpretability of such models.

% \vspace{-0.2cm}
% \subsection{Experiment Setup}
% \vspace{-0.2cm}

\vspace{-0.2cm}
\subsection{Baselines for Graph Perturbation}
\vspace{-0.2cm}

In addition to the Relation Swapping(RS) and Relation Replacement(RR) perturbation heuristics (\textsection~\ref{sec: pilotexpts}), we further introduce two other perturbation methods as baselines in our experiments.

\textbf{Edge Rewiring (ER): } We first randomly select an edge $(h,r,t)$ in the KG. 
%We denote by $\mathcal{N}(h)$ the set of neighbors for the entity $h$. 
Let $k \in \mathcal{E} \setminus \mathcal{N}_1(h)$. 
Then we rewire the edge to another one with the same relation, i.e.,
$
    \mathcal{T} \leftarrow (\mathcal{T} \setminus \{(h,r,t)\}) \cup \{(h,r,k)\}
$.
It alters the structure of the graph but keep the relation distribution across the KG constant. 

\textbf{Edge Deletion (ED):} We randomly select an edge and delete it.
% \begin{align}\label{eq:deletion-heuristic}
%   &i \sim \text{UniformDiscrete}\{1,2,\ldots,|\mathcal{T}|\} \\
% %   ,\quad \text{for } j=1,2,\ldots\\
%     &\mathcal{T} \leftarrow \mathcal{T} \setminus \{e_i=(h,r,t)\} \nonumber
% \end{align}\noindent
%This heuristic clearly changes both the structure of the graph as well as the distribution of relations across the KG.
This heuristic changes both the structure of the graph as well as the relation distribution across the KG. 
Note that the ATS metric will fail to recognize these perturbations to the KG by design, since after deletion the remaining edges are still valid triples .

% In the next subsection we denote Relation Swapping Heuristic and Greedy Heuristic as Semantic Heuristic 1 and Semantic Heuristic 2 respectively. We denote Deletion Heuristic and Rewiring Heuristic as Structure Heuristic 1 and Structure Heuristic 2 respectively. Next we introduce the tasks on which we perform our experiments.

\vspace{-0.2cm}
\subsection{Evaluation Protocol and Metrics}
\vspace{-0.2cm}

As discussed above, the ATS metric is not sensitive to structure perturbation in the KG. Thus, we adopt the \textbf{Similarity on Clustering Coefficient Distribution (SC2D)} as a complementary metric. Given a KG \begin{small}$\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$\end{small}, we define \begin{small}$\mathcal{G}^r$\end{small} as the subgraph containing all the triples with a particular relation $r$, i.e., \begin{small}$\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
    where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$.\end{small}
% \ryan{This strategy looks at triangles that are all homogeneous in terms of their relation $r$, what about triangles that are not all of the same relation $r$, but mixed relations? There are typically far more of these, just by chance. But in any case, its unclear why they were ignored. It was probably done since the above way just makes it simple to apply standard algorithms, but hopefully we have a more solid reason and justification for this.}
We then compute the relation specific clustering coefficient vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective} of the $i^{th}$ entity and compute the average clustering vector $\mathbf{c}$ for the whole graph as the average of $\mathbf{c^r}$ over all $r \in \mathcal{R}$, i.e., $\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$.
We denote the average clustering vector for the unperturbed KG and the perturbed KG by $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ respectively. We then define the SC2D metric as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$, i.e.,
$f^{SC2D}(\mathcal{G},\mathcal{G}^{'}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$
with $b$ as a constant for avoiding zero division.

The SC2D metric is not effective for cases where the KG has a very small local clustering coefficient like the recommendation KG's which are almost bipartite and hence the local clustering coefficient is negligible. To this end, we introduce another metric, \textbf{Similarity on Degree Distribution (SD2)}, which can also capture structural changes. Similar to the SC2D metric, we first create a set of graphs $\mathcal{G}^{r}$ for each relation $r \in \mathcal{R}$. We then calculate the relation specific degree vector $\mathbf{d^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{d^r}$ represents the degree of the $i^{th}$ node and calculate the average degree vector $\mathbf{d}$ for the whole graph as the mean of $\mathbf{d^r}$ over all $r \in \mathcal{R}$, i.e., $\mathbf{d} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{d^r}$.
We denote the average degree vector of the unperturbed KG and the perturbed KG by $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$ respectively. We then define the SD2 metric of the KG as the reciprocal of the L2 distance between $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$, i.e.,
$
f^{SD2}(\mathcal{G},\mathcal{G}^{'}) = \frac{1}{\lVert \mathbf{d_{o}} - \mathbf{d_{p}} \rVert_2 + b}.
$
In the later experiment we would validate these proposed evaluation metrics by comparing them with human evaluation.
  
\begin{table*}[t]
\vspace{-0.6cm}
% \centering
\caption{\textbf{Performance comparison on CSQA and OBQA perturbation experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CSQA and the official test accuracy on OBQA. We perturb all the triples (100\%) in the original KG.
% \xiang{@Mrigank: 1. Use full names for the baselines? 2. go to 3 decimal places for the validation metrics; 3. Let's still show all the three metrics for both task; and explain the issues in writing.}
}
\label{tab:results:csqa}
\hspace{-0.3cm}
\vspace{-0.3cm}
\scalebox{0.49}{
\begin{tabular}{lcccccccccccccccc}
    \toprule 
    %\multirow{2}{*}{\textbf{Methods}}
    &
    \multicolumn{8}{c}{ \textbf{CSQA}}&\multicolumn{8}{c}{ \textbf{OBQA}}\\
    \cmidrule(lr){2-9} \cmidrule(lr){10-17}
    & \multicolumn{4}{c}{ \textbf{RN}}&\multicolumn{4}{c}{ \textbf{MHGRN}} &\multicolumn{4}{c}{ \textbf{RN}} &\multicolumn{4}{c}{ \textbf{MHGRN}}\\
    \cmidrule(lr){2-5}
    \cmidrule(lr){6-9}
    \cmidrule(lr){10-13}
    \cmidrule(lr){14-17}
    \textbf{Methods}& Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) &  Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$)& Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) & Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$)& SD2 ($\downarrow$) \\
    \midrule
    {w/o KG} & ~53.41 & - & - &- & ~53.41 & - &- & - & ~62.00 & - & - &- & ~62.00 & - &-&- \\
    {w/ KG} & 56.87 & 0.940&-&- & 57.21 & 0.940&-&- & 66.80 & 0.934&-&- & 68.00 & 0.934&-&- \\
    \midrule
    {Relation Swapping} & 53.42 & 0.831&0.168&6.20E-3 & 53.42 & 0.831& 0.168 & 6.20E-3 & 67.00 & 0.857&0.189& 7.79E-3& 67.30& 0.857&0.189&7.79E-3 \\
    {Relation Replacement} & 53.42 & 0.329& 0.100&1.70E-3 & 52.22 & 0.329& 0.100&\textbf{1.70E-3} & 66.80 & 0.269&0.105&1.84E-3 & 67.60 & 0.269&0.105&1.84E-3 \\
    {Edge Rewiring} & 53.42 & 0.505&0.131&2.31E-3 & 52.22 & 0.505&0.131&2.31E-3 & 66.60 & 0.620&0.172&7.31E-3 & 67.00 & 0.620&0.172&7.31E-3 \\
    {Edge Deletion} & 52.21 & 0.933&0.144&2.00E-3 & 51.00 & 0.933&0.144&2.00E-3 & 66.80 & 0.923&0.155& 2.19E-3&67.60 & 0.923&0.155&2.19E-3 \\
    \midrule
    {RL-ER} & 54.89 & 0.346&\textbf{0.081}&1.76E-3 & 55.05 & 0.325&\textbf{0.073}&1.78E-3 & 67.00 & 0.518&\textbf{0.100}& 5.55E-4&\textbf{67.80} & 0.584&\textbf{0.104}&6.49E-4 \\
    {RL-RR} & \textbf{55.21} & \textbf{0.322}&0.102 & \textbf{1.66E-3}& \textbf{55.52} & \textbf{0.314}&0.101&1.78E-3 & \textbf{67.30} & \textbf{0.255}&0.108 & \textbf{1.79E-4}& 67.70 & \textbf{0.248}&\textbf{0.104}&\textbf{1.75E-4} \\

    % {RL Edge} & 54.75 & 0.505&\textbf{0.082} & \textbf{55.15} & 0.542&\textbf{0.070} & 66.60 & 0.411&0.163 & 67.20 & 0.341&0.095 \\
    % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
    % \midrule
    % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
    % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
    % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    \bottomrule 
\end{tabular}
}
\vspace{-0.0cm}
\end{table*} 




\subsection{ Commonsense QA Experiments}
\vspace{-0.2cm}

%Given a dataset and a neuro symbolic QA model, we try to deceive the model into learning corrupt graph structures and giving invalid explanations using a perturbed KG. 
%We first introduce our experimental setup for the commonsense question answering task.

% \xiang{what is the task/problem setting (input and output, goal)? Should introduce before going into models..}

% \textbf{Setup.}
We conduct experiments on CommonsenseQA (CSQA) and OpenBookQA (OBQA), both of which require external knowledge beyond context to answer the questions. %In addition to CommonsenseQA dataset that we introduced in section\ref{sec: pilotexpts}, we also exhibit our experiments on OpenBookQA which is a question answering dataset that consists of science questions and shows improvement in performance after augmenting a Language Model with a KG. The labels for the official test set are available and we report our results on the official test set. We run our experiments MHGRN \citep{feng2020scalable}, RelationNet \citep{santoro2017simple} and Graph Networks \citep{battaglia2018relational}.
%\textbf{KG-augmented Models for QA.} 
% \xiang{1-2 sentences to summarize how these models are like (summarizing from previous section is okay).}
The neural-symbolic QA systems we experiment with are MHGRN (\textsection~\ref{sec: pilotexpts}) and Relation Networks~(RN,~\cite{santoro2017simple}), which is a path-based model. MHGRN and RN are shown to significantly outperform baselines without KG  in~\cite{feng2020scalable}. We train both models to replicate their original performance using BERT-Base as the text encoder, and freeze the models throughout the perturbation. The KG we aim to perturb is ConceptNet~\citep{speer2016conceptnet}, a commonsense KG that fits to this task.
% and Graph Networks~\citep{battaglia2018relational} 
 
%For each instance in the dataset these models encode the subgraph containing the concepts from this instance and use these encodings for predicting the correct answer for a given question. Relation Net encodes the relational paths between concepts whereas MHGRN uses a Graph Neural Network to encode the subgraphs for each instance.

% \textbf{Evaluation Protocol and Metrics.}
% As discussed above, the ATS metric is not sensitive to structure perturbation in the KG. Thus, we adopt the \textbf{Similarity on Clustering Coefficient (SC2D)} as a complementary metric. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$, we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$, i.e., $\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
%     where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$.
% % \ryan{This strategy looks at triangles that are all homogeneous in terms of their relation $r$, what about triangles that are not all of the same relation $r$, but mixed relations? There are typically far more of these, just by chance. But in any case, its unclear why they were ignored. It was probably done since the above way just makes it simple to apply standard algorithms, but hopefully we have a more solid reason and justification for this.}
% We then compute the relation specific clustering coefficient vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective} of the $i^{th}$ node and compute the average clustering vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e., $\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$.
% We denote the average clustering vector for the unperturbed KG and the perturbed KG by $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ respectively. We then define the SC2D metric as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$, i.e.,
% $V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$
% with $b$ as a constant for avoiding zero division.

\textbf{Results and Discussion.}
%For experiments on Question Answering, we take the complete conceptnet graph and prune it first such that it only contains edges that are relevant for the given dataset i.e for each edge either the head entity or the tail entity is a part of the given dataset. 
Table~\ref{tab:results:csqa} shows our results of perturbing all the triples in KG. Note that perturbing relations or edges are not guaranteed to yield invalid/novel triples. Thus, a completely perturbed KG would still have a different degree of deviation from the original KG, depending on what perturbation method is used. This can be evidenced by the different evaluation metric scores in Table~\ref{tab:results:csqa}, which show that generally either our RL-RR or RL-ER method yields the perturbed KG with the most degree of deviation. Such a perturbed KG is not meaningless noise. This is supported by Table~\ref{tab:randomized_baseline}, which shows that our designed controlled noisy baselines (\textsection~\ref{sec: pilotexpts}) lead to significant performance drop. Overall, the above observations demonstrate the necessity of introducing our RL-based perturbation method to complement the heuristic methods even when we do complete perturbation. But we notice that the performance drop in OBQA in Table \ref{tab:randomized_baseline} is more severe than compared to CSQA. These results along with with the results in Table \ref{tab:results:csqa} lead us to believe that more than the  connections and semantics in the KG, the entity and the relation embeddings play a major role in the prediction of OBQA. In this work we use the BERT based tzw entity embeddings and TransE based relation embeddings.
%We also report the embedding based and the clustering coefficient evaluation metric to get an idea about how much corrupted the KG is. From table\ref{tab:results:csqa} w

Moreover, we observe that using
heuristic perturbation, both RN and MHGRN do not outperform the non-KG baseline on CSQA while on OBQA they manage to maintain their performance. 
%using heuristic perturbations the performance almost always drop to the level of non KG baseline on the CSQA dataset. Whereas on the OBQA dataset we observe that even with a randomly corrupted KG, we are able to maintain the performance. 
Using RL-based targeted perturbation policy, both QA models achieve a statistically significant improvement according to the T-test over both heuristics and non-KG baselines with 3 independent runs, which demonstrate the superiority of our RL perturbation method over simple heuristics. On OBQA, both our two RL methods even yield a better performance with RN model compared with the original KG. Such success of perturbing KG completely while still preserving and even improving performance suggests both RN and MHGRN are relying on problematic symbolic knowledge for prediction. Thus it validates our doubt on whether symbolic knowledge contributes to the improvement interpretably. Our later human study on the interpretability would further validates our doubt.  %With the help of our human evaluations we also show the edges on which the model gives more weight are not interpretable and the few interpretable edges can also be corrupted.

Figure~\ref{fig:final_curves} illustrates the change in performance of MHGRN on CSQA and the KG evaluation metrics across different scales of perturbation. We observe that both RL-RR and Relation Replacement heuristic are more effective in perturbing KG compared with Relation Swapping. We also observe that for larger scales of perturbations the RL policy can maintain the performance of the model better than the heuristics do, which validates the superiority of our learned RL policy. 
%It indicates that the RL policy is able to perturb the KG to the same extent if not more as is evident from the drastic drop in evaluation metrics.

\begin{wraptable}{h}{0.38\textwidth}
% \vspace{-0.6cm}
\centering
\scalebox{0.8}{
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c}{\textbf{CSQA}} & \multicolumn{2}{c}{\textbf{OBQA}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} & Read. & Use. & Read. & Use. \\
\midrule
Ori. KG & 0.580&0.420&0.711&0.232  \\
%\midrule
%RL1 &0.4178&0.2444&0.4200&0.1550\\
RL-RR &0.452&0.268&0.418&0.156\\
RL-ER&0.429&0.285&0.410&0.179\\
\bottomrule
    \end{tabular}
}
    \caption{\small \textbf{Human evaluation} on the readability (Read.) and Usefulness (Use.) of the paths from MHGRN. }
    \label{tab:user_study}
\end{wraptable}



\textbf{Human Evaluation on Model Explanation.}
% \xiang{@Peifeng: let’s write out the human evaluation paragraph and talk about the scores, inter-annotator agreement metric, and correlation metric}
We conduct human evaluations on the symbolic paths given by MHGRN, which are claimed to serve as the explanation for MHGRN's prediction. We randomly select 10 questions from the CSQA and OBQA test sets which are predicted correctly by the model and obtain the top ranked paths that are attended most by MHGRN. We then ask 5 human annotators to annotate each path for two dimensions, i.e., readability and usefulness. Readability is about whether the paths make sense to the annotators while usefulness is about whether the paths are useful for the annotators to identify the correct answer versus the wrong choices. We take the majority vote as the score for each instance.  The average annotation scores is reported in Table~\ref{tab:user_study} with the fleiss $\kappa$ inter-annotator agreement as $0.312$ and $0.314$ for each dimension, which indicates a fair agreement. We observe that compared with the original KG, the paths from the two RL perturbed KGs contain more invalid symbolic knowledge, indicating our proposed RL perturbation is effective. Meanwhile, for all the KGs our annotators consider the paths from the original can provide more plausible explanation for the prediction compared with the paths from the perturbed graphs. This validates our doubt on the faithfulness of explanation given by KG-based neural-symbolic models. 

\textbf{Quality of Evaluation Metrics.}
We also leverage the validity scores given by human to validate the effectiveness of our three proposed KG evaluation metrics, ATS, SC2D and SD2. The Pearson correlation coefficient between the human evaluation scores in Table~\ref{tab:user_study} and the three KG evaluation metrics in Table~\ref{tab:results:csqa} are $0.845$, $0.932$ and $0.932$ respectively, both showing high correlation. This demonstrates that the KG evaluation metrics well capture KG's semantic validity.


% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on CommonsenseQA and OBQA perturbation experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA and on the official set of OBQA. We perturb all the triples in the KG
% % \xiang{@Mrigank: 1. Use full names for the baselines? 2. go to 3 decimal places for the validation metrics; 3. Let's still show all the three metrics for both task; and explain the issues in writing.}
% }
% \label{tab:results:csqa}
% \scalebox{0.65}{
% \begin{tabular}{lcccccccccccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{8}{c}{ \textbf{CSQA}}&\multicolumn{8}{c}{ \textbf{OBQA}}\\
%     \cmidrule(lr){2-9} \cmidrule(lr){10-17}
%     & \multicolumn{4}{c}{ \textbf{RN}}&\multicolumn{4}{c}{ \textbf{MHGRN}} &\multicolumn{4}{c}{ \textbf{RN}} &\multicolumn{4}{c}{ \textbf{MHGRN}}\\
%     \cmidrule(lr){2-5}
%     \cmidrule(lr){6-9}
%     \cmidrule(lr){10-13}
%     \cmidrule(lr){14-17}
%     & Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) &  Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) & Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$)  & Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) & SD2 ($\downarrow$) \\
%     \midrule
%     {w/o KG $^{\dagger}$} & ~53.71 & - & - & ~53.71 & - & - & ~62.00 & - & - & ~62.00 & -&- \\
%     {w/ KG} & 56.87 & 0.940&- & 57.21 & 0.940&- & 66.80 & 0.934&- & 68.00 & 0.934&- \\
%     \midrule
%     {Relation Swapping} & 53.42 & 0.831&0.168 & 53.42 & 0.831& 0.168 & 67.00 & 0.857&0.189& 67.80& 0.857&0.189 \\
%     {Relation Replacement} & 53.42 & 0.329&0.100 & 52.22 & 0.329&0.100 & 66.80 & 0.269&0.105 & 67.60 & 0.269&0.105 \\
%     {Edge Rewiring} & 53.42 & 0.505&0.131 & 52.22 & 0.505&0.131 & 66.60 & 0.620&0.172 & 67.00 & 0.620&0.172 \\
%     {Edge Deletion} & 52.21 & 0.933&0.144 & 51.00 & 0.933&0.144 & 66.80 & 0.923&0.155& 67.60 & 0.923&0.155 \\
%     \midrule
%     {RL Relation} & \textbf{55.12} & \textbf{0.312}&0.108 & 54.63 & \textbf{0.314}&0.101 & 66.40 & 0.273&0.104 & 67.20 & 0.278&0.104 \\
%     {RL Edge} & 54.75 & 0.505&\textbf{0.082} & \textbf{55.15} & 0.542&\textbf{0.070} & 66.60 & 0.411&0.163 & 67.20 & 0.341&0.095 \\
%     % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
%     % \midrule
%     % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
%     % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
%     % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*} 



% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on CommonsenseQA and OBQA perturbation experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA and on the official set of OBQA. We perturb all the triples in the KG
% % \xiang{@Mrigank: 1. Use full names for the baselines? 2. go to 3 decimal places for the validation metrics; 3. Let's still show all the three metrics for both task; and explain the issues in writing.}
% }
% \label{tab:results:csqa}
% \scalebox{0.65}{
% \begin{tabular}{lcccccccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{6}{c}{ \textbf{CSQA}}&\multicolumn{6}{c}{ \textbf{OBQA}}\\
%     \cmidrule(lr){2-7} \cmidrule(lr){8-13}
%     & \multicolumn{3}{c}{ \textbf{RN}}&\multicolumn{3}{c}{ \textbf{MHGRN}} &\multicolumn{3}{c}{ \textbf{RN}} &\multicolumn{3}{c}{ \textbf{MHGRN}}\\
%     \cmidrule(lr){2-4}
%     \cmidrule(lr){5-7}
%     \cmidrule(lr){8-10}
%     \cmidrule(lr){11-13}
%     & Acc ($\uparrow$) & ATS ($\downarrow$) & SC2D ($\downarrow$) &  Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) & Acc & ATS ($\downarrow$) & SC2D ($\downarrow$)  & Acc & ATS ($\downarrow$) & SC2D ($\downarrow$) \\
%     \midrule
%     {w/o KG $^{\dagger}$} & ~53.71 & - & - & ~53.71 & - & - & ~62.00 & - & - & ~62.00 & -&- \\
%     {w/ KG} & 56.87 & 0.940&- & 57.21 & 0.940&- & 66.80 & 0.934&- & 68.00 & 0.934&- \\
%     \midrule
%     {Relation Swapping} & 53.42 & 0.831&0.168 & 53.42 & 0.831& 0.168 & 67.00 & 0.857&0.189& 67.80& 0.857&0.189 \\
%     {Relation Replacement} & 53.42 & 0.329&0.100 & 52.22 & 0.329&0.100 & 66.80 & 0.269&0.105 & 67.60 & 0.269&0.105 \\
%     {Edge Rewiring} & 53.42 & 0.505&0.131 & 52.22 & 0.505&0.131 & 66.60 & 0.620&0.172 & 67.00 & 0.620&0.172 \\
%     {Edge Deletion} & 52.21 & 0.933&0.144 & 51.00 & 0.933&0.144 & 66.80 & 0.923&0.155& 67.60 & 0.923&0.155 \\
%     \midrule
%     {RL Relation} & \textbf{55.12} & \textbf{0.312}&0.108 & 54.63 & \textbf{0.314}&0.101 & 66.40 & 0.273&0.104 & 67.20 & 0.278&0.104 \\
%     {RL Edge} & 54.75 & 0.505&\textbf{0.082} & \textbf{55.15} & 0.542&\textbf{0.070} & 66.60 & 0.411&0.163 & 67.20 & 0.341&0.095 \\
%     % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
%     % \midrule
%     % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
%     % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
%     % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*} 


\begin{figure}[tb!]
\vspace{-0.7cm}
\centering
\subfloat[][Test Acc on CSQA]{\includegraphics[width=0.25\textwidth]{figures/final_MHGRN_Acc.png}}
\subfloat[][ATS on CSQA]{\includegraphics[width=0.25\textwidth]{figures/final_MHGRN_Val.png}}
\subfloat[][AUC on MovieLens]{\includegraphics[width=0.25\textwidth]{figures/final_reco_AUC.png}}
\subfloat[][ATS on MovieLens]{\includegraphics[width=0.25\textwidth]{figures/Final_reco_Val.png}}
\vspace{-0.1cm}
\caption{Variation of Performance and Evaluation Metrics with different scales of perturbation on MHGRN with CSQA and RippleNet with MovieLens-20M.  \xiang{polish and enrich caption.}}
\label{fig:final_curves}
% \caption{Variation of Performance and Validation Scores with scale of perturbation on MHGRN with CSQA.
% \xiang{add two flat curves for w/ and w/o KG accuracy.}
% \xiang{enlarge font size; remove top/leftmost boundary; remove vertical grey lines.}
% \vspace{-0.1cm}
\end{figure}


\begin{table}[t]
%\vspace{-0.6cm}
% \quad
% \parbox{0.3\linewidth}{
% \vspace{-0.4cm}
% %\centering
% \scalebox{0.65}{
% \begin{tabular}{lcccc}
% \toprule
%         Model & Test Acc & ATS & SC2D & SD2  \\
%         \midrule
%          Edge Rewiring& 56 & 0.46\\
%          RL-ER& 56 & 0.46\\
%          RL-RR& 56 & 0.46\\
% \bottomrule
%     \end{tabular}
%     }
%     \caption{\small Ablation Study of study different perturbation techniques on MHGRN with OBQA}
%     \label{tab:ablation}
% }
% \quad
\parbox{0.47\linewidth}{
\centering
\small\scalebox{0.75}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{CSQA}} & \multicolumn{2}{c}{\textbf{OBQA}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} & \textbf{RN}&\textbf{MHGRN}& \textbf{RN}&\textbf{MHGRN}\\
\midrule
w/o KG &53.41&53.41&62.00&62.00\\
w/ KG &56.87&57.21&66.80&68.00\\
w/ zero graph emb. &53.10&53.99&64.80&66.40\\
w/ rand. graph emb. &52.60&52.48&64.75&65.90\\
w/ rand. KG emb. &53.02&54.03&64.45&64.85\\
\bottomrule
\end{tabular}
}
\caption{\small Results of controlled noisy baselines on CSQA and OBQA. We replace the  subgraph embeddings for each instance with (1) zero vectors (w/ zero graph emb.), (2) random vectors (w/ rand. graph emb.) or replace the entities and relation embeddings with random vectors (w/ rand. KG emb.)}
\label{tab:randomized_baseline}
}
\hfill
\parbox{0.475\linewidth}{
\small
\centering
\scalebox{0.75}{\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Last.FM}} & \multicolumn{2}{c}{\textbf{MovieLens 20M}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} & \textbf{KGCN}&\textbf{RippleNet}& \textbf{KGCN}&\textbf{RippleNet}\\
\midrule
w/o KG &50.75&50.75&91.30&91.30\\
w/ KG &55.99&56.23&96.62&97.46\\
w/ rand. ngbd. &55.91&51.04&96.21&92.11\\
% w/ rand. KG emb. &53.02&54.03&53.01&56.85\\
\bottomrule
\end{tabular}}
\caption{Performance of Recommendation Models with controlled noisy baselines. \xiang{polish and enrich caption.}
% \footnote{need to explain what happen to the SC2D metric for rec dataset in footnote.}
}
}
\vspace{-0.3cm}
\end{table}


\vspace{-0.1cm}
\subsection{Recommender System Experiments}
\vspace{-0.2cm}
%Given a dataset and a KG augmented recommendation model, we try to perturb the KG using different methods and analyze the performance of the model. This task uses a subgraph sampled from the Microsoft Satori Knowledge Base.
% \xiang{what is the task/problem setting (input and output, goal)? Should introduce before going into models..}

% \textbf{Setup.} 
We conduct experiments on two recommender system benchmarks, Last.FM~\citep{rendle2012libfm} and MovieLens-20M dataset~\citep{harper2016movielens}. In particular, we use 20\% of the train set for Last.FM and 40\% of the train set for Movie Lens-20M to stimulate a cold start scenario, for which KGs are shown to be helpful~\citep{wang2018ripplenet}.
%\textbf{KG-augmented Models for Recommender Systems.}
% \xiang{similarly, 2 sentences to overview these methods.}
We adopt KGCN  and RippleNet (\textsection~\ref{sec: pilotexpts}) as our neural-symbolic recommender system. Both models are trained on the datasets and then fixed throughout the perturbation. The item KGs we aim to perturb are constructed by~\cite{wang2019aknowledge} for Last.FM and MovieLens-20M respectively. Due to the sparse nature of these item KG, the local clustering coefficient of each node is extremely small which makes the SC2D metric meaningless. Therefore, we do not report the SC2D values in this section.

% \textbf{Evaluation Protocol and Metrics.}
% The KG used for recommendation tasks has a very low clustering coefficient. Therefore, we introduce another evaluation metric, Similarity on Degree Distribution (SD2), which can also capture structural changes. Similar to the SC2D metric, we first create a set of graphs $\mathcal{G}^{r}$ for each relation $r \in \mathcal{R}$. We then calculate the relation specific degree vector $\mathbf{d^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{d^r}$ represents the degree of the $i^{th}$ node and calculate the average degree vector $\mathbf{d}$ for the whole graph as the mean of $\mathbf{d^r}$ over all $r \in \mathcal{R}$, i.e., $\mathbf{d} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{d^r}$.
% We denote the average degree vector of the unperturbed KG and the perturbed KG by $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$ respectively. We then define the SD2 metric of the KG as the reciprocal of the L2 distance between $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$, i.e.,
% $
% V_{dc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{d_{o}} - \mathbf{d_{p}} \rVert_2 + b}.
% $


\begin{table*}[tb!]
\vspace{-0.4cm}
\centering
\caption{\textbf{Performance comparison on recommender system datasets.} We report the test AUC for two KG-augmented models (KGCN and RippleNet) on Last.FM and MovieLens-20M. We perturb all the triples  (100\%) in the KG. Note that SD2C metric is not included as the local clustering coefficient is too small for the KG and thus does not provide useful insights.
% \footnote{need to explain what happen to the SC2D metric for rec dataset in footnote.}
}
\label{tab:results:reco}
\scalebox{0.60}{
\begin{tabular}{lcccccccccccc}
    \toprule  
    \multirow{2}{*}{\textbf{Methods}}&
    \multicolumn{6}{c}{ \textbf{Last.FM}}&\multicolumn{6}{c}{ \textbf{MovieLens 20M}}\\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13}
    & \multicolumn{3}{c}{ \textbf{KGCN}}&\multicolumn{3}{c}{ \textbf{RippleNet}} &\multicolumn{3}{c}{ \textbf{KGCN}} &\multicolumn{3}{c}{ \textbf{RippleNet}}\\
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    \cmidrule(lr){11-13}
    & AUC ($\uparrow$) & ATS ($\downarrow$) & SD2 ($\downarrow$) &  AUC ($\uparrow$)& ATS ($\downarrow$)  & SD2 ($\downarrow$)& AUC ($\uparrow$)& ATS ($\downarrow$)  & SD2 ($\downarrow$) & AUC ($\uparrow$)& ATS ($\downarrow$) & SD2 ($\downarrow$) \\
    \midrule
    {w/o KG} & ~50.75 & -&- & ~50.75 & -&- & ~91.30 & -&- & ~91.30 & -&- \\
    {w/ KG} & 55.99 & 0.972&- & 56.23 & 0.972&- & 96.62 & 0.960&- & 97.46 & 0.960&- \\
    \midrule
    {Relation Swapping} & 55.98 & 0.681&3.05E-2 & 56.23 & 0.681&3.05E-2 & \textbf{96.62} & 0.678&6.14E-4 & \textbf{97.46} & 0.678&6.14E-4 \\
    {Relation Replacement} & 55.98 & 0.415&0.339 & 56.22 & 0.415&0.339 & 96.50 & 0.413&\textbf{7.74E-5} & 97.45 & 0.413&\textbf{7.74E-5} \\
    {Edge Rewiring} & 55.98 & 0.437&1.89E-2 & 56.22& 0.437&1.89E-2 & 96.24 & 0.679&4.44E-4 & 96.62 & 0.679&4.44E-4 \\
    {Edge Deletion} & 55.96 & 0.941& 3.38E-3 & 56.21 & 0.941& 3.38E-3 & 96.36 & 0.982&1.02E-4 & 97.22 & 0.982&1.02E-4 \\
    \midrule
    {RL-ER}  & 55.49 & 0.345&5.45E-2 & 53.36 & 0.640&4.87E-2 & 94.34 & 0.654& 6.50E-2&94.08 & 0.791&5.51E-4 \\
    {RL-RR} & \textbf{56.04} & \textbf{0.320}&\textbf{1.3E-3} & \textbf{56.28} & \textbf{0.310}&\textbf{1.2E-3} & 96.53 & \textbf{0.401}&2.23E-4 & 97.25 & \textbf{0.268}&2.21E-4 \\
%     {RL Edge} & 56.23 & 7.8E-1&9.6E-1 & 56.21 & 9.4E-1&3.6E-1 & 97.46 & 6.1E-1&1.7E-1 & 97.43 & 9.3E-1&3.1E-2 \\
    % {RL Edge} & 54.75 & 0.505&\textbf{0.082} & \textbf{55.15} & 0.542&\textbf{0.070} & 66.60 & 0.411&0.163 & 67.20 & 0.341&0.095 \\
    % {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
    % \midrule
    % {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
    % {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
    % {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
    \bottomrule 
\end{tabular}
}
\vspace{-0.1cm}
\end{table*} 


\textbf{Results and analysis.} In Table~\ref{tab:results:reco}, we report the test AUC in \% and the evaluation metrics after perturbing all the triples in the KG. 
%Since clustering coefficient based evaluation metric is not very suitable for this task, we report the degree evaluation metric along with the embedding based evaluation metric. The key takeaway from Table~\ref{tab:results:reco} is that a
%We use the official split of 6:2:2 for train, dev and test set as specified in \citep{wang2019knowledge} for our experiments.
% We observe that despite a completely perturbed graph, the change in performance is statistically insignificant according to the T test with 3 independent runs regardless of what type of perturbation we do. This strongly suggests that it is the (false) connection between entities instead of the semantic stored in the KG that leads to the improvement over non-KG baseline. Thus, the neural-symbolic recommender system built on top of these false connection could hardly provide any faithful explanation.
We observe that despite a completely perturbed graph, the change in performance is statistically insignificant according to the T test with 3 independent runs regardless of what type of perturbation we do. This is an evidence to the fact that even with a completely corrupt graph the downstream models are providing improved performance over the non-KG baselines. Thus, the neural-symbolic recommender system built on top of these corrupt graphs can hardly provide any faithful explanation.
%These results provide a strong evidence to us for validating our claims that current neuro symbolic models do not capture the KG semantics and structure faithfully.

Figure~\ref{fig:final_curves} shows how the performance and the KG evaluation metric change across different scale of perturbation with RippleNet on MovieLens-20M dataset.
%We also plot curves showing the variation of performance with scale of perturbation on KGCN with Last.FM dataset. 
We observe insignificant change in performance (flat curve) regardless of the perturbation methods while the drastic drop in ATS validates the semantic of KG is indeed largely perturbed. This again strongly suggests that the models are not relying on any faithful symbolic knowledge to conduct prediction.  %Note that the drop in performance is insignificant for all scales of perturbation but the KG changes considerably as can be seen from the drastic drop in the evaluation metrics.

% \xiang{too short for this subsection; need to expand on the result discussion.}


% \begin{table*}[t]
% \centering
% \vspace{-0.2cm}
% \caption{\textbf{Performance comparison on recommendation based perturbation experiments} We report the test AUC on Last.FM and MovieLens-20M}
% \label{tab:results:reco}
% \scalebox{0.55}{
% \begin{tabular}{lcccccccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%   \multicolumn{6}{c}{ \textbf{Last.FM}}&\multicolumn{6}{c}{ \textbf{MovieLens 20M}}\\
%     \cmidrule(lr){2-7} \cmidrule(lr){8-13}
%     & \multicolumn{3}{c}{ \textbf{KGCN}}&\multicolumn{3}{c}{ \textbf{RippleNet}} &\multicolumn{3}{c}{ \textbf{KGCN}} &\multicolumn{3}{c}{ \textbf{Ripplenet}}\\
%     \cmidrule(lr){2-4}
%     \cmidrule(lr){5-7}
%     \cmidrule(lr){8-10}
%     \cmidrule(lr){11-13}
%     & Acc ($\uparrow$) & ATS ($\downarrow$) & SD2 ($\downarrow$) &  Acc & ATS ($\downarrow$) &  SD2 ($\downarrow$)& Acc & ATS ($\downarrow$) & SD2 ($\downarrow$) & Acc & ATS ($\downarrow$) &  SD2 ($\downarrow$)//
%     \midrule
%     {w/o KG $^{\dagger}$} & ~50.75 & -&- & ~50.75 & -&- & ~91.30 & -&- & ~91.30 & -&- \\
%     {w/ KG} & 55.99 & 0.972&- & 56.23 & 0.951&- & 96.62 & 0.962&- & 96.62 & 0.962&- \\
%     \midrule
%     {Relation Swapping} & 55.98 & 0.681&0.967 & 56.23 & 0.779&0.967 & 96.62 & 0.678&0.176 & 97.46 & 0.612&0.172 \\
%     {Greedy Relation Replacement} & 55.98 & 0.415&0.339 & 56.22 & 0.495&0.339 & 96.50 & 0.413&0.121 & 97.45 & 0.458&0.132 \\
%     {Edge Rewiring} & 56.04 & 0.437&0.417 & 56.22& 0.437&0.427 & 96.24 & 0.679&0.073 & 96.62 & 0.679&0.073 \\
%     {Edge Deletion} & 55.96 & 0.941&0.362 & 56.21 & 0.941&0.362 & 96.36 & 0.982&0.031 & 97.22 & 0.982&0.031 \\
%     \midrule
%     {RL Relation} & 56.23 & 0.95&- & 56.23 & 0.95&- & 97.46 & 0.96&- & 97.46 & 0.96&- \\
%     % {RL Edge} & 56.23 & 7.8E-1&9.6E-1 & 56.21 & 9.4E-1&3.6E-1 & 97.46 & 6.1E-1&1.7E-1 & 97.43 & 9.3E-1&3.1E-2 \\
%     % {RippleNet- Heuristic2} & 56.22 & 4.9E-1/-/3.4E-1 & 52.22 & 7.8E-1/-/4.2E-1 & 97.45 & 4.5E-1/-/1.3E-1 & 93.62 & 7.9E-1/-/7.6E-2 \\
%     % {RippleNet- RL} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*}

% \begin{figure}[tb!]
% \vspace{-0.2cm}
% \centering
% \subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_AUC_Music.png}}
% \subfloat[][Emb Val Score]{\includegraphics[width=0.25\textwidth]{figures/Relation_Val_score_music.png}}
% \subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Edge_AUC_Music.png}}
% \subfloat[][Degree Val Score]{\includegraphics[width=0.25\textwidth]{figures/Edge_Val_score_music.png}}
% \vspace{-0.2cm}
% \caption{Variation of Performance and Validation Scores with scale of perturbation on KGCN with Last.FM. \xiang{enlarge font size; remove top/leftmost boundary; remove vertical grey lines.}}
% \label{fig:heur_curvesKGCN}
% \end{figure}


% % In addition to MHGRN which we introduced in \ref{sec: pilotexpts} we also experiment on the following models for Commonsense Question Answering. 

% \textbf{Relation Net \citep{santoro2017simple}}: This is a path based model that has been adapted by \citep{feng2020scalable} for commonsense question answering. We use this model as it is simple yet powerful for the Commonsense Question Answering task. We augment this model with bert-base and use it on the CSQA \citep{talmor-etal-2019-commonsenseqa} and with roberta-large to use it on OBQA \citep{mihaylov-etal-2018-suit}. 

% \textbf{Graph Networks \citep{battaglia2018relational}}: Graph Networks is a general framework of encoding relational graphs such as a KG which we adapt to perform Commonsense Question Answering. As for Relation Net we augment this model with bert-base on CSQA and with roberta-large on OBQA.

% Since we will also perturb the structure of the KG, we need some evaluation metric that is more robust to structural changes than the ones introduced \ref{sec: pilotexpts}. To this end we introduce the following evaluation metric:

% \textbf{Clustering Coefficient based evaluation metric}: We design this evaluation metric in a way that it is robust to structural perturbation to the KG as well as perturbation to the edge types. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$ we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$ i.e $\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
%     where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$
% % \ryan{This strategy looks at triangles that are all homogeneous in terms of their relation $r$, what about triangles that are not all of the same relation $r$, but mixed relations? There are typically far more of these, just by chance. But in any case, its unclear why they were ignored. It was probably done since the above way just makes it simple to apply standard algorithms, but hopefully we have a more solid reason and justification for this.}
% We then calculate the relation specific clustering coefficient vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective} of the $i^{th}$ node and calculate the average clustering vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e $\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$
% We denote by $\mathbf{c_{o}}$, the average clustering vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{c_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ i.e
% $$V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$$
% with $b$ as a constant for avoiding zero division.

% \subsection{Recommendation}
% We introduce KGCN in \ref{sec: pilotexpts} for showcasing our pilot experiments. For this task we also work on the following model

% \textbf{Ripplenet \citep{wang2018ripplenet}} This is a KG based recommendation model that combines path based encoding and embedding based encoding of a KG. We use this model on the Last.FM and the Movie-Lens 20M datasets.

% One thing to note here is that we have a different KG for each dataset. The local clustering coefficients for the KG in this task are very small and do not provide much information. Thus for this task we introduce another evaluation metric which is quite similar to the clustering coefficient based evaluation metric.

%  \textbf{Degree Coefficient based evaluation metric: } Similar to the clustering coefficient based evaluation we first create a set of graphs $\mathcal{G}^{r}$ for each relation $r \in \mathcal{R}$. We then calculate the relation specific degree vector $\mathbf{d^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{d^r}$ represents the degree of the $i^{th}$ node and calculate the average degree vector $\mathbf{d}$ for the whole graph as the mean of $\mathbf{d^r}$ over all $r \in \mathcal{R}$ i.e $$\mathbf{d} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{d^r}$$
% We denote by $\mathbf{d_{o}}$, the average degree vector of the unperturbed KG and denote the average clustering vector of the perturbed KG with $\mathbf{d_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{d_{o}}$ and $\mathbf{d_{p}}$ i.e
% \begin{equation}
% V_{dc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{d_{o}} - \mathbf{d_{p}} \rVert_2 + b}.
% \end{equation}

% To perturb the KG to a much lower evaluation metric while preserving the accuracy, we use DQNs to model the process.To ensure we only perturb relevant facts in the KG, we extract the subgraph containing only those concepts that appear in the Question Answer statements.

% We decompose the perturbation of a relation edge into three sub-actions: choosing a subject, choosing a object connected with the chosen subject, and substituting the relation edge between the chosen subject and object with another one. We choose the first sub-action randomly at each step, and use two DQNs to predict the reward after a fixed number of steps for the other two sub-actions.
% After a fixed number of steps, we use the change of accuracy on downstream tasks as the rewards.

% We've also tried 2 variants of DQN.

% For DQN Variant 1,
% we use the difference in probabilities of the correct answer in place of accuracy as the reward. We feel this can be a more informative reward.

% For DQN Variant 2, in order to make evaluation metric as low as possible,
% we use only 1 DQN to select the tail entity and use the relation that has the lowest evaluation metric as the action. Here we only use the probability change as reward and use the greedy strategy to decrease the evaluation metric.

% In comparison, we use two random methods for perturbation.  The heuristic 1 is that we select two edges at random and swap relations and heuristic 2 is we choose tail relation randomly and select the relation which minimizes the val metric of the triple.

% Results show that our RL method does work.

% Currently our DQN method does not contain previous actions as states, but only gives predictions based on current actions. Therefore, at evaluation, if we choose the same first sub-action, the second and third sub-action will be the same, which will limit the total number of changes. 
% Therefore, we'll next try to contain previous actions as states, and use it to make more changes. This will make evaluation metric much lower.
% In addition to the models, introduced in \ref{sec: pilotexpts} we also experiment on the following models.
% % \subsection{Heuristics}
% % We consider the following heuristics as a baseline for comparison of the experiments.

% % \textbf{Heuristic1}: Choose two edges at random and swap relations. (Write it more formally)

% % \textbf{Heuristic2}: Choose an edge at random and select the relation that minimizes the embedding based evaluation metric.(Write it more formally)

% % \textbf{Edge Heuristic1}: Select an edge at random and delete it. (Write it more formally)

% % \textbf{Edge Heuristic2}: Choose an edge at random and a third node at random. Remove the original edge and add it to the third node.

% % \subsection{Question Answering}
% % We experiment on the following Question Answering datasets. We also mention the Graph Encoder used in each of them. For this set of experiments we take the complete conceptnet graph and prune it first such that it only contains edges that are relevant for the given dataset i.e for each edge either the head entity or the tail entity is a part of the given dataset.

% % \textbf{CommonsenseQA}: CommonsenseQA is a commonsense question answering benchmark dataset that is derived from conceptnet and is one of those tasks which requires external knowledge in the form of a KG to perform well. Since the labels for the official test are not available we report our results on the inhouse test split of \citep{lin2019kagnet}. We exhibit our experiments on this dataset using MHGRN \citep{feng2020scalable}, RelationNet \citep{santoro2017simple} and Graph Networks \citep{velivckovic2018graph}. 

% % \textbf{OpenBookQA}: OpenBookQA is question answering dataset that consists of science questions which shows improvement in performance after augmenting a Language Model with a KG. The labels for the official test set are available and we report our results on the official test set. As in the case of CSQA we run our experiments on MHGRN, RelationNet and Graph Networks. 

% % \subsection{Recommendation}
% % We experiment on the following Recommendation datasets. We also mention the Graph Encoder used in each of them.

% % \textbf{Last.FM}: Last.FM contains user rating information on musicians and music from a set of 2 thousand users from Last.fm online music system. We demonstrate our experiments on this dataset on KGCN and Ripplenet

% % \textbf{MovieLens 20M}: MovieLens 20M is a widely used benchmark dataset in movie recommendations, which consists of approximately 20 million explicit ratings (ranging from 1 to 5) on the MovieLens website. We showcase our experiments on this dataset using KGCN and Ripplenet.
% \textbf{Relation Net \citep{santoro2017simple}}: This is a path based model that has been adapted by \citep{feng2020scalable} for commonsense question answering. We use this model as it is simple yet powerful for the COmmonsense Question Answering task. We augment this model with bert-base and use it on the CSQA \citep{talmor-etal-2019-commonsenseqa} and with roberta-large to use it on OBQA \citep{mihaylov-etal-2018-suit}. 

% \textbf{Graph Networks \citep{battaglia2018relational}}: Graph Networks is a general framework of encoding relational graphs such as a KG which we adapt to perform Commonsense Question Answering. As for Relation Net we augment this model with bert-base on CSQA and with roberta-large on OBQA.

% \textbf{Ripplenet \citep{wang2018ripplenet}} This is a KG based recommendation model that combines path based encoding and embedding based encoding of a KG. We use this model on the Last.FM and the Movie-Lens 20M datasets.

% In the next subsection we introduce some baseline methods for the perturbation of KG.
% \subsection{Baseline Methods}
% We introduced some heuristic perturbation methods in section \ref{sec: pilotexpts}. Now we introduce some other baselines to compare our perturbation policy in addition to those introduced in \ref{sec: pilotexpts}.

% \textbf{Rewiring Heuristic: } This is a heuristic that we design to alter the structure of the graph but keep the relation distribution across the KG constant. In this heuristic we first select an edge $(h,r,t)$ randomly. We denote by $\mathcal{N}(v)$, the set of neighbors of the node v. Let $k \in \mathcal{E} \setminus \mathcal{N}(h)$. 
% Then:
% \begin{align}\label{rewiring-heuristic}
%     \mathcal{T} \leftarrow \mathcal{T} \setminus \{(h,r,t)\} \cup \{(h,r,k)\}
% \end{align}
 

% \textbf{Deletion Heuristic:} In this heuristic we randomly select an edge and delete it.
% \begin{align}\label{eq:deletion-heuristic}
%   &i \sim \text{UniformDiscrete}\{1,2,\ldots,|\mathcal{T}|\} \\
% %   ,\quad \text{for } j=1,2,\ldots\\
%     &\mathcal{T} \leftarrow \mathcal{T} \setminus \{e_i=(h,r,t)\} \nonumber
% \end{align}\noindent
% This heuristic clearly changes both the structure of the graph as well as the distribution of relations across the KG.
% This is a heuristic that clearly changes both the structure of the graph as well as the relation distribution across the KG. 
% A very interesting observation should be that the embedding based evaluation metric will fail to recognize these perturbations to the KG by design. Since even if we delete edges the remaining edges are still valid triples of the KG which in turn keeps this evaluation metric almost unchanged. 
% For the next section we denote Relation Swapping Heuristic and Greedy Heuristic as Semantic Heuristic 1 and Semantic Heuristic 2 respectively. We denote Deletion Heuristic and Rewiring Heuristic as Structure Heuristic 1 and Structure Heuristic 2 respectively

% We also introduce two more evaluation metrics in this section that are more robust to structure of the KG than the embedding based evaluation metric.

% \textbf{Clustring Coefficient/Degree based evaluation metrics} We design this evaluation metric in a way that it is robust to structural perturbation to the KG as well as perturbation to the edge types. Given a KG $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{T})$ we define $\mathcal{G}^r$ as the subgraph containing all the triples with a particular relation $r$ i.e $\mathcal{G}^r = (\mathcal{E},\mathcal{T}^{'})$
%   where $\mathcal{T}^{'}=\{(h,r',t)|h,t\in\mathcal{E},r'=r\}$
% We then calculate the relation specific clustering coefficient vector/ degee vector $\mathbf{c^r}$ for each $\mathcal{G}^r$ where $i^{th}$ element of $\mathbf{c^r}$ represents the local clustering coefficient \citep{Watts1998Collective}/ degree of the $i^{th}$ node and calculate the average clustering vector/ degree vector $\mathbf{c}$ for the whole graph as the mean of $\mathbf{c^r}$ over all $r \in \mathcal{R}$ i.e $$\mathbf{c} = \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}^{}}\mathbf{c^r}$$
% We denote by $\mathbf{c_{o}}$, the average clustering/degree vector of the unperturbed KG and denote the average clustering/degree vector of the perturbed KG with $\mathbf{c_{p}}$. We then define the evaluation metric of the KG as the reciprocal of the L2 distance between $\mathbf{c_{o}}$ and $\mathbf{c_{p}}$ i.e
% $$V_{cc}(\mathcal{G}) = \frac{1}{\lVert \mathbf{c_{o}} - \mathbf{c_{p}} \rVert_2 + b},$$
% with $b$ as a constant for avoiding zero division.

% In the next section we report our results and analysis of our experiments.

% \begin{table}[t]
% \parbox{0.45\linewidth}{
%     \begin{tabular}{lrrrr}
% \toprule
% \multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c}{CSQA} & \multicolumn{2}{c}{OBQA} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} & Val. & Int. & Val. & Int. \\
% \midrule
% Ori.& 3.03&2.17&3.48&2.17  \\
% \midrule
% RL1 &2.68&2.19&2.82&1.90\\
% RL2 &2.99&2.29&2.79&2.09\\
% \bottomrule
%     \end{tabular}
%     \caption{User Study on Paths}
%     \label{tab:user_study}
% }
% \quad
% \parbox{0.55\linewidth}{
% \begin{tabular}{c|c}
% \toprule
%          &  \\
%          & 
%     \end{tabular}
%     \caption{Abalation Study}
%     \label{tab:ablation}
% }
% \end{table}

==> backup/backup_Oct22/6_result.tex <==
% !TEX root = main.tex
\section{Results and Discussions}
Details about the results and the plots.

% \begin{table}[h]
% \centering
% \label{result-table-QA}
% \begin{center}
% \begin{tabular}{llllll}
% \multicolumn{1}{c}{\bf Model}& \multicolumn{1}{c}{\bf Perturb}  &\multicolumn{2}{c}{\bf QA1}  &\multicolumn{2}{c}{\bf QA2} 
% \\ & & Acc. &Val. & Acc. &Val.

% \\\hline \\
% Bert & - & 57.13 & 0.94& & \\
% Bert+RN & - & 59.50 &0.94 & & \\
% Bert+RN & Heuristic1 &58.10  &0.90 & & \\
% Bert+RN & Heuristic2 &58.60  &0.87 & & \\
% Bert+RN & DQN(Vanilla) &\textbf{59.45}  &\textbf{0.87} & & \\
% Bert+RN & DQN(Variant1) &59.00  &0.87 & & \\
% Bert+RN & DQN(Variant2) &59.30  &0.87 & & \\
% % \hline
% % AlBert+RN & - &  & & & \\
% % AlBert+RN & Random &  & & & \\
% % AlBert+RN & DQN &  & & & \\
% \hline
% \end{tabular}
% \caption{Accuracy of downstream tasks and validation score of the original or perturbed KG}
% \end{center}
% \end{table}

% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on CommonsenseQA and OBQA perturbation experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA and on the official set of OBQA}
% \label{tab:results:csqa}
% \scalebox{0.62}{
% \begin{tabular}{lcccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{4}{c}{ \textbf{CSQA}}&\multicolumn{4}{c}{ \textbf{OBQA}}\\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%     & \multicolumn{2}{c}{ \textbf{Semantic Perturbation}}&\multicolumn{2}{c}{ \textbf{Structure Perturbation}} &\multicolumn{2}{c}{ \textbf{Semantic Perturbation}} &\multicolumn{2}{c}{ \textbf{Structure Perturbation}}\\
%     \cmidrule(lr){2-3}
%     \cmidrule(lr){4-5}
%     \cmidrule(lr){6-7}
%     \cmidrule(lr){8-9}
%     & Acc & Emb/CC/DC &  Acc & Emb/CC/DC & Acc & Emb/CC/DC  & Acc & Emb/CC/DC \\
%     \midrule
%     {w/o KG $^{\dagger}$} & ~53.71 & -/-/- & ~53.71 & -/-/- & ~62.00 & -/-/- & ~62.00 & -/-/- \\
%     \midrule
%     {RN w KG} & 56.87 & 9.4E-1/-/- & 56.87 & 9.4E-1/-/- & 58.97 & 9.3E-1/-/- & 58.97 & 9.3E-1/-/- \\
%     {RN- Heuristic1} & 53.42 & 8.3E-1/1.6E-1/6.2E-3 & 52.21 & 9.3E-1/1.4E-1/2.0E-3 & 66.80 & 8.5E-1/1.8E-1/7.8E-3 & 66.80 & 9.2E-1/1.5E-1/2.2E-3 \\
%     {RN- Heuristic2} & 53.42 & 3.3E-1/1.0E-1/1.7E-3 & 52.53 & 5.6E-1/1.3E-1/5.4E-4 & 66.80 & 2.7E-1/1.1E-1/1.8E-3 & 66.60 & 6.2E-1/1.7E-1/7.3E-3 \\
%      {RN- RL} & 55.12 & 3.1E-1/1.1E-1/1.1E-2 & 54.15 & 5.1E-1/8.2E-2/5.2E-4 & 66.40 & 2.7E-1/1.0E-1/1.8E-3 & 66.60 & 6.5E-1/1.6E-1/8.8E-3 \\
%     \midrule
%     {MHGRN w KG} & 57.21 & 9.4E-1/-/- & 57.21 & 9.4E-1/-/- & 68 & 9.3E-1/-/- & 68 & 9.3E-1/-/- \\
%     {MHGRN- Heuristic1} & 53.42 & 8.3E-1/1.6E-1/6.2E-3 & 51.00 & 9.3E-1/1.4E-1/2.0E-3 & 67.80 & 8.5E-1/1.8E-1/7.8E-3 & 67.60 & 9.2E-1/1.5E-1/2.2E-3 \\
%     {MHGRN- Heuristic2} & 53.74 & 3.3E-1/1.0E-1/1.7E-3 & 53.02 & 6.4E-1/1.6E-1/6.1E-3 & 67.60 & 2.7E-1/1.1E-1/1.8E-3 & 67.00 & 6.5E-1/1.6E-1/8.8E-3 \\
%     {MHGRN- RL} & 53.59 & 3.4E-1/1.0E-1/1.8E-3 & 54.15 & 6.2E-1/1.2E-1/7.3E-4 & 67.20 & 2.8E-1/1.1E-1/1.8E-3 & 67.20 & 5.4E-1/9.5E-2/5.7E-4 \\
%     \midrule
%     {GN w KG} & 57.61 & 0.94/-/- & 57.61 & 0.94/-/- & 67.20 & 0.94/-/- & 67.20 & 0.94/-/- \\
%     {GN- Heuristic1} & 52.50 & 8.3E-1/1.6E-1/6.2E-3 & 50.92 & 9.3E-1/1.4E-1/2.0E-3 & 67.20 & 8.5E-1/1.8E-1/7.8E-3 & 67.20 & 9.2E-1/1.5E-1/2.2E-3 \\
%     {GN- Heuristic2} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     {GN- RL} & 53.02 & 3.3E-1/1.0E-1/1.7E-1 & 50.68 & 6.4E-1/1.6E-1/6.1E-3 & 67.20 & 2.7E-1/1.1E-1/1.8E-3 & 67.20 & 6.5E-1/1.6E-1/8.8E-3 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on CommonsenseQA in-house split for semantic based experiments.} We report in-house test accuracy using the data split of \citet{lin2019kagnet} on CommonsenseQA.}
% \label{tab:results:csqa}
% \scalebox{0.62}{
% \hskip-6.5cm
% \begin{tabular}{lcccccccccccccccccccccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{13}{c}{ \textbf{CSQA}}&\multicolumn{13}{c}{ \textbf{OBQA}}\\
%     \cmidrule(lr){2-14} \cmidrule(lr){15-27} 
%     & \multicolumn{1}{c}{\textbf{Original}}& \multicolumn{2}{c}{ \textbf{Relation Swapping}}&\multicolumn{2}{c}{ \textbf{Greedy}}&\multicolumn{2}{c}{ \textbf{RL}} &\multicolumn{2}{c}{ \textbf{Rewiring}} &\multicolumn{2}{c}{ \textbf{Deletion}}&\multicolumn{2}{c}{ \textbf{RL}}&\multicolumn{1}{c}{\textbf{Original}}&\multicolumn{2}{c}{ \textbf{Relation Swapping}}&\multicolumn{2}{c}{ \textbf{Greedy}} &\multicolumn{2}{c}{ \textbf{RL}} &\multicolumn{2}{c}{ \textbf{Rewiring}} &\multicolumn{2}{c}{ \textbf{Deletion}}&\multicolumn{2}{c}{ \textbf{RL}}\\
%     \cmidrule(lr){3-4}
%     \cmidrule(lr){5-6}
%     \cmidrule(lr){7-8}
%     \cmidrule(lr){9-10}
%     \cmidrule(lr){11-12}
%     \cmidrule(lr){13-14}
%     \cmidrule(lr){16-17}
%     \cmidrule(lr){18-19}
%     \cmidrule(lr){20-21}
%     \cmidrule(lr){22-23}
%     \cmidrule(lr){24-25}
%     \cmidrule(lr){26-27}
%     & Acc & Acc & Emb &  Acc & Emb&  Acc & Emb & Acc & CC  & Acc & CC & Acc & CC & Acc & Acc & Emb &  Acc & Emb & Acc & CC  & Acc & CC & Acc & CC & Acc & CC \\
%     \midrule
%      {w/o KG}& ~53.47 & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~62.00 & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & - \\
%      \midrule
%      RN & ~56.87 & ~53.42 & 0.831 & ~53.42 & 0.329 & ~55.12 & 0.313 & ~53.42 & 0.131 & ~52.21 &  & ~62.00 & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & -  & ~62.00 & - \\
    
%      MHGRN & ~53.47 & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~62.00 & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & -  & ~62.00 & - \\
%      GN & ~53.47 & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~53.47 & - & ~62.00 & ~62.00 & - & ~62.00 & - & ~62.00 & - & ~62.00 & -  & ~62.00 & - \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*}



% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison on recommendation based perturbation experiments} We report the test AUC on Last.FM and MovieLens-20M}
% \label{tab:results:reco}
% \scalebox{0.65}{
% \begin{tabular}{lcccccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{4}{c}{ \textbf{Last.FM}}&\multicolumn{4}{c}{ \textbf{MovieLens 20M}}\\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%     & \multicolumn{2}{c}{ \textbf{Semantic Perturbation}}&\multicolumn{2}{c}{ \textbf{Structure Perturbation}} &\multicolumn{2}{c}{ \textbf{Semantic Perturbation}} &\multicolumn{2}{c}{ \textbf{Structure Perturbation}}\\
%     \cmidrule(lr){2-3}
%     \cmidrule(lr){4-5}
%     \cmidrule(lr){6-7}
%     \cmidrule(lr){8-9}
%     & AUC & Emb/CC/DC &  AUC & Emb/CC/DC & AUC & Emb/CC/DC  & AUC & Emb/CC/DC \\
%     \midrule
%     {w/o KG $^{\dagger}$} & ~50.75 & -/-/- & ~50.75 & -/-/- & ~91.30 & -/-/- & ~91.30 & -/-/- \\
%     \midrule
%     {KGCN w KG} & 55.99 & 0.97/-/- & 55.97 & 0.97/-/- & 96.62 & 0.96/-/- & 96.62 & 0.96/-/- \\
%     {KGCN- Heuristic1} & 55.98 & 6.8E-1/-/9.7E-1 & 55.96 & 9.4E-1/-/3.6E-1 & 96.62 & 6.8E-1/-/1.8E-1 & 90.36 & 9.3E-1/-/3.1E-2 \\
%     {KGCN- Heuristic2} & 55.98 & 4.2E-1/-/3.4E-1 & 56.04 & 4.4E-1/-/4.2E-1 & 96.50 & 4.1E-1/-/1.2E-1 & 96.24 & 6.8E-1/-/7.3E-2 \\
%     {KGCN- RL} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \midrule
%     {RippleNet w KG} & 56.23 & 0.95/-/- & 56.23 & 0.95/-/- & 97.46 & 0.96/-/- & 97.46 & 0.96/-/- \\
%     {RippleNet- Heuristic1} & 56.23 & 7.8E-1/-/9.6E-1 & 56.21 & 9.4E-1/-/3.6E-1 & 97.46 & 6.1E-1/-/1.7E-1 & 97.43 & 9.3E-1/-/3.1E-2 \\
%     {RippleNet- Heuristic2} & 56.22 & 4.9E-1/-/3.4E-1 & 52.22 & 7.8E-1/-/4.2E-1 & 97.45 & 4.5E-1/-/1.3E-1 & 93.62 & 7.9E-1/-/7.6E-2 \\
%     {RippleNet- RL} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     % {RN- Rewiring} & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 & 56 & 8.9E-1/1.8E-4/2.1E-4 & 53.58 & 9.3E-1/1.6E-4/3.1E-4 \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \end{table*}



% \begin{table*}[t]
% \centering
% \scalebox{0.70}{
% \begin{tabular}{lcccccc}
%     \toprule  
%     \multirow{2}{*}{\textbf{Methods}}&
%     \multicolumn{3}{c}{ \textbf{RN with Bert-base}}&\multicolumn{3}{c}{ \textbf{GN with Bert-base}}\\
%     \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%      & Heuristic1 & Heuristic2  & RL & Heuristic1 & Heuristic2 & RL \\
%     % \midrule  
%     % {w/o KG}  & ~($\pm$)  &  .~($\pm$.)  &  52.30~($\pm$0.16) & 55.39~($\pm$0.40) & 65.56~($\pm$0.76) & 68.69($\pm$0.56) \\
%     \midrule
%     {Embedding based Val Score}  &  0.891 &  0.678  &  0.6842 & 0.891 & 0.6785 & .~($\pm$.) \\
%     {Structure based Val Score} & 18e-05  &  12e-05  &  9.54e-05 & 18e-05 & 12e-05 & .~($\pm$.) \\
%     {Dev Acc}  & 57.8 & 56.18 & 56.92 &  57.65 & 56.1 & .~($\pm$.) \\
%     {Test Acc}  & 56 & 54.15 & 55.84 &  57.05 & 57.05 & .~($\pm$.)\\
%     % {RN + Link Prediction}  & .~($\pm$.) & .~($\pm$.) & 53.96~($\pm$0.56) &  56.02~($\pm$0.55) & 66.29($~\pm$0.29) & 69.33~($\pm$0.98)\\
%     % {KagNet$^{\dagger}$~\citep{lin2019kagnet}}  &  .  &  56.19  &  . & 57.16 & - & - \\
%     % {GN}  & .~($\pm$.) & .~($\pm$.) & .~($\pm$.) &  .~($\pm$.) & 69.24($~\pm$0.56) &
%     % 72.12~($\pm$0.45)\\
%     % \midrule
%     % {Hybrid GN without edge weights} & .~($\pm$.) & \textbf{.}~($\pm$.) & .($\pm$.) &  \textbf{.}~($\pm$.)  & 70.46~($\pm$0.81)   & 72.76~($\pm$1.02)  \\
%     % {Hybrid GN with Pruning} & .~($\pm$.) & \textbf{.}~($\pm$.) & .($\pm$.) &  \textbf{.}~($\pm$.)  & 70.13~($\pm$0.82)   & 72.82~($\pm$0.89)  \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-0.1cm}
% \caption{\textbf{Performance comparison on OpenBookQA official split for semantic based perturbation.} We report test accuracy using the official data split on OpenBookQA.}
% \label{tab:results:csqa}
% \end{table*}
% \begin{figure}[h]
% \subfigure[Val score during eval]{
% \includegraphics[width=0.45\textwidth]{val_score.JPG}
% %\caption{val score during eval}
% }
% \subfigure[Loss during training of DQN(Vanilla)]{
% \includegraphics[width=0.45\textwidth]{loss_DQN.JPG}
% %\caption{loss during training of DQN(Vanilla)}
% }

% \subfigure[Accuracy on 400-size dev set during evaluation]{
% \includegraphics[width=0.45\textwidth]{acc.JPG}
% %\caption{loss during training of DQN(Vanilla)}
% }
% \caption{Plot of results.}
% \end{figure}

\begin{figure}[ht!]\label{fig:heur_curvesKGCN}
\centering
\subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Relation_AUC_Music.png}}
\subfloat[][Emb Val Score]{\includegraphics[width=0.25\textwidth]{figures/Relation_Val_score_music.png}}
\subfloat[][Test AUC on Last.FM]{\includegraphics[width=0.25\textwidth]{figures/Edge_AUC_Music.png}}
\subfloat[][Degree Val Score]{\includegraphics[width=0.25\textwidth]{figures/Edge_Val_score_music.png}}
\caption{Variation of Performance and Validation Scores with scale of perturbation on KGCN with Last.FM}
\end{figure}

\begin{figure}[ht!]\label{fig:final_curves}
\centering
\subfloat[][Test Acc on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Rel_Acc_MHGRN.png}}
\subfloat[][Emb Val Score]{\includegraphics[width=0.25\textwidth]{figures/Rel_Val_Score_MHGRN.png}}
\subfloat[][Test Acc on CSQA]{\includegraphics[width=0.25\textwidth]{figures/Edge_Acc_MHGRN.png}}
\subfloat[][Degree Val Score]{\includegraphics[width=0.25\textwidth]{figures/EDGE_val_MHGRN.png}}
\caption{Variation of Performance and Validation Scores with scale of perturbation on MHGRN with CSQA}
\end{figure}

==> backup/intro_Sep27.tex <==
% !TEX root = main.tex

\section{Introduction}
\vspace{-0.1cm}

% In many recently proposed tasks, it has been shown that performance of the system can be improved with the introduction of external knowledge. Currently Knowledge Graphs (KGs) have become the most common source of external knowledge that systems try to leverage to improve their performance. Despite having large pre-trained Language Models such as BERT, RoBERT-A, ALBERT there is a considerable performance gap between with humans on most NLP tasks. 
% Thus for these tasks researchers try to augment these language models with external knowledge for KGs. 
% The research problem of recommendation also suffers from the cold start problem \citep{wang2019knowledge} wherein the researchers try to alleviate this problem using external knowledge in the form ok a KG. In the past KGs have been used in various tasks such as Commonsense Question Answering \citep{lin2019kagnet,Shen2020ExploitingSK,Lv2020GraphBasedRO,musa2019answering}, Recommendations \citep{wang2019knowledge,Wang2020ReinforcedNS,Song2019ExplainableKG,cao2019unifying}, Natural Language Inference \citep{wang2019improving} and many others \citep{Chen2019KnowledgeawareTE,kapanipathi2020infusing}, greatly boosting model's performance compared to non-KG methods. 
% KGs have also been regarded as an important way to make the model more interpretable and generate explanations \citep{lin2019kagnet,Zhang2019InteractionEF,Song2019ExplainableKG,cao2019unifying,gao2019explainable,ai2018learning}. 
% To ensure that these KG's are used appropriately, it is of prime importance that KG based models are able to capture the semantics of a KG.

% In this paper, we investigate whether current KG methods have properly captured the semantic information from the KG, and whether the current ways of processing and encoding a KG are robust. 
% In our work, through our targeted perturbation strategy we aim to highlight potential concerns regarding reliability of current KG based models. 
% Through our experiments we also bring into light that the KG is not being utilized to its full potential and the performance can be boosted even more. We also try to argue that the interpretations generated by KG augmented models may be corrupt and thus cannot be relied upon. 
Recent machine learning benchmarks in natural language processing and data mining  pose a challenge to machines' ability in leveraging external knowledge beyond learning from the data. In particular, several commonsense Question Answering (QA) datasets~\citep{talmor2018commonsenseqa,mihaylov2018can} are designed by nature to omit the critical information that leads to the answers. In the field of recommendation systems, a commonly used recommendation algorithm, i.e., collaborative filtering, often suffers from data sparsity and cold start problem~\citep{wang2018ripplenet}. 

In response, researchers leverage knowledge graph (KG) as the source of external knowledge for tackling the aforementioned tasks with KG-augmented models. Several recent works have demonstrated KG can greatly improve the performance of the models. In commonsense QA, a sub-graph about the context is retrieved from a commonsense KG like ConceptNet~\citep{speer2016conceptnet} and serves as the evidence to infer the answer~\citep{lin2019kagnet,feng2020scalable}. In recommendation system, a KG about the items provides their semantic relatedness and thus helps machines to recommend similar items to users~\citep{wang2018ripplenet,wang2019knowledge}.

A graph encoder that learns a representation for the whole graph or each node is commonly used in these KG-augmented models. Given the heavy reliance on the graph encoders to represent the knowledge by recent works~\citep{feng2020scalable,wang2018ripplenet,wang2019knowledge}, one potential risk is that these graph encoders do not well capture both the \textit{semantic} and the \textit{graph structure} of KG as expected, which are key to incorporating helpful background knowledge for downstream tasks. Then whether the  improvement is truly brought by KG is doubtful. Therefore, we aim to investigate whether a seemly improvement can still be achieved by KG-augmented models through \textit{perturbing} the underlying KG. This is based on the assumption that, if the improvement truly comes from KG, then the KG perturbation should lead to considerable performance drop.

%However, perturbing a KG while still preserving the original performance to a large extent is challenging. 
As our pilot study, we adopt simple heuristics to randomly perturb the edges and relations of the KG and see whether a well-trained KG-augmented model would have significant performance drop. On one hand, we observe that some model can still maintain a competitive performance on the recommendation system task. On the other hand, we also observe a drastic performance drop of a recent KG-augmented model, MHGRN~\citep{feng2020scalable} on the commonsense QA task. With this regard, we conduct a more targeted study where we propose a reinforcement learning (RL) algorithm, with a dual objective of 1) perturbing the graph maximally while 2) maintaining the original performance. Our results show that with our RL-based perturbation, these KG-augmented models again manage to maintain a similar performance even though both the semantic and the structure of the underlying KG are perturbed largely. Both stydies indicate that KG is not being leveraged appropriately, or at least is not contributing to the performance of the models as we expect it to.

%It is a known fact that humans not only learn from experience but also use external knowledge to complete most of their tasks. Similarly some tasks for a machine are designed by nature to rely on external knowledge like Commonsense Question Answering and some of the tasks such as Recommendation are aided by external knowledge. Currently Knowledge Graphs (KGs) have become the most common source of external knowledge that systems try to leverage to improve their performance. Despite having large pre-trained Language Models such as BERT, RoBERT-A, ALBERT there is a considerable performance gap between with humans on most NLP tasks. Thus for these tasks researchers try to augment these language models with external knowledge for KGs. The research problem of recommendation also suffers from the cold start problem \citep{wang2019knowledge} wherein the researchers try to alleviate this problem using valuable information from a KG. 

%Most Knowledge Graph augmented models use a Graph Encoder to encode the KG. These encoders can be path based where they encode the paths between nodes or message passing based where messages are passed between neighboring nodes. In many tasks especially Commonsense QA tasks \citep{lin2019kagnet,Shen2020ExploitingSK,Lv2020GraphBasedRO,musa2019answering} we notice that the improvement of the KG augmented models over the non-KG baselines are minimal. This motivates us to examine whether the KG is truly helping in a way we believe them to help. In this work we assume that if the semantics of a KG are truly the reason for the improvement of performance then corrupting the semantics of the KG should have a very adverse effect on the performance. Through our experiments we bring into light the fact that the semantic information in the KG is probably not being utilized to its full potential. We also try to argue that the interpretations generated by KG augmented models may be corrupted and thus cannot be relied upon. To the best of our knowledge this is the first work that deals with the analysis of KG augmented models using targeted perturbations.

In summary, our main findings and contributions are as follows: (1) \textbf{Knowledge Graph Perturbation Framework:} 
We study perturbations to the knowledge graph along two dimensions, \emph{semantically} by randomization of the relation types while holding the distribution of those types to be the same (and therefore controlling for the different factors), and \emph{structure-based perturbations} that changes the connections in the knowledge graph.
(2) \textbf{Reinforcement Learning: }We demonstrate that on some tasks it is not trivial to achieve our goal of perturbing a KG while maintaining downstream performance with simple perturbations. Therefore we come up with Reinforcement Learning based perturbation policy to maximally perturb the graph while trying to maintain the downstream performance.
% summarize the main finding maybe?
(3) We find via our experiments that even with a KG that is corrupted by a sizeable amount, we are able to maintain the downstream performance on most tasks. Through our different types of perturbations we try to  demonstrate how sensitive the downstream model is to different attributes of a KG such as semantics and structure. To the best of our knowledge this is the first work that deals with the analysis of graph augmented models using targeted perturbations.

==> backup/intro_sep28.tex <==
% !TEX root = main.tex
\section{Introduction}
\vspace{-0.1cm}

%%% 1st paragraph: neural-symbolic models which incorporate symbolic structures from external knowledge graph are gaining growing popularity. 
% --> what are these models like in general?
% --> they are gaining popularity because: 1) improved accuracy on downstream tasks (e.g., overcoming data sparsity in recommendation; augmenting with commonsense knowledge in QA); and 2) these structures, in conjunction with the learn attention weights, are claimed to help provide explanation of model predictions. [Cite papers that claiming the above points].
%%
Recently the neural-symbolic models that incorporate KGs are gaining immense popularity in machine learning, especially for NLP and Data Mining tasks. A typical KG-augmented neural-symbolic model leverage either the knowledge from KGs as additional input~\citep{lin2019kagnet,feng2020scalable}, or the relational connections in KGs as a way to propagate information among the data~\citep{wang2018ripplenet,wang2019aknowledge}. %uses a graph encoder that learns a representation for the whole graph or each node and these representations are used for the downstream task \citep{lin2019kagnet, wang2019aknowledge}.
By doing so, they successfully improve the performance on downstream tasks by bringing symbolic knowledge which is essential yet absent in the input as in commonsense question answering~\citep{talmor2018commonsenseqa,mihaylov2018can} or help to address data sparsity and cold start issues as in recommendation system~\citep{jamali2010matrix,wang2018shine}.
%The increase in popularity of such models can be attributed to the boost that KG's have been shown to provide to the downstream performance \citep{feng2020scalable, Lv2020GraphBasedRO, kapanipathi2020infusing, wang2019knowledge, Wang2020ReinforcedNS}. 
More importantly, such symbolic knowledge is claimed to serve as the explanation for the models' prediction~\citep{feng2020scalable, lin2019kagnet, cao2019unifying, gao2019explainable, wang2018ripplenet}.
%Some neuro symbolic models also leverage the KG along with attention mechanisms to generate explanations for their predictions \citep{feng2020scalable, lin2019kagnet, cao2019unifying, gao2019explainable, wang2018ripplenet} which contributes to the ever rising popularity of such models.
% Recently neuro-symbolic models that incorporate symbolic data from an external knowledge base are gaining immense popularity especially for NLP and Data Mining tasks. A typical neuro-symbolic model uses a graph encoder that learns a representation for the whole graph or each node and these representations are used for the downstream task. Several recent works have demonstrated KG can greatly improve the performance of the models. In commonsense QA, a sub-graph about the context is retrieved from a commonsense KG like ConceptNet~\citep{speer2016conceptnet} and serves as the evidence to infer the answer~\citep{lin2019kagnet,feng2020scalable}. In recommendation system, a KG about the items provides their semantic relatedness and thus helps machines to recommend similar items to users~\citep{wang2018ripplenet,wang2019knowledge}.  There are many KG augmented neural models are used in conjunction with attention weights which help to make the predictions interpretable \citep{feng2020scalable, lin2019kagnet}. For recommendation systems a KG has been shown to alleviate the data sparsity and the cold start problem \citep{wang2018ripplenet, wang2019knowledge}. There have also been quite a few recent works on explainable recommendation models \citep{Song2019ExplainableKG, cao2019unifying, gao2019explainable, wang2018ripplenet} that use a KG to generate explanations. Thus the rise in popularity of neuro symbolic models can be attributed to the boost in performance and the interpretability of such models. One potential risk is that these models may not capture both the \textit{semantic} and the \textit{graph structure} of KG as expected, which are key to incorporating helpful background knowledge for downstream tasks as well as interpretability. Therefore, we aim to investigate whether the generated symbolic explanations are faithful and whether the model captures the information in the KG by  \textit{perturbing} the underlying KG. This is based on the assumption that, if the improvement truly comes from KG, then the KG perturbation should lead to considerable performance drop.
% Recent machine learning benchmarks in natural language processing and data mining  pose a challenge to machines' ability in leveraging external knowledge beyond learning from the data. In particular, several commonsense Question Answering (QA) datasets~\citep{talmor2018commonsenseqa,mihaylov2018can} are designed by nature to omit the critical information that leads to the answers. In the field of recommendation systems, a commonly used recommendation algorithm, i.e., collaborative filtering, often suffers from data sparsity and cold start problem~\citep{wang2018ripplenet}. In response, researchers leverage knowledge graph (KG) as the source of external knowledge for tackling the aforementioned tasks with KG-augmented models. Several recent works have demonstrated KG can greatly improve the performance of the models. In commonsense QA, a sub-graph about the context is retrieved from a commonsense KG like ConceptNet~\citep{speer2016conceptnet} and serves as the evidence to infer the answer~\citep{lin2019kagnet,feng2020scalable}. In recommendation system, a KG about the items provides their semantic relatedness and thus helps machines to recommend similar items to users~\citep{wang2018ripplenet,wang2019knowledge}.

%% merge into above paragraph and compress down together.
% A graph encoder that learns a representation for the whole graph or each node is commonly used in these KG-augmented models. Given the heavy reliance on the graph encoders to represent the knowledge by recent works~\citep{feng2020scalable,wang2018ripplenet,wang2019knowledge}, one potential risk is that these graph encoders do not well capture both the \textit{semantic} and the \textit{graph structure} of KG as expected, which are key to incorporating helpful background knowledge for downstream tasks. Then whether the  improvement is truly brought by information in the KG is doubtful. Therefore, we aim to investigate whether a seemly improvement can still be achieved by KG-augmented models through \textit{perturbing} the underlying KG. This is based on the assumption that, if the improvement truly comes from KG, then the KG perturbation should lead to considerable performance drop.

%%% 2nd paragraph: 
% 1) should start the paragraph with "we question whether the symbolic structures from KG (together with the associated weights) necessarily indicate the model's predictions and enhance the performance." 
% 2） and then bring out the pilot study with these simple heuristics. The main focus should be on faithfulness of the explanation (we also will include human evaluation and those are direct proof; pls stress on that).
% 3) the performance drop is a secondary claim. Please follow the abstract narrative.

In this work, we question whether the symbolic knowledge from a KG necessarily explains the model's predictions and contributes to  the performance improvement.
As our pilot study, we adopt simple heuristics to randomly perturb the edges and relations of the KG and see whether a well-trained KG-augmented model would have significant performance drop. On some cases, despite a deceptive symbolic structure, which completely deviates from the original KG, these models still manage to maintain their performance. What's worse, our later user study shows that the resulting knowledge is not faithful for explaining the models' prediction. On other cases, however, we observe noticeable performance drop for the models, indicating that a more targeted perturbation is necessary.
%Using these heuristics we try to challenge the faithfulness of the interpretations generated by the models. We also perform a user study to show the unfaithful explanations generated for a prediction by the models. There are some models that have a drastic performance drop with simple heuristic perturbations.


%%% 3rd paragraph: We need a paragraph to talk about:
% 1）what is our proposed method for solving the remaining issue in previous paragraph, and thus motivate the RL policy learning. 
% 2) And briefly introduce the solution idea of the proposed method

% \xiang{Need a paragraph for learning the policy.}
%In our pilot studies we observe a drastic performance drop of a recent KG-augmented model, MHGRN~\citep{feng2020scalable} on the commonsense QA task. 
With this regard, we conduct a more sophisticated study where we propose a reinforcement learning (RL) based perturbation algorithm. The RL algorithm learns a perturbation policy with a dual objective of 1) perturbing the graph maximally while 2) maintaining the original performance. Our results show that the proposed perturbation algorithm can learn to identify which neighbors or relations in the KG to perturb such that, these KG-augmented models again preserve their competitive performance, compared with non-KG baselines. %manage to learn deceptive symbolic structures which enable it to perform better than non KG baselines. 
%Both studies indicate that KG is not being leveraged appropriately, and the interpretations generated by the models cannot be relied upon.


%%% 4th paragraph: 1) summary of our exps and findings; 2) discuss about the implications/insights we could give to the community.
In summary, our main findings and contributions are as follows: (1) \textbf{Knowledge Graph Perturbation Framework:} 
We study perturbations to the knowledge graph along two dimensions, \emph{semantically} by randomization of the relation types while holding the distribution of those types to be the same (and therefore controlling for the different factors), and \emph{structure-based perturbations} that changes the connections in the knowledge graph.
(2) \textbf{RL-based Perturbation:} We demonstrate that on some tasks it is not trivial to achieve our goal of perturbing a KG while maintaining downstream performance with simple perturbations. Therefore we come up with RL-based perturbation policy to maximally perturb the graph while trying to maintain the downstream performance.
% summarize the main finding maybe?
(3) We find via our experiments that even with a KG that is corrupted by a sizeable amount, we are able to maintain the downstream performance on most tasks. Through our different types of perturbations we try to  demonstrate how sensitive the downstream model is to different attributes of a KG such as semantics and structure. To the best of our knowledge this is the first work that deals with the analysis of graph augmented models using targeted perturbations. 
